A Block Coordinate Descent Method for Nonsmooth Composite Optimization under Orthogonality Constraints

Nonsmooth composite optimization with orthogonality constraints has a wide range of applications in statistical learning and data science. However, this problem is challenging due to its nonsmooth objective and computationally expensive nonconvex constraints. In this paper, we propose a new approach called \textbf{OBCD}, which leverages block coordinate descent to address these challenges. \textbf{OBCD} is a feasible method with a small computational footprint. In each iteration, it updates \(k\) rows of the solution matrix, where \(k \geq 2\), by globally solving a small nonsmooth optimization problem under orthogonality constraints. We prove the completeness of the proposed update scheme, showing that row-wise orthogonal updates can reach any feasible point from any feasible initialization. We further prove that the limit points generated by \textbf{OBCD}, referred to as global block-\(k\) stationary points, offer stronger optimality than standard critical points. Furthermore, we show that \textbf{OBCD} finds an \(\epsilon\)-block-\(k\) stationary point with an iteration complexity of \(\mathcal{O}(1/\epsilon)\). Additionally, under the Kurdyka--Lojasiewicz (KL) inequality, we establish the non-ergodic convergence rate of \textbf{OBCD}. We also demonstrate how novel breakpoint search methods can be used to solve the subproblems arising in \textbf{OBCD}. Empirical results show that our approach consistently outperforms existing methods.

==> L1PCA/L0SPCA.tex <==
 


\begin{figure*}[h]
\centering
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_1.eps}
      \caption{`w1a'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_2.eps}
      \caption{`TDT2'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_3.eps}
      \caption{`20News'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_4.eps}
      \caption{`sector'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_5.eps}
      \caption{`E2006'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_6.eps}
      \caption{`MNIST'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_7.eps}
      \caption{`Gisette'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_8.eps}
      \caption{`CnnCaltech'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_9.eps}
      \caption{`Cifar'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L0PCA//demo_fig_10.eps}
      \caption{`randn'}
    \end{subfigure}
 
    \caption{The convergence curve of the compared methods for solving $L_0$ norm-based SPCA with $\lambda=100$.}
    \label{fig:L0PCA}
  \end{figure*}



 \begin{table*}[!h]
\centering
\scalebox{0.5}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n}   & \multirow{2}*{$F^*$}   & \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{PADM}  & \multirow{2}*{ODBC-R} & \multirow{2}*{ODBC-SV} &\multirow{2}*{ODBC-OR} & LADMM   & PADM \\
      &   & &    &   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=10} \\ \hline
w1a-2477-300 & -6.0e+03 & 20 & 8.70e+02& 4.98e+03& \ctwo{3.67e+01}& 3.39e+02& \cone{0.00e+00}& 3.45e+02\cone{ (+)}& \cthree{7.40e+01}\cone{ (+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.75e+00& \cthree{1.85e-02}& \ctwo{2.06e-03}& \cone{0.00e+00}& \cthree{1.85e-02}\cone{ (+)}& \cthree{1.85e-02}\cone{ (+)}\\
20News-8000-1000 & 1.8e+01 & 20 & \cthree{1.66e+00}& \cthree{1.66e+00}& \ctwo{2.19e-02}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{2.19e-02}\cone{ (+)}& \ctwo{2.19e-02}\cone{ (+)}\\
sector-6412-1000 & -2.6e+01 & 20 & 4.27e+01& 4.27e+01& \cthree{1.65e+00}& \cone{0.00e+00}& \ctwo{2.60e-01}& \cthree{1.65e+00}\cone{ (+)}& \cthree{1.65e+00}\cone{ (+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & 6.36e-01& 6.36e-01& \ctwo{5.00e-04}& \cone{0.00e+00}& \cthree{3.40e-03}& \ctwo{5.00e-04}\cone{ (+)}& \ctwo{5.00e-04}\cone{ (+)}\\
MNIST-60000-784 & -3.4e+05 & 20 & 2.40e+04& 3.41e+05& 4.09e+04& \cone{0.00e+00}& \ctwo{5.63e+03}& \cthree{1.46e+04}\cone{ (+)}& 4.09e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & 2.39e+04& 2.28e+04& 4.49e+04& \cone{0.00e+00}& 3.18e+04& \cthree{1.47e+04}\cone{ (+)}& \ctwo{1.38e+04}\cone{ (+)}\\
CnnCaltech-3000-1000 & -2.4e+03 & 20 & 8.26e+01& 1.16e+03& 7.44e+01& \ctwo{1.35e-01}& 5.04e+02& \cone{0.00e+00}\cone{ (+)}& \cthree{1.07e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 6.99e+02& \ctwo{6.56e+01}& 1.04e+04& 2.23e+03& 5.39e+03& \cthree{6.56e+02}& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -1.7e+04 & 20 & \ctwo{1.90e-03}& 1.18e+03& 7.60e+03& 7.01e+03& 6.49e+03& \cone{0.00e+00}\cone{ (+)}& \cthree{1.17e+03}\\
 \hline
w1a-2477-300 & -8.6e+03 & 50 & 2.92e+03& 2.46e+03& \cone{0.00e+00}& 7.11e+02& \cthree{2.60e+02}& \ctwo{1.99e+02}\cone{ (+)}& 2.73e+02\cone{ (+)}\\
TDT2-500-1000 & 4.6e+01 & 50 & 4.28e+00& 4.28e+00& 2.06e-02& \ctwo{3.43e-03}& \cone{0.00e+00}& \cthree{9.60e-03}\cone{ (+)}& 2.06e-02\cone{ (+)}\\
20News-8000-1000 & 4.8e+01 & 50 & 8.56e-01& 8.56e-01& \cthree{5.04e-03}& \ctwo{8.04e-04}& \cone{0.00e+00}& \cthree{5.04e-03}\cone{ (+)}& \cthree{5.04e-03}\cone{ (+)}\\
sector-6412-1000 & -1.5e+01 & 50 & 5.99e+01& 5.99e+01& \ctwo{1.18e-02}& \cone{0.00e+00}& \cthree{4.60e-02}& \ctwo{1.18e-02}\cone{ (+)}& \ctwo{1.18e-02}\cone{ (+)}\\
E2006-2000-1000 & 4.9e+01 & 50 & 6.64e-01& 6.64e-01& \ctwo{2.13e-04}& \cone{0.00e+00}& \cthree{2.51e-04}& \ctwo{2.13e-04}\cone{ (+)}& \ctwo{2.13e-04}\cone{ (+)}\\
MNIST-60000-784 & -3.5e+05 & 50 & 3.09e+04& 3.28e+04& 5.88e+04& \cone{0.00e+00}& \ctwo{8.81e+02}& \cthree{2.21e+04}\cone{ (+)}& 2.32e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 50 & 2.85e+04& 2.47e+04& 7.78e+04& \cone{0.00e+00}& 2.56e+04& \cthree{8.31e+03}\cone{ (+)}& \ctwo{3.41e+03}\cone{ (+)}\\
CnnCaltech-3000-1000 & -2.9e+03 & 50 & 4.22e+02& 1.57e+03& \cthree{1.35e+02}& \cone{0.00e+00}& 5.89e+02& 1.49e+02\cone{ (+)}& \ctwo{1.26e+02}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 50 & 3.34e+03& \ctwo{4.67e+01}& 9.69e+03& \cthree{2.88e+03}& 5.36e+03& 3.34e+03& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -3.8e+04 & 50 & \ctwo{2.26e-03}& \cthree{3.33e+03}& 1.99e+04& 1.74e+04& 1.75e+04& \cone{0.00e+00}\cone{ (+)}& \cthree{3.33e+03}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 3.52e+03& 3.26e+03& \cone{0.00e+00}& \cthree{4.81e+02}& \cthree{4.81e+02}& 7.65e+02\cone{ (+)}& \ctwo{3.06e+02}\cone{ (+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & 4.45e+00& 4.45e+00& \cone{0.00e+00}& \ctwo{1.10e-02}& \cthree{2.06e-02}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
20News-8000-1000 & 9.8e+01 & 100 & 9.25e-01& 9.25e-01& \cone{0.00e+00}& \ctwo{7.54e-04}& \cthree{8.98e-04}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.42e+01& 7.42e+01& \cone{0.00e+00}& \cthree{8.65e-01}& \ctwo{8.88e-02}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & 6.71e-01& 6.71e-01& \ctwo{1.05e-05}& \cone{0.00e+00}& \cthree{2.33e-04}& \ctwo{1.05e-05}\cone{ (+)}& \ctwo{1.05e-05}\cone{ (+)}\\
MNIST-60000-784 & -3.5e+05 & 100 & 1.93e+04& 2.08e+04& 4.40e+04& \cone{0.00e+00}& \ctwo{5.29e+03}& \cthree{7.33e+03}\cone{ (+)}& 8.46e+03\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 4.86e+04& 7.20e+04& 8.01e+04& \cone{0.00e+00}& \cthree{1.29e+04}& \ctwo{1.28e+04}\cone{ (+)}& 3.15e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & -3.5e+03 & 100 & 9.37e+02& 1.98e+03& \ctwo{1.29e+01}& \cthree{1.57e+01}& 5.08e+02& 5.26e+02\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 100 & 2.12e+04& 1.96e+04& \cthree{7.03e+03}& \cone{0.00e+00}& \ctwo{3.38e+03}& 2.12e+04& 1.95e+04\\
randn-500-1000 & -6.7e+04 & 100 & \ctwo{2.03e-03}& 3.53e+04& 3.42e+04& 3.03e+04& \cthree{2.98e+04}& \cone{0.00e+00}\cone{ (+)}& 3.53e+04\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=20} \\ \hline
w1a-2477-300 & -6.0e+03 & 20 & 8.75e+02& 4.99e+03& \cone{0.00e+00}& 4.22e+02& \ctwo{3.74e+01}& 3.26e+02\cone{ (+)}& \cthree{6.99e+01}\cone{ (+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.75e+00& \cthree{1.03e-02}& \cone{0.00e+00}& \ctwo{3.43e-03}& 1.10e-02\cone{ (+)}& 1.10e-02\cone{ (+)}\\
20News-8000-1000 & 1.8e+01 & 20 & 1.66e+00& 1.66e+00& \ctwo{7.62e-05}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{1.08e-02}\cone{ (+)}& \cthree{1.08e-02}\cone{ (+)}\\
sector-6412-1000 & -2.5e+01 & 20 & 4.25e+01& 4.25e+01& \cthree{8.84e-01}& \cone{0.00e+00}& \ctwo{6.83e-02}& 9.95e-01\cone{ (+)}& 9.95e-01\cone{ (+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & 6.38e-01& 6.38e-01& \cone{0.00e+00}& \cthree{1.20e-03}& \ctwo{4.92e-04}& 1.73e-03\cone{ (+)}& 1.73e-03\cone{ (+)}\\
MNIST-60000-784 & -3.4e+05 & 20 & 2.63e+04& 3.43e+05& 2.03e+04& \cone{0.00e+00}& \ctwo{5.73e+03}& \cthree{1.47e+04}\cone{ (+)}& 3.43e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & 2.82e+04& 2.71e+04& 3.02e+04& \cone{0.00e+00}& 2.27e+04& \cthree{1.82e+04}\cone{ (+)}& \ctwo{1.71e+04}\cone{ (+)}\\
CnnCaltech-3000-1000 & -2.5e+03 & 20 & 1.69e+02& 1.25e+03& \ctwo{5.65e+01}& \cone{0.00e+00}& 4.84e+02& 7.67e+01\cone{ (+)}& \cthree{7.64e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 7.09e+02& \ctwo{7.31e+01}& 9.22e+03& 1.34e+03& 5.01e+03& \cthree{6.61e+02}& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -1.7e+04 & 20 & \ctwo{2.02e-03}& 1.18e+03& 7.29e+03& 6.95e+03& 6.42e+03& \cone{0.00e+00}\cone{ (+)}& \cthree{1.17e+03}\\
 \hline
w1a-2477-300 & -8.6e+03 & 50 & 2.98e+03& 2.52e+03& \cone{0.00e+00}& 5.80e+02& \ctwo{7.02e+01}& \cthree{2.93e+02}\cone{ (+)}& 3.06e+02\cone{ (+)}\\
TDT2-500-1000 & 4.6e+01 & 50 & 4.29e+00& 4.29e+00& \cone{0.00e+00}& \ctwo{2.74e-03}& \cthree{4.80e-03}& 1.17e-02\cone{ (+)}& 1.17e-02\cone{ (+)}\\
20News-8000-1000 & 4.8e+01 & 50 & 8.55e-01& 8.55e-01& \ctwo{2.79e-04}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{1.76e-03}\cone{ (+)}& \cthree{1.76e-03}\cone{ (+)}\\
sector-6412-1000 & -1.5e+01 & 50 & 6.01e+01& 6.01e+01& \cthree{5.54e-02}& \cone{0.00e+00}& \ctwo{3.70e-02}& 6.44e-02\cone{ (+)}& 6.44e-02\cone{ (+)}\\
E2006-2000-1000 & 4.9e+01 & 50 & 6.64e-01& 6.64e-01& \ctwo{5.06e-05}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{2.55e-04}\cone{ (+)}& \cthree{2.55e-04}\cone{ (+)}\\
MNIST-60000-784 & -3.6e+05 & 50 & 3.95e+04& 4.14e+04& 4.59e+04& \cone{0.00e+00}& \ctwo{6.36e+03}& \cthree{3.06e+04}\cone{ (+)}& 3.16e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 50 & 3.24e+04& 2.86e+04& 7.02e+04& \cone{0.00e+00}& 2.50e+04& \cthree{1.23e+04}\cone{ (+)}& \ctwo{7.33e+03}\cone{ (+)}\\
CnnCaltech-3000-1000 & -2.9e+03 & 50 & 3.67e+02& 1.51e+03& \cone{0.00e+00}& \ctwo{2.46e+01}& 4.73e+02& 9.37e+01\cone{ (+)}& \cthree{7.52e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 50 & 3.35e+03& \ctwo{4.67e+01}& 8.98e+03& \cthree{1.69e+03}& 5.10e+03& 3.34e+03& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -3.8e+04 & 50 & \ctwo{2.25e-03}& \cthree{3.33e+03}& 1.98e+04& 1.76e+04& 1.74e+04& \cone{0.00e+00}\cone{ (+)}& \cthree{3.33e+03}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 3.54e+03& 3.28e+03& \cone{0.00e+00}& 5.14e+02& \ctwo{2.95e+02}& 6.96e+02\cone{ (+)}& \cthree{3.23e+02}\cone{ (+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & 4.45e+00& 4.45e+00& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{2.06e-03}& \cthree{3.43e-03}\cone{ (+)}& \cthree{3.43e-03}\cone{ (+)}\\
20News-8000-1000 & 9.8e+01 & 100 & 9.26e-01& 9.26e-01& \ctwo{5.67e-04}& \cone{0.00e+00}& \cthree{1.10e-03}& 1.40e-03\cone{ (+)}& 1.40e-03\cone{ (+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.45e+01& 7.45e+01& \cone{0.00e+00}& \ctwo{1.28e-01}& 2.76e-01& \cthree{2.50e-01}\cone{ (+)}& \cthree{2.50e-01}\cone{ (+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & 6.72e-01& 6.72e-01& \ctwo{3.58e-05}& \cone{0.00e+00}& \cthree{1.00e-04}& 3.60e-04\cone{ (+)}& 3.60e-04\cone{ (+)}\\
MNIST-60000-784 & -3.6e+05 & 100 & 2.70e+04& 2.85e+04& 4.69e+04& \cone{0.00e+00}& \ctwo{6.40e+03}& \cthree{1.51e+04}\cone{ (+)}& 1.61e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 4.51e+04& 4.27e+04& 7.71e+04& \cone{0.00e+00}& 1.38e+04& \cthree{8.70e+03}\cone{ (+)}& \ctwo{3.50e+03}\cone{ (+)}\\
CnnCaltech-3000-1000 & -3.6e+03 & 100 & 6.82e+02& 2.01e+03& \cone{0.00e+00}& \ctwo{1.14e+01}& 4.44e+02& 2.79e+02\cone{ (+)}& \cthree{2.52e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 100 & 8.07e+03& \cthree{2.79e+03}& 7.05e+03& \cone{0.00e+00}& 3.69e+03& 8.06e+03& \ctwo{2.73e+03}\\
randn-500-1000 & -6.7e+04 & 100 & \ctwo{2.04e-03}& \cthree{7.83e+03}& 3.41e+04& 3.01e+04& 3.02e+04& \cone{0.00e+00}\cone{ (+)}& \cthree{7.83e+03}\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=30} \\ \hline
w1a-2477-300 & -6.1e+03 & 20 & 8.78e+02& 4.99e+03& \cone{0.00e+00}& 4.78e+02& \cthree{1.39e+02}& 3.18e+02\cone{ (+)}& \ctwo{5.09e+01}\cone{ (+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.75e+00& \ctwo{6.86e-03}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{1.10e-02}\cone{ (+)}& \cthree{1.10e-02}\cone{ (+)}\\
20News-8000-1000 & 1.8e+01 & 20 & \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{1.08e-02}\cone{ (+)}& \ctwo{1.08e-02}\cone{ (+)}\\
sector-6412-1000 & -2.6e+01 & 20 & 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{1.42e-14}& \cthree{1.19e+00}\cone{ (+)}& \cthree{1.19e+00}\cone{ (+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & 6.38e-01& 6.38e-01& \cone{0.00e+00}& \ctwo{3.36e-04}& \ctwo{3.36e-04}& \cthree{1.73e-03}\cone{ (+)}& \cthree{1.73e-03}\cone{ (+)}\\
MNIST-60000-784 & -3.4e+05 & 20 & 2.63e+04& 3.43e+05& \cthree{1.29e+04}& \cone{0.00e+00}& \ctwo{2.74e+03}& 1.49e+04\cone{ (+)}& 3.61e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & 2.35e+04& 2.24e+04& 2.06e+04& \cone{0.00e+00}& 1.41e+04& \cthree{1.34e+04}\cone{ (+)}& \ctwo{1.25e+04}\cone{ (+)}\\
CnnCaltech-3000-1000 & -2.5e+03 & 20 & 1.43e+02& 1.22e+03& \cone{0.00e+00}& \ctwo{1.53e+01}& 3.15e+02& 5.35e+01\cone{ (+)}& \cthree{4.84e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 7.10e+02& \ctwo{7.32e+01}& 8.90e+03& 1.71e+03& 4.79e+03& \cthree{6.61e+02}& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -1.7e+04 & 20 & \ctwo{1.99e-03}& 1.18e+03& 7.15e+03& 6.91e+03& 6.73e+03& \cone{0.00e+00}\cone{ (+)}& \cthree{1.17e+03}\\
 \hline
w1a-2477-300 & -8.6e+03 & 50 & 2.99e+03& 2.53e+03& \cone{0.00e+00}& 6.30e+02& \ctwo{3.24e+01}& \cthree{2.98e+02}\cone{ (+)}& 3.56e+02\cone{ (+)}\\
TDT2-500-1000 & 4.6e+01 & 50 & 4.29e+00& 4.29e+00& \cone{0.00e+00}& \ctwo{3.43e-03}& \ctwo{3.43e-03}& \cthree{1.23e-02}\cone{ (+)}& 1.44e-02\cone{ (+)}\\
20News-8000-1000 & 4.8e+01 & 50 & 8.55e-01& 8.55e-01& \ctwo{6.77e-05}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{1.76e-03}\cone{ (+)}& \cthree{1.76e-03}\cone{ (+)}\\
sector-6412-1000 & -1.5e+01 & 50 & 6.00e+01& 6.00e+01& \ctwo{3.79e-03}& \cone{0.00e+00}& 1.25e-01& \cthree{4.80e-02}\cone{ (+)}& \cthree{4.80e-02}\cone{ (+)}\\
E2006-2000-1000 & 4.9e+01 & 50 & 6.64e-01& 6.64e-01& \cone{0.00e+00}& \ctwo{1.53e-05}& \cone{0.00e+00}& \cthree{8.88e-05}\cone{ (+)}& \cthree{8.88e-05}\cone{ (+)}\\
MNIST-60000-784 & -3.6e+05 & 50 & 4.09e+04& 4.28e+04& 3.76e+04& \cone{0.00e+00}& \ctwo{5.22e+03}& \cthree{3.19e+04}\cone{ (+)}& 3.31e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 50 & 3.45e+04& 3.07e+04& 6.56e+04& \cone{0.00e+00}& 2.24e+04& \cthree{1.43e+04}\cone{ (+)}& \ctwo{9.52e+03}\cone{ (+)}\\
CnnCaltech-3000-1000 & -3.0e+03 & 50 & 4.87e+02& 1.63e+03& \ctwo{6.71e+01}& \cone{0.00e+00}& 5.21e+02& 2.17e+02\cone{ (+)}& \cthree{1.93e+02}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 50 & 3.35e+03& \ctwo{4.65e+01}& 8.48e+03& \cthree{1.56e+03}& 4.86e+03& 3.35e+03& \cone{0.00e+00}\cone{ (+)}\\
randn-500-1000 & -3.8e+04 & 50 & \ctwo{2.26e-03}& \cthree{3.33e+03}& 1.97e+04& 1.77e+04& 1.73e+04& \cone{0.00e+00}\cone{ (+)}& \cthree{3.33e+03}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 3.55e+03& 3.29e+03& \cone{0.00e+00}& 5.28e+02& \cthree{4.09e+02}& 8.37e+02\cone{ (+)}& \ctwo{3.17e+02}\cone{ (+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & \cthree{4.45e+00}& \cthree{4.45e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{4.80e-03}\cone{ (+)}& \ctwo{4.80e-03}\cone{ (+)}\\
20News-8000-1000 & 9.8e+01 & 100 & 9.26e-01& 9.26e-01& \cthree{9.31e-05}& \cone{0.00e+00}& \ctwo{1.69e-05}& 1.25e-03\cone{ (+)}& 1.25e-03\cone{ (+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.45e+01& 7.45e+01& \cthree{9.80e-03}& \ctwo{1.50e-03}& \cone{0.00e+00}& 2.72e-01\cone{ (+)}& 2.72e-01\cone{ (+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & 6.72e-01& 6.72e-01& \ctwo{3.81e-05}& \cone{0.00e+00}& \cthree{3.56e-04}& 4.16e-04\cone{ (+)}& 4.16e-04\cone{ (+)}\\
MNIST-60000-784 & -3.6e+05 & 100 & 2.64e+04& 2.80e+04& 4.42e+04& \cone{0.00e+00}& \ctwo{2.36e+03}& \cthree{1.46e+04}\cone{ (+)}& 1.56e+04\cone{ (+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 4.89e+04& 4.64e+04& 7.75e+04& \cone{0.00e+00}& \cthree{1.10e+04}& 1.26e+04\cone{ (+)}& \ctwo{7.26e+03}\cone{ (+)}\\
CnnCaltech-3000-1000 & -3.6e+03 & 100 & 7.40e+02& 2.07e+03& \ctwo{2.64e+01}& \cone{0.00e+00}& 5.13e+02& 3.36e+02\cone{ (+)}& \cthree{8.59e+01}\cone{ (+)}\\
Cifar-1000-1000 & -1.4e+05 & 100 & 8.91e+03& \cthree{3.56e+03}& 7.52e+03& \cone{0.00e+00}& 4.47e+03& 8.90e+03& \ctwo{3.49e+03}\\
randn-500-1000 & -6.7e+04 & 100 & \ctwo{2.03e-03}& \cthree{7.83e+03}& 3.41e+04& 2.97e+04& 3.02e+04& \cone{0.00e+00}\cone{ (+)}& \cthree{7.83e+03}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F_{\text{min}})$ of $L_0$ norm-based SPCA for all the compared methods with $\lambda=1$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$.}
\label{tab:L0PCA:1}
\end{table*}






 \begin{table*}[!h]
\centering
\scalebox{0.5}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n}   & \multirow{2}*{$F^*$}   & \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{PADM}  & \multirow{2}*{ODBC-R} & \multirow{2}*{ODBC-SV} &\multirow{2}*{ODBC-OR} & LADMM   & PADM \\
      &   & &    &   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 300.00, time limit=10} \\ \hline
w1a-2477-300 & 1.3e+03 & 20 & \cthree{2.35e+03}& 3.90e+03& \ctwo{9.09e-13}& \ctwo{9.09e-13}& \ctwo{9.09e-13}& \ctwo{9.09e-13}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 6.0e+03 & 20 & 1.00e+00& 6.82e-01& \ctwo{1.10e-02}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{2.19e-02}\cone{ (+)}& \cthree{2.19e-02}\cone{ (+)}\\
20News-8000-1000 & 6.0e+03 & 20 & 3.71e-01& 3.41e-01& \cthree{1.08e-02}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{4.76e-03}\cone{ (+)}& \ctwo{4.76e-03}\cone{ (+)}\\
sector-6412-1000 & 6.0e+03 & 20 & 6.19e+02& 3.05e+02& \cthree{9.27e-01}& \ctwo{3.06e-01}& \cone{0.00e+00}& 3.01e+02\cone{ (+)}& 3.01e+02\\
E2006-2000-1000 & 6.0e+03 & 20 & 1.20e+03& 1.44e-01& \cthree{1.03e-03}& \cone{0.00e+00}& \ctwo{4.95e-04}& 6.00e+02\cone{ (+)}& \cthree{1.03e-03}\cone{ (+)}\\
MNIST-60000-784 & -1.8e+05 & 20 & 4.01e+04& 1.82e+05& \cone{0.00e+00}& \cthree{1.73e+04}& 3.70e+04& \ctwo{1.46e+04}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
Gisette-3000-1000 & -7.7e+05 & 20 & 2.29e+04& 4.28e+05& 1.03e+05& \cone{0.00e+00}& \cthree{1.30e+04}& \ctwo{1.08e+04}\cone{ (+)}& 3.13e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 5.4e+03 & 20 & 2.59e+03& 1.42e+04& \cthree{4.63e+00}& \ctwo{2.62e-01}& \cone{0.00e+00}& 1.15e+03\cone{ (+)}& 9.73e+03\cone{ (+)}\\
Cifar-1000-1000 & 2.0e+03 & 20 & 4.15e+04& \cthree{1.10e+03}& \ctwo{1.81e+00}& \cone{0.00e+00}& \cone{0.00e+00}& 3.91e+04& \ctwo{1.81e+00}\cone{ (+)}\\
randn-500-1000 & 1.4e+02 & 20 & 1.62e+04& 1.51e+04& \ctwo{1.69e+01}& \cone{0.00e+00}& \cone{0.00e+00}& 5.09e+03\cone{ (+)}& \cthree{3.93e+03}\cone{ (+)}\\
 \hline
w1a-2477-300 & 6.8e+03 & 50 & 5.26e+03& \cthree{4.14e+03}& \ctwo{3.64e-12}& \ctwo{3.64e-12}& \ctwo{3.64e-12}& \cone{0.00e+00}\cone{ (+)}& \ctwo{3.64e-12}\cone{ (+)}\\
TDT2-500-1000 & 1.5e+04 & 50 & 9.01e+02& 1.17e+00& \cthree{7.54e-03}& \cone{0.00e+00}& \ctwo{6.86e-04}& 3.00e+02\cone{ (+)}& 1.23e-02\cone{ (+)}\\
20News-8000-1000 & 1.5e+04 & 50 & 2.76e+04& 3.85e-01& 1.79e-03& \cone{0.00e+00}& \cthree{5.50e-04}& 1.11e+04\cone{ (+)}& \ctwo{4.40e-04}\cone{ (+)}\\
sector-6412-1000 & 1.5e+04 & 50 & 2.12e+03& 1.51e+03& \ctwo{7.02e-02}& \cone{0.00e+00}& \cthree{1.33e-01}& 2.10e+03& 1.20e+03\cone{ (+)}\\
E2006-2000-1000 & 1.5e+04 & 50 & 2.40e+03& 1.42e-01& \cone{0.00e+00}& \cthree{1.02e-04}& 2.43e-04& 2.10e+03\cone{ (+)}& \ctwo{1.11e-05}\cone{ (+)}\\
MNIST-60000-784 & -2.1e+05 & 50 & 6.06e+04& 1.07e+05& \cone{0.00e+00}& \cthree{1.19e+04}& 3.98e+04& \ctwo{1.18e+04}\cone{ (+)}& 1.58e+04\cone{ (+)}\\
Gisette-3000-1000 & -7.9e+05 & 50 & 2.18e+05& 7.30e+05& \cthree{9.65e+04}& \cone{0.00e+00}& \ctwo{8.62e+03}& 1.89e+05\cone{ (+)}& 1.03e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.4e+04 & 50 & 1.14e+03& 2.47e+03& \ctwo{4.09e-01}& \cone{0.00e+00}& \cthree{6.09e-01}& 6.01e+02\cone{ (+)}& 2.09e+03\cone{ (+)}\\
Cifar-1000-1000 & 5.1e+03 & 50 & 3.63e+04& 2.38e+03& \cthree{9.66e+00}& \cone{0.00e+00}& \ctwo{3.64e-12}& 3.34e+04& \cthree{9.66e+00}\cone{ (+)}\\
randn-500-1000 & 7.6e+02 & 50 & 2.93e+04& 2.02e+03& \cthree{4.90e+00}& \cone{0.00e+00}& \ctwo{1.73e+00}& 1.31e+04\cone{ (+)}& 5.58e+02\cone{ (+)}\\
 \hline
w1a-2477-300 & 1.8e+04 & 100 & 5.87e+03& 6.01e+03& \ctwo{1.17e-05}& \cthree{3.00e+00}& \ctwo{1.17e-05}& \ctwo{1.17e-05}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 3.0e+04 & 100 & 9.90e+03& 1.20e+03& \cone{0.00e+00}& \ctwo{6.86e-04}& \cthree{4.12e-03}& 8.70e+03\cone{ (+)}& 6.00e+02\cone{ (+)}\\
20News-8000-1000 & 3.0e+04 & 100 & 1.20e+04& 9.01e+02& \cone{0.00e+00}& \ctwo{1.02e-03}& \cthree{1.80e-03}& 7.20e+03\cone{ (+)}& 9.00e+02\\
sector-6412-1000 & 3.0e+04 & 100 & 1.23e+04& 6.02e+03& \cone{0.00e+00}& \cthree{3.82e-01}& \ctwo{3.60e-01}& 1.05e+04\cone{ (+)}& 3.90e+03\cone{ (+)}\\
E2006-2000-1000 & 3.0e+04 & 100 & 1.17e+04& 1.31e-01& \ctwo{1.51e-04}& \cthree{2.44e-04}& 2.79e-04& 9.90e+03\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
MNIST-60000-784 & -2.6e+05 & 100 & 1.01e+05& 2.25e+05& \cone{0.00e+00}& \ctwo{1.79e+04}& 4.50e+04& \cthree{1.92e+04}\cone{ (+)}& 3.04e+04\cone{ (+)}\\
Gisette-3000-1000 & -8.3e+05 & 100 & 6.40e+04& 7.13e+05& 9.31e+04& \cone{0.00e+00}& \cthree{1.43e+04}& \ctwo{1.58e+03}\cone{ (+)}& 9.92e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 2.8e+04 & 100 & 1.54e+03& 4.88e+03& \cone{0.00e+00}& \cthree{9.84e-01}& \ctwo{5.11e-02}& 6.00e+02\cone{ (+)}& 3.51e+03\cone{ (+)}\\
Cifar-1000-1000 & 1.1e+04 & 100 & 3.43e+04& 3.82e+03& \cthree{1.33e+01}& \cone{0.00e+00}& \ctwo{2.24e+00}& 2.84e+04\cone{ (+)}& \cthree{1.33e+01}\cone{ (+)}\\
randn-500-1000 & 2.1e+03 & 100 & 3.63e+04& 2.90e+03& \cthree{1.12e+00}& \cone{0.00e+00}& \ctwo{1.09e+00}& 2.05e+04\cone{ (+)}& 2.67e+02\cone{ (+)}\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 300.00, time limit=20} \\ \hline
w1a-2477-300 & 1.3e+03 & 20 & \ctwo{2.35e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 6.0e+03 & 20 & 1.00e+00& 6.82e-01& \ctwo{1.03e-02}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{2.19e-02}\cone{ (+)}& \cthree{2.19e-02}\cone{ (+)}\\
20News-8000-1000 & 6.0e+03 & 20 & 3.71e-01& 3.41e-01& \ctwo{7.62e-05}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{4.76e-03}\cone{ (+)}& \cthree{4.76e-03}\cone{ (+)}\\
sector-6412-1000 & 6.0e+03 & 20 & 6.20e+02& 3.06e+02& \ctwo{1.08e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{3.01e+02}\cone{ (+)}& \cthree{3.01e+02}\\
E2006-2000-1000 & 6.0e+03 & 20 & 1.20e+03& 1.45e-01& \cone{0.00e+00}& \ctwo{1.61e-04}& \cthree{3.36e-04}& 6.00e+02\cone{ (+)}& 1.73e-03\cone{ (+)}\\
MNIST-60000-784 & -1.8e+05 & 20 & 4.54e+04& 1.87e+05& \cone{0.00e+00}& \cthree{1.28e+04}& 4.01e+04& 2.09e+04\cone{ (+)}& \ctwo{5.36e+03}\cone{ (+)}\\
Gisette-3000-1000 & -7.7e+05 & 20 & 2.75e+04& 4.32e+05& 1.04e+05& \cone{0.00e+00}& \ctwo{1.18e+04}& \cthree{1.50e+04}\cone{ (+)}& 3.16e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 5.4e+03 & 20 & 2.59e+03& 1.42e+04& \cthree{3.00e+00}& \ctwo{2.62e-01}& \cone{0.00e+00}& 1.15e+03\cone{ (+)}& 9.73e+03\cone{ (+)}\\
Cifar-1000-1000 & 2.0e+03 & 20 & 4.15e+04& 1.10e+03& \cthree{9.33e-01}& \cone{0.00e+00}& \ctwo{9.09e-13}& 3.91e+04& 1.81e+00\cone{ (+)}\\
randn-500-1000 & 1.4e+02 & 20 & 1.62e+04& 1.51e+04& \ctwo{6.40e+00}& \cone{0.00e+00}& \cone{0.00e+00}& 5.09e+03\cone{ (+)}& \cthree{3.93e+03}\cone{ (+)}\\
 \hline
w1a-2477-300 & 6.8e+03 & 50 & 5.26e+03& \cthree{4.14e+03}& \ctwo{1.82e-12}& \ctwo{1.82e-12}& \ctwo{1.82e-12}& \cone{0.00e+00}\cone{ (+)}& \ctwo{1.82e-12}\cone{ (+)}\\
TDT2-500-1000 & 1.5e+04 & 50 & 9.01e+02& 1.17e+00& \cone{0.00e+00}& \ctwo{2.74e-03}& \cthree{4.80e-03}& 3.00e+02\cone{ (+)}& 1.65e-02\cone{ (+)}\\
20News-8000-1000 & 1.5e+04 & 50 & 2.76e+04& 3.86e-01& \cthree{6.77e-04}& \ctwo{3.98e-04}& \cone{0.00e+00}& 1.11e+04\cone{ (+)}& 8.13e-04\cone{ (+)}\\
sector-6412-1000 & 1.5e+04 & 50 & 2.12e+03& 1.51e+03& \ctwo{6.12e-02}& \cthree{1.66e-01}& \cone{0.00e+00}& 2.10e+03& 1.20e+03\cone{ (+)}\\
E2006-2000-1000 & 1.5e+04 & 50 & 2.40e+03& 1.42e-01& \cthree{1.61e-04}& \cone{0.00e+00}& \ctwo{6.30e-05}& 2.10e+03\cone{ (+)}& 1.95e-04\cone{ (+)}\\
MNIST-60000-784 & -2.2e+05 & 50 & 6.61e+04& 1.12e+05& \cone{0.00e+00}& \ctwo{8.39e+03}& 4.46e+04& \cthree{1.61e+04}\cone{ (+)}& 2.12e+04\cone{ (+)}\\
Gisette-3000-1000 & -7.9e+05 & 50 & 2.09e+05& 7.34e+05& \cthree{9.61e+04}& \cone{0.00e+00}& \ctwo{8.37e+03}& 1.80e+05\cone{ (+)}& 1.07e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.4e+04 & 50 & 1.14e+03& 2.47e+03& \ctwo{3.68e-01}& \cone{0.00e+00}& \ctwo{3.68e-01}& \cthree{6.01e+02}\cone{ (+)}& 2.09e+03\cone{ (+)}\\
Cifar-1000-1000 & 5.1e+03 & 50 & 3.63e+04& 2.38e+03& \cthree{3.78e+00}& \ctwo{1.82e-12}& \cone{0.00e+00}& 3.34e+04& 9.66e+00\cone{ (+)}\\
randn-500-1000 & 7.6e+02 & 50 & 2.93e+04& 2.02e+03& \cthree{2.34e+00}& \cone{0.00e+00}& \ctwo{1.31e+00}& 1.28e+04\cone{ (+)}& 5.59e+02\cone{ (+)}\\
 \hline
w1a-2477-300 & 1.8e+04 & 100 & \cthree{5.87e+03}& 6.01e+03& \ctwo{3.48e-05}& \ctwo{3.48e-05}& \ctwo{3.48e-05}& \ctwo{3.48e-05}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 3.0e+04 & 100 & 9.90e+03& 1.20e+03& \cone{0.00e+00}& \ctwo{6.86e-04}& \cthree{2.06e-03}& 8.70e+03\cone{ (+)}& 6.00e+02\cone{ (+)}\\
20News-8000-1000 & 3.0e+04 & 100 & 1.20e+04& 9.01e+02& \ctwo{5.17e-04}& \cone{0.00e+00}& \cthree{9.74e-04}& 7.20e+03\cone{ (+)}& 9.00e+02\\
sector-6412-1000 & 3.0e+04 & 100 & 1.23e+04& 6.02e+03& \ctwo{2.12e-02}& \cone{0.00e+00}& \cthree{3.71e-01}& 1.05e+04\cone{ (+)}& 3.90e+03\cone{ (+)}\\
E2006-2000-1000 & 3.0e+04 & 100 & 1.17e+04& 1.31e-01& \cthree{6.55e-05}& \cone{0.00e+00}& \ctwo{2.58e-05}& 9.90e+03\cone{ (+)}& 2.39e-04\cone{ (+)}\\
MNIST-60000-784 & -2.6e+05 & 100 & 1.08e+05& 2.33e+05& \cone{0.00e+00}& \ctwo{1.92e+04}& 4.84e+04& \cthree{2.68e+04}\cone{ (+)}& 3.88e+04\cone{ (+)}\\
Gisette-3000-1000 & -8.4e+05 & 100 & 7.16e+04& 7.20e+05& 9.50e+04& \cone{0.00e+00}& \cthree{9.73e+03}& \ctwo{9.05e+03}\cone{ (+)}& 1.05e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 2.8e+04 & 100 & 1.54e+03& 4.88e+03& \cthree{3.33e-01}& \ctwo{2.94e-01}& \cone{0.00e+00}& 6.01e+02\cone{ (+)}& 3.52e+03\cone{ (+)}\\
Cifar-1000-1000 & 1.1e+04 & 100 & 3.43e+04& 3.82e+03& \ctwo{4.20e+00}& \cone{0.00e+00}& \cthree{4.58e+00}& 2.85e+04\cone{ (+)}& 1.77e+01\cone{ (+)}\\
randn-500-1000 & 2.1e+03 & 100 & 3.63e+04& 2.91e+03& \ctwo{9.40e-01}& \cone{0.00e+00}& \cthree{2.20e+00}& 2.05e+04\cone{ (+)}& 2.72e+02\cone{ (+)}\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 300.00, time limit=30} \\ \hline
w1a-2477-300 & 1.3e+03 & 20 & \ctwo{2.35e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 6.0e+03 & 20 & 1.00e+00& 6.82e-01& \cthree{6.86e-03}& \cone{0.00e+00}& \ctwo{3.43e-03}& 2.19e-02\cone{ (+)}& 2.19e-02\cone{ (+)}\\
20News-8000-1000 & 6.0e+03 & 20 & 3.71e-01& \cthree{3.41e-01}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{4.76e-03}\cone{ (+)}& \ctwo{4.76e-03}\cone{ (+)}\\
sector-6412-1000 & 6.0e+03 & 20 & 6.20e+02& \cthree{3.06e+02}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{3.01e+02}\cone{ (+)}& \ctwo{3.01e+02}\\
E2006-2000-1000 & 6.0e+03 & 20 & 1.20e+03& 1.45e-01& \cone{0.00e+00}& \ctwo{3.36e-04}& \cone{0.00e+00}& 6.00e+02\cone{ (+)}& \cthree{1.73e-03}\cone{ (+)}\\
MNIST-60000-784 & -1.8e+05 & 20 & 4.69e+04& 1.88e+05& \cone{0.00e+00}& 2.80e+04& 4.05e+04& \cthree{2.14e+04}\cone{ (+)}& \ctwo{6.85e+03}\cone{ (+)}\\
Gisette-3000-1000 & -7.7e+05 & 20 & 2.71e+04& 4.32e+05& 1.01e+05& \cone{0.00e+00}& \ctwo{9.38e+03}& \cthree{1.53e+04}\cone{ (+)}& 3.14e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 5.4e+03 & 20 & 2.59e+03& 1.42e+04& \cthree{1.91e+00}& \cone{0.00e+00}& \ctwo{2.62e-01}& 1.15e+03\cone{ (+)}& 9.73e+03\cone{ (+)}\\
Cifar-1000-1000 & 2.0e+03 & 20 & 4.15e+04& 1.10e+03& \ctwo{1.38e-01}& \cone{0.00e+00}& \cone{0.00e+00}& 3.91e+04& \cthree{1.81e+00}\cone{ (+)}\\
randn-500-1000 & 1.4e+02 & 20 & 1.62e+04& 1.51e+04& \cthree{9.61e-01}& \cone{0.00e+00}& \ctwo{1.82e-12}& 5.09e+03\cone{ (+)}& 3.93e+03\cone{ (+)}\\
 \hline
w1a-2477-300 & 6.8e+03 & 50 & 5.26e+03& \cthree{4.14e+03}& \ctwo{1.82e-12}& \ctwo{1.82e-12}& \ctwo{1.82e-12}& \cone{0.00e+00}\cone{ (+)}& \ctwo{1.82e-12}\cone{ (+)}\\
TDT2-500-1000 & 1.5e+04 & 50 & 9.01e+02& 1.17e+00& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{6.86e-03}& 3.00e+02\cone{ (+)}& \cthree{1.71e-02}\cone{ (+)}\\
20News-8000-1000 & 1.5e+04 & 50 & 2.76e+04& 3.86e-01& \ctwo{4.66e-04}& \cone{0.00e+00}& \cone{0.00e+00}& 1.11e+04\cone{ (+)}& \cthree{8.13e-04}\cone{ (+)}\\
sector-6412-1000 & 1.5e+04 & 50 & 2.12e+03& 1.51e+03& \ctwo{2.60e-02}& \cone{0.00e+00}& \cthree{1.41e-01}& 2.10e+03& 1.20e+03\cone{ (+)}\\
E2006-2000-1000 & 1.5e+04 & 50 & 2.40e+03& 1.42e-01& \ctwo{6.30e-05}& \cone{0.00e+00}& \ctwo{6.30e-05}& 2.10e+03\cone{ (+)}& \cthree{1.63e-04}\cone{ (+)}\\
MNIST-60000-784 & -2.2e+05 & 50 & 7.01e+04& 1.16e+05& \cone{0.00e+00}& \cthree{2.20e+04}& 4.82e+04& \ctwo{2.15e+04}\cone{ (+)}& 2.62e+04\cone{ (+)}\\
Gisette-3000-1000 & -8.0e+05 & 50 & 2.17e+05& 7.41e+05& \cthree{9.95e+04}& \cone{0.00e+00}& \ctwo{1.21e+04}& 1.89e+05\cone{ (+)}& 1.13e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.4e+04 & 50 & 1.14e+03& 2.47e+03& \ctwo{3.54e-01}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{6.01e+02}\cone{ (+)}& 2.09e+03\cone{ (+)}\\
Cifar-1000-1000 & 5.1e+03 & 50 & 3.63e+04& 2.38e+03& \cthree{3.65e+00}& \ctwo{3.64e-12}& \cone{0.00e+00}& 3.34e+04& 9.66e+00\cone{ (+)}\\
randn-500-1000 & 7.6e+02 & 50 & 2.93e+04& 2.02e+03& \ctwo{7.15e-01}& \cthree{9.00e-01}& \cone{0.00e+00}& 1.28e+04\cone{ (+)}& 5.59e+02\cone{ (+)}\\
 \hline
w1a-2477-300 & 1.8e+04 & 100 & \cthree{5.87e+03}& 6.01e+03& \ctwo{4.46e-06}& \ctwo{4.46e-06}& \ctwo{4.46e-06}& \ctwo{4.46e-06}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 3.0e+04 & 100 & 9.90e+03& 1.20e+03& \cone{0.00e+00}& \ctwo{2.06e-03}& \cthree{2.74e-03}& 8.70e+03\cone{ (+)}& 6.00e+02\cone{ (+)}\\
20News-8000-1000 & 3.0e+04 & 100 & 1.20e+04& 9.01e+02& \ctwo{2.62e-04}& \cone{0.00e+00}& \cthree{9.48e-04}& 7.20e+03\cone{ (+)}& 9.00e+02\\
sector-6412-1000 & 3.0e+04 & 100 & 1.23e+04& 6.02e+03& \cone{0.00e+00}& \ctwo{6.26e-02}& \cthree{1.73e-01}& 1.05e+04\cone{ (+)}& 4.20e+03\cone{ (+)}\\
E2006-2000-1000 & 3.0e+04 & 100 & 1.17e+04& 1.31e-01& \cone{0.00e+00}& \ctwo{1.10e-04}& \cthree{2.39e-04}& 9.90e+03\cone{ (+)}& 2.42e-04\cone{ (+)}\\
MNIST-60000-784 & -2.6e+05 & 100 & 1.09e+05& 2.34e+05& \cone{0.00e+00}& \ctwo{2.08e+04}& 4.91e+04& \cthree{2.94e+04}\cone{ (+)}& 4.34e+04\cone{ (+)}\\
Gisette-3000-1000 & -8.4e+05 & 100 & 7.56e+04& 7.24e+05& 9.50e+04& \cone{0.00e+00}& \ctwo{1.18e+04}& \cthree{1.52e+04}\cone{ (+)}& 1.12e+05\cone{ (+)}\\
CnnCaltech-3000-1000 & 2.8e+04 & 100 & 1.54e+03& 4.88e+03& \cthree{2.36e-01}& \ctwo{1.54e-02}& \cone{0.00e+00}& 6.02e+02\cone{ (+)}& 3.52e+03\cone{ (+)}\\
Cifar-1000-1000 & 1.1e+04 & 100 & 3.43e+04& 3.82e+03& \cthree{3.34e+00}& \cone{0.00e+00}& \ctwo{6.39e-01}& 2.88e+04\cone{ (+)}& 1.97e+01\cone{ (+)}\\
randn-500-1000 & 2.1e+03 & 100 & 3.63e+04& 2.91e+03& \ctwo{8.94e-01}& \cone{0.00e+00}& \cthree{3.11e+00}& 2.17e+04\cone{ (+)}& 2.80e+02\cone{ (+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F^*)$ of $L_0$ norm-based SPCA for all the compared methods with $\lambda=300$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$.}
\label{tab:L0PCA:2}

\end{table*}





 \begin{table*}[!h]
\centering
\scalebox{0.5}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n}   & \multirow{2}*{$F^*$}   & \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{PADM}  & \multirow{2}*{ODBC-R} & \multirow{2}*{ODBC-SV} &\multirow{2}*{ODBC-OR} & LADMM   & PADM \\
      &   & &    &   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=10} \\ \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{2.64e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.00e+03& 6.82e-01& \cthree{1.85e-02}& \cone{0.00e+00}& \ctwo{1.71e-02}& 1.00e+03& 2.95e-02\cone{ (+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 3.00e+03& 3.00e+03& \ctwo{2.19e-02}& \cone{0.00e+00}& \cone{0.00e+00}& 3.00e+03& \cthree{1.00e+03}\cone{ (+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 3.01e+03& 3.00e+03& \cthree{1.65e+00}& \cone{0.00e+00}& \ctwo{2.60e-01}& 3.00e+03& 3.00e+03\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.00e+03& 1.15e-01& \cthree{9.69e-04}& \cone{0.00e+00}& \ctwo{2.75e-04}& 1.00e+03& \cthree{9.69e-04}\cone{ (+)}\\
MNIST-60000-784 & -6.3e+04 & 20 & 9.86e+04& 8.25e+04& \cone{0.00e+00}& \cthree{7.62e+03}& 1.73e+04& 3.81e+04\cone{ (+)}& \ctwo{2.88e+02}\cone{ (+)}\\
Gisette-3000-1000 & -2.2e+05 & 20 & 6.15e+05& 2.20e+05& \ctwo{1.19e+03}& \cone{0.00e+00}& \cthree{1.50e+03}& 5.26e+05\cone{ (+)}& 1.10e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 1.41e+04& 3.09e+04& \ctwo{4.63e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{7.94e+03}\cone{ (+)}& 1.99e+04\cone{ (+)}\\
Cifar-1000-1000 & 1.6e+04 & 20 & 1.81e+04& \cthree{1.10e+03}& \ctwo{3.03e+00}& \cone{0.00e+00}& \cone{0.00e+00}& 1.40e+04\cone{ (+)}& \ctwo{3.03e+00}\cone{ (+)}\\
randn-500-1000 & 1.4e+04 & 20 & 2.34e+04& 5.81e+04& \cthree{1.57e+01}& \cone{0.00e+00}& \ctwo{1.24e+00}& 1.27e+04\cone{ (+)}& 1.86e+04\cone{ (+)}\\
 \hline
w1a-2477-300 & 4.2e+04 & 50 & 5.09e+03& \cthree{4.79e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{5.00e-01}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 5.0e+04 & 50 & 9.00e+03& 4.00e+03& \ctwo{4.12e-03}& \cthree{1.51e-02}& \cone{0.00e+00}& 7.00e+03\cone{ (+)}& 4.00e+03\\
20News-8000-1000 & 5.0e+04 & 50 & 2.60e+04& 2.00e+03& \cthree{2.16e-03}& \ctwo{3.05e-04}& \cone{0.00e+00}& 8.00e+03\cone{ (+)}& 2.00e+03\\
sector-6412-1000 & 5.0e+04 & 50 & 7.02e+03& \cthree{3.00e+03}& \cone{0.00e+00}& \ctwo{7.31e-02}& \ctwo{7.31e-02}& 5.00e+03\cone{ (+)}& \cthree{3.00e+03}\\
E2006-2000-1000 & 5.0e+04 & 50 & 8.00e+03& 1.00e-01& 2.92e-04& \ctwo{2.11e-04}& \cone{0.00e+00}& 8.00e+03& \cthree{2.79e-04}\cone{ (+)}\\
MNIST-60000-784 & -8.6e+04 & 50 & 1.01e+05& 1.92e+05& \cone{0.00e+00}& \cthree{8.98e+03}& 2.03e+04& \ctwo{1.81e+02}\cone{ (+)}& 6.62e+04\cone{ (+)}\\
Gisette-3000-1000 & -2.3e+05 & 50 & 7.24e+05& 2.08e+05& 1.16e+04& \cone{0.00e+00}& \ctwo{2.81e+03}& 8.56e+05& \cthree{1.01e+04}\cone{ (+)}\\
CnnCaltech-3000-1000 & 4.9e+04 & 50 & 6.46e+03& 3.23e+04& \ctwo{4.09e-01}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{3.97e+03}\cone{ (+)}& 2.39e+04\cone{ (+)}\\
Cifar-1000-1000 & 4.0e+04 & 50 & 2.64e+04& \cthree{2.38e+03}& \ctwo{8.20e+00}& \cone{0.00e+00}& \cone{0.00e+00}& 2.40e+04& \ctwo{8.20e+00}\cone{ (+)}\\
randn-500-1000 & 3.6e+04 & 50 & 4.59e+04& 9.36e+03& \cthree{5.69e+00}& \ctwo{2.43e+00}& \cone{0.00e+00}& 3.45e+04\cone{ (+)}& 5.89e+03\cone{ (+)}\\
 \hline
w1a-2477-300 & 8.8e+04 & 100 & 5.95e+03& 9.30e+03& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{5.00e-01}& \cone{0.00e+00}\cone{ (+)}& \cthree{2.50e+00}\cone{ (+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 5.00e+03& 4.00e+03& \cone{0.00e+00}& \ctwo{1.37e-03}& \cthree{1.92e-02}& 5.00e+03& 4.00e+03\\
20News-8000-1000 & 1.0e+05 & 100 & 1.80e+04& 1.00e+03& \cone{0.00e+00}& \cthree{1.24e-03}& 2.54e-03& 1.70e+04& \ctwo{1.19e-04}\cone{ (+)}\\
sector-6412-1000 & 1.0e+05 & 100 & 2.60e+04& 2.40e+04& \cone{0.00e+00}& \cthree{6.34e-01}& \ctwo{4.86e-01}& 1.90e+04\cone{ (+)}& 2.40e+04\\
E2006-2000-1000 & 1.0e+05 & 100 & 5.20e+04& 1.07e-01& \cthree{2.16e-04}& \cone{0.00e+00}& 4.25e-04& 3.80e+04\cone{ (+)}& \ctwo{1.46e-04}\cone{ (+)}\\
MNIST-60000-784 & -1.2e+05 & 100 & 1.65e+05& 2.02e+05& \cone{0.00e+00}& 2.03e+04& 3.03e+04& \cthree{1.14e+04}\cone{ (+)}& \ctwo{7.02e+03}\cone{ (+)}\\
Gisette-3000-1000 & -2.4e+05 & 100 & 2.96e+04& 2.01e+05& 1.25e+04& \cone{0.00e+00}& \ctwo{6.70e+02}& \cthree{5.66e+03}\cone{ (+)}& 1.38e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 6.84e+03& 1.67e+04& \cone{0.00e+00}& \ctwo{1.40e+00}& \cthree{1.87e+00}& 5.99e+03\cone{ (+)}& 1.59e+04\\
Cifar-1000-1000 & 8.1e+04 & 100 & 7.16e+04& 3.82e+03& \cthree{1.51e+01}& \cone{0.00e+00}& \ctwo{5.56e+00}& 3.39e+04\cone{ (+)}& \cthree{1.51e+01}\cone{ (+)}\\
randn-500-1000 & 7.2e+04 & 100 & 1.05e+05& 8.62e+03& \ctwo{3.29e+00}& \cone{0.00e+00}& \cthree{4.35e+00}& 9.80e+04& 3.91e+03\cone{ (+)}\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=20} \\ \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{2.64e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.00e+03& 6.82e-01& \ctwo{1.03e-02}& \cthree{1.51e-02}& \cone{0.00e+00}& 1.00e+03& 2.19e-02\cone{ (+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 3.00e+03& 3.00e+03& \ctwo{7.62e-05}& \cone{0.00e+00}& \cone{0.00e+00}& 3.00e+03& \cthree{1.00e+03}\cone{ (+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 3.01e+03& \cthree{3.00e+03}& \ctwo{1.08e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{3.00e+03}& \cthree{3.00e+03}\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.00e+03& 1.16e-01& \cone{0.00e+00}& \cthree{6.66e-04}& \ctwo{4.34e-04}& 1.00e+03& 1.73e-03\cone{ (+)}\\
MNIST-60000-784 & -6.6e+04 & 20 & 1.02e+05& 8.60e+04& \cone{0.00e+00}& \cthree{6.08e+03}& 1.80e+04& 4.05e+04\cone{ (+)}& \ctwo{2.39e+03}\cone{ (+)}\\
Gisette-3000-1000 & -2.2e+05 & 20 & 6.09e+05& 2.21e+05& \cone{0.00e+00}& \cthree{2.07e+03}& \ctwo{1.52e+03}& 5.20e+05\cone{ (+)}& 1.13e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 1.41e+04& 3.09e+04& \ctwo{3.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{7.94e+03}\cone{ (+)}& 1.89e+04\cone{ (+)}\\
Cifar-1000-1000 & 1.6e+04 & 20 & 1.81e+04& 1.10e+03& \ctwo{9.33e-01}& \cone{0.00e+00}& \cone{0.00e+00}& 1.00e+04\cone{ (+)}& \cthree{1.81e+00}\cone{ (+)}\\
randn-500-1000 & 1.4e+04 & 20 & 2.34e+04& 5.81e+04& \cthree{6.92e+00}& \cone{0.00e+00}& \ctwo{1.82e-12}& 1.27e+04\cone{ (+)}& 1.47e+04\cone{ (+)}\\
 \hline
w1a-2477-300 & 4.2e+04 & 50 & \cthree{5.09e+03}& \ctwo{4.79e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 5.0e+04 & 50 & 9.00e+03& \cthree{4.00e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \ctwo{4.80e-03}& 7.00e+03\cone{ (+)}& \cthree{4.00e+03}\\
20News-8000-1000 & 5.0e+04 & 50 & 2.60e+04& 2.00e+03& \cthree{5.76e-04}& \ctwo{3.73e-04}& \cone{0.00e+00}& 8.00e+03\cone{ (+)}& 2.00e+03\\
sector-6412-1000 & 5.0e+04 & 50 & 7.02e+03& 3.00e+03& \cone{0.00e+00}& \cthree{8.58e-02}& \ctwo{2.87e-02}& 5.00e+03\cone{ (+)}& 3.00e+03\\
E2006-2000-1000 & 5.0e+04 & 50 & 8.00e+03& 1.00e-01& \ctwo{1.25e-04}& \cone{0.00e+00}& \cthree{2.81e-04}& 8.00e+03& 3.17e-04\cone{ (+)}\\
MNIST-60000-784 & -9.2e+04 & 50 & 1.06e+05& 1.17e+05& \cone{0.00e+00}& \cthree{1.03e+04}& 1.68e+04& \ctwo{6.41e+03}\cone{ (+)}& 1.87e+04\cone{ (+)}\\
Gisette-3000-1000 & -2.3e+05 & 50 & 5.82e+05& 2.09e+05& \cthree{9.98e+03}& \cone{0.00e+00}& \ctwo{2.49e+03}& 4.98e+05\cone{ (+)}& 1.22e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 4.9e+04 & 50 & 6.46e+03& 1.93e+04& \ctwo{3.68e-01}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{3.97e+03}\cone{ (+)}& 1.19e+04\cone{ (+)}\\
Cifar-1000-1000 & 4.0e+04 & 50 & 2.64e+04& 2.38e+03& \cthree{3.78e+00}& \cone{0.00e+00}& \ctwo{7.28e-12}& 2.40e+04& 9.66e+00\cone{ (+)}\\
randn-500-1000 & 3.6e+04 & 50 & 4.59e+04& 9.36e+03& \cthree{2.49e+00}& \ctwo{5.36e-01}& \cone{0.00e+00}& 3.45e+04\cone{ (+)}& 5.89e+03\cone{ (+)}\\
 \hline
w1a-2477-300 & 8.8e+04 & 100 & \cthree{5.95e+03}& 9.30e+03& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \ctwo{2.50e+00}\cone{ (+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 5.00e+03& 4.00e+03& \ctwo{6.86e-04}& \cthree{2.06e-03}& \cone{0.00e+00}& 5.00e+03& 4.00e+03\\
20News-8000-1000 & 1.0e+05 & 100 & 1.80e+04& 1.00e+03& \cone{0.00e+00}& \cthree{8.04e-04}& \ctwo{6.10e-04}& 1.70e+04& 9.48e-04\cone{ (+)}\\
sector-6412-1000 & 1.0e+05 & 100 & 2.60e+04& 2.40e+04& \cone{0.00e+00}& \ctwo{3.08e-01}& \cthree{4.34e-01}& 1.90e+04\cone{ (+)}& 2.40e+04\\
E2006-2000-1000 & 1.0e+05 & 100 & 5.20e+04& 1.07e-01& \cone{0.00e+00}& \cthree{9.01e-05}& \ctwo{4.69e-05}& 3.80e+04\cone{ (+)}& 2.54e-04\cone{ (+)}\\
MNIST-60000-784 & -1.2e+05 & 100 & 1.69e+05& 2.05e+05& \cone{0.00e+00}& 2.34e+04& 2.16e+04& \cthree{1.53e+04}\cone{ (+)}& \ctwo{1.09e+04}\cone{ (+)}\\
Gisette-3000-1000 & -2.5e+05 & 100 & 3.28e+04& 2.04e+05& 1.26e+04& \cone{0.00e+00}& \ctwo{1.35e+03}& \cthree{8.83e+03}\cone{ (+)}& 1.66e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 6.84e+03& 1.67e+04& \cone{0.00e+00}& \ctwo{7.36e-02}& \cthree{1.20e-01}& 5.99e+03\cone{ (+)}& 1.59e+04\\
Cifar-1000-1000 & 8.1e+04 & 100 & 7.16e+04& 3.82e+03& \ctwo{4.20e+00}& \cone{0.00e+00}& \cthree{4.40e+00}& 3.29e+04\cone{ (+)}& 1.77e+01\cone{ (+)}\\
randn-500-1000 & 7.2e+04 & 100 & 1.05e+05& 8.63e+03& \cone{0.00e+00}& \ctwo{8.01e-01}& \cthree{1.94e+00}& 9.80e+04& 3.91e+03\cone{ (+)}\\
 \hline
 \hline\hline  \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=30} \\ \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{2.64e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.00e+03& 6.82e-01& \ctwo{1.03e-02}& \cone{0.00e+00}& \cone{0.00e+00}& 1.00e+03& \cthree{2.95e-02}\cone{ (+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 3.00e+03& 3.00e+03& \ctwo{7.62e-05}& \cone{0.00e+00}& \cone{0.00e+00}& 3.00e+03& \cthree{1.00e+03}\cone{ (+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 3.01e+03& \cthree{3.00e+03}& \ctwo{8.73e-01}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{3.00e+03}& \cthree{3.00e+03}\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.00e+03& 1.16e-01& \ctwo{9.75e-05}& \cthree{4.33e-04}& \cone{0.00e+00}& 1.00e+03& 1.83e-03\cone{ (+)}\\
MNIST-60000-784 & -6.7e+04 & 20 & 1.03e+05& 8.70e+04& \cone{0.00e+00}& \cthree{1.17e+04}& 2.34e+04& 4.14e+04\cone{ (+)}& \ctwo{4.76e+03}\cone{ (+)}\\
Gisette-3000-1000 & -2.2e+05 & 20 & 6.09e+05& 2.22e+05& \ctwo{3.02e+02}& \cone{0.00e+00}& \cthree{1.81e+03}& 5.21e+05\cone{ (+)}& 1.25e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 1.41e+04& 3.09e+04& \ctwo{2.22e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cthree{7.94e+03}\cone{ (+)}& 1.99e+04\cone{ (+)}\\
Cifar-1000-1000 & 1.6e+04 & 20 & 1.81e+04& 1.10e+03& \cthree{1.38e-01}& \ctwo{1.82e-12}& \cone{0.00e+00}& 1.40e+04\cone{ (+)}& 3.03e+00\cone{ (+)}\\
randn-500-1000 & 1.4e+04 & 20 & 2.34e+04& 5.81e+04& \cthree{2.17e+00}& \cone{0.00e+00}& \ctwo{1.82e-12}& 1.37e+04\cone{ (+)}& 1.86e+04\cone{ (+)}\\
 \hline
w1a-2477-300 & 4.2e+04 & 50 & \cthree{5.09e+03}& \ctwo{4.79e+03}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \cone{0.00e+00}\cone{ (+)}\\
TDT2-500-1000 & 5.0e+04 & 50 & 9.00e+03& 4.00e+03& \cone{0.00e+00}& \cthree{7.54e-03}& \ctwo{6.86e-04}& 7.00e+03\cone{ (+)}& 4.00e+03\\
20News-8000-1000 & 5.0e+04 & 50 & 2.60e+04& 2.00e+03& \ctwo{5.33e-04}& \cthree{6.27e-04}& \cone{0.00e+00}& 9.00e+03\cone{ (+)}& 2.00e+03\\
sector-6412-1000 & 5.0e+04 & 50 & 7.02e+03& 3.00e+03& \ctwo{1.83e-02}& \cthree{1.00e-01}& \cone{0.00e+00}& 5.00e+03\cone{ (+)}& 3.00e+03\\
E2006-2000-1000 & 5.0e+04 & 50 & 8.00e+03& 1.00e-01& \cthree{9.50e-05}& \ctwo{2.09e-05}& \cone{0.00e+00}& 8.00e+03& 3.53e-04\cone{ (+)}\\
MNIST-60000-784 & -9.2e+04 & 50 & 1.07e+05& 1.17e+05& \cone{0.00e+00}& \cthree{7.67e+03}& 1.77e+04& \ctwo{7.37e+03}\cone{ (+)}& 1.98e+04\cone{ (+)}\\
Gisette-3000-1000 & -2.3e+05 & 50 & 6.32e+05& 2.10e+05& \cthree{1.02e+04}& \cone{0.00e+00}& \ctwo{2.81e+03}& 4.04e+05\cone{ (+)}& 1.27e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 4.9e+04 & 50 & 6.46e+03& 1.93e+04& \ctwo{3.68e-01}& \cone{0.00e+00}& \cthree{6.14e-01}& 3.97e+03\cone{ (+)}& 1.39e+04\cone{ (+)}\\
Cifar-1000-1000 & 4.0e+04 & 50 & 2.64e+04& 2.38e+03& \cthree{3.65e+00}& \cone{0.00e+00}& \ctwo{7.28e-12}& 2.40e+04& 1.50e+01\cone{ (+)}\\
randn-500-1000 & 3.6e+04 & 50 & 4.59e+04& 9.36e+03& \cthree{8.90e-01}& \cone{0.00e+00}& \ctwo{7.13e-01}& 3.55e+04\cone{ (+)}& 7.86e+03\cone{ (+)}\\
 \hline
w1a-2477-300 & 8.8e+04 & 100 & \cthree{5.95e+03}& 9.30e+03& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{ (+)}& \ctwo{9.73e+02}\cone{ (+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 5.00e+03& 4.00e+03& \cone{0.00e+00}& \cthree{1.37e-03}& \ctwo{6.86e-04}& 5.00e+03& 4.00e+03\\
20News-8000-1000 & 1.0e+05 & 100 & 1.80e+04& 1.00e+03& \cthree{2.46e-04}& \cone{0.00e+00}& \ctwo{2.54e-05}& 1.70e+04& 1.00e+03\\
sector-6412-1000 & 1.0e+05 & 100 & 2.60e+04& 2.40e+04& \ctwo{1.89e-02}& \cone{0.00e+00}& \cthree{2.12e-01}& 2.00e+04\cone{ (+)}& 2.40e+04\\
E2006-2000-1000 & 1.0e+05 & 100 & 5.20e+04& 1.07e-01& \ctwo{2.37e-05}& \cone{0.00e+00}& \cthree{1.58e-04}& 3.90e+04\cone{ (+)}& 3.69e-04\cone{ (+)}\\
MNIST-60000-784 & -1.2e+05 & 100 & 1.69e+05& 2.06e+05& \cone{0.00e+00}& \cthree{1.51e+04}& 2.11e+04& 1.73e+04\cone{ (+)}& \ctwo{1.39e+04}\cone{ (+)}\\
Gisette-3000-1000 & -2.5e+05 & 100 & 3.35e+04& 2.05e+05& 1.30e+04& \cone{0.00e+00}& \ctwo{2.21e+03}& \cthree{9.74e+03}\cone{ (+)}& 1.89e+04\cone{ (+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 6.84e+03& 1.67e+04& \ctwo{1.49e-01}& \cone{0.00e+00}& \cthree{1.14e+00}& 5.99e+03\cone{ (+)}& 1.59e+04\\
Cifar-1000-1000 & 8.1e+04 & 100 & 7.16e+04& 3.82e+03& \ctwo{3.34e+00}& \cone{0.00e+00}& \cone{0.00e+00}& 3.49e+04\cone{ (+)}& \cthree{1.97e+01}\cone{ (+)}\\
randn-500-1000 & 7.2e+04 & 100 & 1.05e+05& 8.63e+03& \ctwo{1.45e+00}& \cone{0.00e+00}& \cthree{4.08e+00}& 1.00e+05& 3.92e+03\cone{ (+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F^*)$ of $L_0$ norm-based SPCA for all the compared methods with $\lambda=1000$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$.}
\label{tab:L0PCA:3}

\end{table*}



==> L1PCA/L1SPCA.tex <==



\begin{figure*}[h]
\centering
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_1.eps}
      \caption{`w1a'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_2.eps}
      \caption{`TDT2'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_3.eps}
      \caption{`20News'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_4.eps}
      \caption{`sector'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_5.eps}
      \caption{`E2006'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_6.eps}
      \caption{`MNIST'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_7.eps}
      \caption{`Gisette'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_8.eps}
      \caption{`CnnCaltech'}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_9.eps}
      \caption{`Cifar'}
    \end{subfigure} \\
    \begin{subfigure}[b]{0.33\textwidth}
      \includegraphics[width=\textwidth]{L1PCA//demo_fig_10.eps}
      \caption{`randn'}
    \end{subfigure}

    \caption{The convergence curve of the compared methods for solving $L_1$ norm-based SPCA with $\lambda=100$.}
    \label{fig:L0PCA}
  \end{figure*}




\begin{table*}[!h]
\centering
\scalebox{0.52}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n} & \multirow{2}*{$F_{\text{min}}$}& \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{RSubGrad}  & \multirow{2}*{ADMM} & \multirow{2}*{ManPG} &\multirow{2}*{ODBC-OR} & LADMM   & ManPG \\
 &   &    &&   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
  \hline
   \hline\multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=10} \\ \hline
w1a-2477-300 & -5.7e+03 & 10 & \cthree{2.52e+01}& 4.71e+03& 4.85e+03& 4.71e+03& \cone{0.00e+00}& \ctwo{1.99e+01}\cone{(+)}& 4.45e+01\cone{(+)}\\
TDT2-500-1000 & 6.6e+00 & 10 & 3.40e+00& 3.40e+00& 1.51e+00& 3.40e+00& \cone{0.00e+00}& \ctwo{3.09e-02}\cone{(+)}& \cthree{9.81e-02}\cone{(+)}\\
20News-8000-1000 & 8.5e+00 & 10 & 1.49e+00& 1.62e+00& \cthree{1.30e+00}& 1.49e+00& \cone{0.00e+00}& \ctwo{3.07e-02}\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & -2.2e+01 & 10 & 3.00e+01& 3.00e+01& \cthree{1.62e+01}& 3.00e+01& \cone{0.00e+00}& \ctwo{2.73e-01}\cone{(+)}& \ctwo{2.73e-01}\cone{(+)}\\
E2006-2000-1000 & 9.4e+00 & 10 & 6.17e-01& 6.37e-01& \cthree{1.60e-01}& 6.17e-01& \ctwo{2.32e-04}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
MNIST-60000-784 & -3.1e+05 & 10 & \cthree{1.91e+02}& 3.13e+05& 3.13e+05& 3.13e+05& \cone{0.00e+00}& \ctwo{1.60e+02}\cone{(+)}& 1.23e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 2.24e+04& 4.78e+05& 7.31e+04& 3.43e+05& \cone{0.00e+00}& \ctwo{7.94e+03}\cone{(+)}& \cthree{1.39e+04}\cone{(+)}\\
CnnCaltech-3000-1000 & -4.2e+03 & 10 & 2.87e+01& \cthree{1.50e+00}& 9.33e+02& \ctwo{8.62e-03}& 2.18e+01& 2.47e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 2.75e+03& 4.28e+04& 1.22e+04& \ctwo{1.26e+00}& 2.54e+03& \cthree{1.53e+03}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
randn-500-1000 & -1.3e+04 & 10 & 2.78e+01& \cthree{1.42e+00}& 2.51e+02& \ctwo{1.10e-04}& 3.62e+01& 2.63e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -7.1e+03 & 20 & \cthree{8.04e+01}& 5.95e+03& 6.05e+03& 5.94e+03& \cone{0.00e+00}& \ctwo{4.91e+01}\cone{(+)}& 1.42e+02\cone{(+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.91e+00& \cthree{1.89e+00}& 3.75e+00& \cone{0.00e+00}& \ctwo{7.54e-03}\cone{(+)}& \ctwo{7.54e-03}\cone{(+)}\\
20News-8000-1000 & 1.8e+01 & 20 & \cthree{1.66e+00}& 1.94e+00& 5.55e+00& \cthree{1.66e+00}& \cone{0.00e+00}& \ctwo{1.08e-02}\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & -2.5e+01 & 20 & 4.25e+01& \cthree{2.97e+01}& 3.04e+01& 4.25e+01& \cone{0.00e+00}& \ctwo{9.39e-01}\cone{(+)}& \ctwo{9.39e-01}\cone{(+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & \cthree{6.37e-01}& 8.10e-01& 7.62e-01& \cthree{6.37e-01}& \cone{0.00e+00}& \ctwo{1.06e-03}\cone{(+)}& \ctwo{1.06e-03}\cone{(+)}\\
MNIST-60000-784 & -3.5e+05 & 20 & \ctwo{1.26e+02}& 3.54e+05& 3.54e+05& 3.54e+05& \cthree{1.45e+03}& \cone{0.00e+00}\cone{(+)}& 4.33e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{1.31e+04}& 5.01e+05& 7.75e+04& 3.57e+05& \cone{0.00e+00}& \ctwo{1.90e+03}\cone{(+)}& 2.23e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -5.1e+03 & 20 & 6.73e+01& \cthree{5.75e+00}& 1.46e+03& \ctwo{7.21e-03}& 3.08e+02& 6.04e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 20 & 3.31e+03& 4.95e+04& 1.37e+04& \ctwo{1.56e+02}& 6.46e+03& \cthree{2.66e+03}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
randn-500-1000 & -2.6e+04 & 20 & 2.56e+01& \cthree{5.82e+00}& 4.11e+02& \ctwo{1.51e-03}& 2.61e+02& 2.44e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -1.2e+04 & 100 & 1.01e+03& \ctwo{5.73e+02}& 4.31e+03& 3.97e+03& \cone{0.00e+00}& \cthree{8.59e+02}\cone{(+)}& 8.63e+02\cone{(+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & \cthree{4.44e+00}& 9.22e+00& \ctwo{3.90e+00}& \cthree{4.44e+00}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
20News-8000-1000 & 9.8e+01 & 100 & \cthree{9.25e-01}& 4.15e+00& 7.41e+01& \cthree{9.25e-01}& \ctwo{2.50e-03}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.42e+01& 6.64e+01& 6.09e+01& 7.42e+01& \cthree{1.04e+00}& \ctwo{2.84e-14}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & \cthree{6.71e-01}& 4.47e+00& 3.73e+02& \cthree{6.71e-01}& \ctwo{5.06e-05}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
MNIST-60000-784 & -3.9e+05 & 100 & \ctwo{2.89e+03}& 1.09e+05& 1.93e+05& 2.24e+05& \cthree{1.60e+04}& \cone{0.00e+00}\cone{(+)}& 7.58e+04\cone{(+)}\\
Gisette-3000-1000 & -1.2e+06 & 100 & \cthree{3.60e+04}& 8.49e+05& 1.13e+05& 3.11e+05& \ctwo{2.43e+04}& \cone{0.00e+00}\cone{(+)}& 5.83e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -6.7e+03 & 100 & \cthree{5.35e+02}& \cone{0.00e+00}& 4.43e+03& 1.40e+03& 2.24e+03& \ctwo{5.33e+02}\cone{(+)}& 1.36e+03\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 100 & \ctwo{1.08e+02}& 7.04e+04& 1.00e+04& 2.00e+04& \cthree{7.70e+03}& \cone{0.00e+00}\cone{(+)}& 8.15e+03\cone{(+)}\\
randn-500-1000 & -1.0e+05 & 100 & \cthree{1.14e+02}& \cone{0.00e+00}& 1.50e+03& \ctwo{6.03e+01}& 4.76e+04& \cthree{1.14e+02}\cone{(+)}& \ctwo{6.03e+01}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=30} \\ \hline
w1a-2477-300 & -5.7e+03 & 10 & \cthree{2.60e+01}& 4.71e+03& 4.85e+03& 4.71e+03& \cone{0.00e+00}& \ctwo{2.07e+01}\cone{(+)}& 4.53e+01\cone{(+)}\\
TDT2-500-1000 & 6.6e+00 & 10 & 3.40e+00& 3.40e+00& \cthree{1.51e+00}& 3.40e+00& \cone{0.00e+00}& \ctwo{3.09e-02}\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 8.5e+00 & 10 & 1.49e+00& 1.53e+00& \cthree{1.30e+00}& 1.49e+00& \cone{0.00e+00}& \ctwo{3.07e-02}\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & -2.2e+01 & 10 & 3.00e+01& 3.00e+01& \cthree{1.62e+01}& 3.00e+01& \cone{0.00e+00}& \ctwo{2.73e-01}\cone{(+)}& \ctwo{2.73e-01}\cone{(+)}\\
E2006-2000-1000 & 9.4e+00 & 10 & 6.17e-01& 6.23e-01& \cthree{1.60e-01}& 6.17e-01& \ctwo{6.54e-04}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
MNIST-60000-784 & -3.1e+05 & 10 & \cthree{1.97e+02}& 3.13e+05& 3.13e+05& 3.13e+05& \cone{0.00e+00}& \ctwo{1.65e+02}\cone{(+)}& 1.19e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 2.53e+04& 4.35e+05& 7.61e+04& 3.24e+05& \cone{0.00e+00}& \ctwo{1.06e+04}\cone{(+)}& \cthree{1.59e+04}\cone{(+)}\\
CnnCaltech-3000-1000 & -4.2e+03 & 10 & 2.97e+01& \cthree{1.96e+00}& 9.34e+02& \ctwo{7.40e-07}& 1.63e+01& 2.56e+01\cone{(+)}& \cone{0.00e+00}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 2.79e+03& \cone{0.00e+00}& 1.22e+04& \cthree{1.20e+01}& 1.96e+02& 1.57e+03\cone{(+)}& \ctwo{1.18e+01}\cone{(+)}\\
randn-500-1000 & -1.3e+04 & 10 & 2.87e+01& \cthree{1.88e+00}& 2.52e+02& \ctwo{6.80e-10}& 9.32e+00& 2.72e+01\cone{(+)}& \cone{0.00e+00}\\
 \hline \hline
w1a-2477-300 & -7.1e+03 & 20 & \cthree{8.24e+01}& 5.95e+03& 6.05e+03& 5.95e+03& \cone{0.00e+00}& \ctwo{5.07e+01}\cone{(+)}& 1.43e+02\cone{(+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.81e+00& \cthree{1.89e+00}& 3.75e+00& \cone{0.00e+00}& \ctwo{8.92e-03}\cone{(+)}& \ctwo{8.92e-03}\cone{(+)}\\
20News-8000-1000 & 1.8e+01 & 20 & \cthree{1.66e+00}& 1.76e+00& 5.55e+00& \cthree{1.66e+00}& \cone{0.00e+00}& \ctwo{1.08e-02}\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & -2.5e+01 & 20 & 4.25e+01& \cthree{2.92e+01}& 3.04e+01& 4.25e+01& \cone{0.00e+00}& \ctwo{9.61e-01}\cone{(+)}& \ctwo{9.61e-01}\cone{(+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & \cthree{6.38e-01}& 6.45e-01& 7.61e-01& \cthree{6.38e-01}& \cone{0.00e+00}& \ctwo{1.30e-03}\cone{(+)}& \ctwo{1.30e-03}\cone{(+)}\\
MNIST-60000-784 & -3.5e+05 & 20 & \ctwo{1.25e+02}& 3.54e+05& 3.54e+05& 3.54e+05& \cthree{2.02e+02}& \cone{0.00e+00}\cone{(+)}& 4.33e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{2.50e+04}& 4.55e+05& 8.95e+04& 3.55e+05& \cone{0.00e+00}& \ctwo{1.38e+04}\cone{(+)}& 3.72e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -5.1e+03 & 20 & 7.47e+01& \cthree{1.17e+01}& 1.47e+03& \ctwo{1.07e-05}& 4.52e+01& 6.77e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 20 & 4.40e+03& 1.02e+04& 1.48e+04& \ctwo{3.16e-01}& \cthree{2.75e+03}& 3.73e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
randn-500-1000 & -2.6e+04 & 20 & 2.78e+01& \cthree{6.97e+00}& 4.13e+02& \ctwo{5.23e-04}& 7.67e+01& 2.66e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -1.2e+04 & 100 & 1.11e+03& \ctwo{6.63e+02}& 4.41e+03& 2.20e+03& \cone{0.00e+00}& \cthree{9.60e+02}\cone{(+)}& 1.14e+03\cone{(+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & 4.45e+00& 5.91e+00& \cthree{3.90e+00}& 4.45e+00& \cone{0.00e+00}& \ctwo{3.43e-03}\cone{(+)}& \ctwo{3.43e-03}\cone{(+)}\\
20News-8000-1000 & 9.8e+01 & 100 & \cthree{9.26e-01}& 4.77e+00& 7.06e+01& \cthree{9.26e-01}& \cone{0.00e+00}& \ctwo{9.23e-04}\cone{(+)}& \ctwo{9.23e-04}\cone{(+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.45e+01& 6.46e+01& \cthree{6.12e+01}& 7.45e+01& \cone{0.00e+00}& \ctwo{2.65e-01}\cone{(+)}& \ctwo{2.65e-01}\cone{(+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & \cthree{6.72e-01}& 1.79e+00& 3.67e+02& \cthree{6.72e-01}& \cone{0.00e+00}& \ctwo{3.03e-04}\cone{(+)}& \ctwo{3.03e-04}\cone{(+)}\\
MNIST-60000-784 & -4.0e+05 & 100 & \cthree{1.38e+04}& 7.60e+04& 2.04e+05& 2.09e+05& \cone{0.00e+00}& \ctwo{1.10e+04}\cone{(+)}& 9.39e+04\cone{(+)}\\
Gisette-3000-1000 & -1.2e+06 & 100 & \cthree{3.95e+04}& 2.65e+05& 1.16e+05& 3.13e+05& \cone{0.00e+00}& \ctwo{3.52e+03}\cone{(+)}& 6.23e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -6.8e+03 & 100 & 5.46e+02& \cone{0.00e+00}& 4.43e+03& \cthree{4.48e+02}& 1.55e+03& 5.44e+02\cone{(+)}& \ctwo{4.47e+02}\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 100 & \ctwo{1.08e+02}& 4.95e+04& 9.99e+03& 1.13e+04& \cthree{4.78e+03}& \cone{0.00e+00}\cone{(+)}& 9.25e+03\cone{(+)}\\
randn-500-1000 & -1.0e+05 & 100 & \cthree{1.31e+02}& \cone{0.00e+00}& 1.50e+03& \ctwo{1.08e+00}& 2.23e+04& \cthree{1.31e+02}\cone{(+)}& \ctwo{1.08e+00}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=60} \\ \hline
w1a-2477-300 & -5.7e+03 & 10 & \cthree{2.54e+01}& 4.71e+03& 4.85e+03& 4.71e+03& \cone{0.00e+00}& \ctwo{2.01e+01}\cone{(+)}& 4.35e+01\cone{(+)}\\
TDT2-500-1000 & 6.6e+00 & 10 & 3.40e+00& 3.40e+00& \cthree{1.51e+00}& 3.40e+00& \cone{0.00e+00}& \ctwo{3.09e-02}\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 8.5e+00 & 10 & 1.49e+00& 1.50e+00& \cthree{1.30e+00}& 1.49e+00& \cone{0.00e+00}& \ctwo{3.07e-02}\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & -2.2e+01 & 10 & 3.00e+01& 3.01e+01& \cthree{1.63e+01}& 3.00e+01& \cone{0.00e+00}& \ctwo{3.54e-01}\cone{(+)}& \ctwo{3.54e-01}\cone{(+)}\\
E2006-2000-1000 & 9.4e+00 & 10 & 6.18e-01& 6.21e-01& \cthree{1.61e-01}& 6.18e-01& \cone{0.00e+00}& \ctwo{1.59e-03}\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -3.1e+05 & 10 & \cthree{1.98e+02}& 3.13e+05& 3.13e+05& 3.13e+05& \cone{0.00e+00}& \ctwo{1.66e+02}\cone{(+)}& 1.15e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 2.51e+04& 3.21e+05& 7.62e+04& 4.52e+05& \cone{0.00e+00}& \ctwo{1.06e+04}\cone{(+)}& \cthree{1.92e+04}\cone{(+)}\\
CnnCaltech-3000-1000 & -4.2e+03 & 10 & 2.97e+01& \cthree{1.77e+00}& 9.34e+02& \ctwo{3.44e-08}& 1.19e+01& 2.56e+01\cone{(+)}& \cone{0.00e+00}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 2.79e+03& \cone{0.00e+00}& 1.22e+04& \cthree{4.22e+00}& 6.36e+01& 1.60e+03\cone{(+)}& \ctwo{4.19e+00}\cone{(+)}\\
randn-500-1000 & -1.3e+04 & 10 & 2.87e+01& \cthree{1.76e+00}& 2.52e+02& \ctwo{8.33e-09}& 6.36e+00& 2.72e+01\cone{(+)}& \cone{0.00e+00}\\
 \hline \hline
w1a-2477-300 & -7.1e+03 & 20 & \cthree{9.14e+01}& 5.96e+03& 6.06e+03& 5.95e+03& \cone{0.00e+00}& \ctwo{5.89e+01}\cone{(+)}& 1.49e+02\cone{(+)}\\
TDT2-500-1000 & 1.6e+01 & 20 & 3.75e+00& 3.76e+00& \cthree{1.89e+00}& 3.75e+00& \cone{0.00e+00}& \ctwo{1.10e-02}\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 1.8e+01 & 20 & \cthree{1.66e+00}& 1.70e+00& 5.55e+00& \cthree{1.66e+00}& \cone{0.00e+00}& \ctwo{1.08e-02}\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & -2.6e+01 & 20 & 4.27e+01& \cthree{2.93e+01}& 3.07e+01& 4.27e+01& \cone{0.00e+00}& \ctwo{1.22e+00}\cone{(+)}& \ctwo{1.22e+00}\cone{(+)}\\
E2006-2000-1000 & 1.9e+01 & 20 & \cthree{6.38e-01}& 6.41e-01& 7.62e-01& \cthree{6.38e-01}& \cone{0.00e+00}& \ctwo{1.70e-03}\cone{(+)}& \ctwo{1.70e-03}\cone{(+)}\\
MNIST-60000-784 & -3.5e+05 & 20 & \cthree{3.33e+02}& 3.55e+05& 3.55e+05& 3.55e+05& \cone{0.00e+00}& \ctwo{2.09e+02}\cone{(+)}& 4.30e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{3.01e+04}& 3.92e+05& 9.47e+04& 5.14e+05& \cone{0.00e+00}& \ctwo{1.86e+04}\cone{(+)}& 3.99e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -5.1e+03 & 20 & 7.53e+01& \cthree{1.16e+01}& 1.47e+03& \ctwo{1.57e-05}& 3.28e+01& 6.83e+01\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 20 & 4.44e+03& \cone{0.00e+00}& 1.48e+04& \cthree{2.72e+01}& 1.53e+03& 3.80e+03\cone{(+)}& \ctwo{2.71e+01}\cone{(+)}\\
randn-500-1000 & -2.6e+04 & 20 & 2.85e+01& \cthree{7.30e+00}& 4.14e+02& \ctwo{1.32e-07}& 2.91e+01& 2.74e+01\cone{(+)}& \cone{0.00e+00}\\
 \hline \hline
w1a-2477-300 & -1.2e+04 & 100 & 1.16e+03& \ctwo{7.00e+02}& 4.46e+03& 1.55e+03& \cone{0.00e+00}& 1.01e+03\cone{(+)}& \cthree{9.42e+02}\cone{(+)}\\
TDT2-500-1000 & 9.5e+01 & 100 & 4.45e+00& 5.14e+00& \cthree{3.90e+00}& 4.45e+00& \cone{0.00e+00}& \ctwo{4.80e-03}\cone{(+)}& \ctwo{4.80e-03}\cone{(+)}\\
20News-8000-1000 & 9.8e+01 & 100 & \cthree{9.26e-01}& 2.71e+00& 7.06e+01& \cthree{9.26e-01}& \cone{0.00e+00}& \ctwo{1.20e-03}\cone{(+)}& \ctwo{1.20e-03}\cone{(+)}\\
sector-6412-1000 & 1.6e+01 & 100 & 7.45e+01& 6.25e+01& \cthree{6.13e+01}& 7.45e+01& \cone{0.00e+00}& \ctwo{2.94e-01}\cone{(+)}& \ctwo{2.94e-01}\cone{(+)}\\
E2006-2000-1000 & 9.9e+01 & 100 & \cthree{6.72e-01}& 1.24e+00& 3.67e+02& \cthree{6.72e-01}& \cone{0.00e+00}& \ctwo{4.65e-04}\cone{(+)}& \ctwo{4.65e-04}\cone{(+)}\\
MNIST-60000-784 & -4.1e+05 & 100 & \cthree{2.29e+04}& 6.95e+04& 2.13e+05& 2.14e+05& \cone{0.00e+00}& \ctwo{2.00e+04}\cone{(+)}& 9.80e+04\cone{(+)}\\
Gisette-3000-1000 & -1.2e+06 & 100 & \cthree{5.38e+04}& 4.49e+05& 1.30e+05& 3.25e+05& \cone{0.00e+00}& \ctwo{1.79e+04}\cone{(+)}& 7.67e+04\cone{(+)}\\
CnnCaltech-3000-1000 & -6.8e+03 & 100 & 5.51e+02& \cone{0.00e+00}& 4.43e+03& \ctwo{2.67e+02}& 1.13e+03& \cthree{5.49e+02}\cone{(+)}& \ctwo{2.67e+02}\\
Cifar-1000-1000 & -1.5e+05 & 100 & \ctwo{1.08e+02}& 4.01e+04& 9.99e+03& 1.99e+03& 2.42e+03& \cone{0.00e+00}\cone{(+)}& \cthree{1.71e+03}\cone{(+)}\\
randn-500-1000 & -1.0e+05 & 100 & 1.53e+02& \cthree{1.56e+01}& 1.53e+03& \ctwo{3.45e-03}& 1.04e+04& 1.53e+02\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F_{\text{min}})$ of $L_1$ norm-based SPCA for all the compared methods with $\lambda=1$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$.}
\label{tab:L1PCA:1}
\end{table*}


\begin{table*}[!h]
\centering
\scalebox{0.52}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n} & \multirow{2}*{$F_{\text{min}}$}& \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{RSubGrad}  & \multirow{2}*{ADMM} & \multirow{2}*{ManPG} &\multirow{2}*{ODBC-OR} & LADMM   & ManPG \\
 &   &    &&   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
  \hline
\multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=10} \\ \hline
w1a-2477-300 & -3.0e+03 & 10 & 9.05e+02& 3.48e+03& 3.57e+03& 3.57e+03& \cone{0.00e+00}& \cthree{3.74e+01}\cone{(+)}& \ctwo{1.36e+01}\cone{(+)}\\
TDT2-500-1000 & 1.0e+03 & 10 & 3.24e+01& 1.64e+02& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 2.90e+01\cone{(+)}& \ctwo{9.81e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+03 & 10 & 6.88e+01& 1.11e+03& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.76e+01\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 9.7e+02 & 10 & 1.55e+01& 8.08e+02& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{3.21e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+03 & 10 & 4.77e+01& 4.69e+02& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 1.01e+01\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -3.0e+05 & 10 & \cthree{7.53e+02}& 3.00e+05& 3.00e+05& 3.00e+05& \cone{0.00e+00}& \ctwo{6.65e+02}\cone{(+)}& 7.27e+03\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 2.35e+04& 4.70e+05& 6.42e+04& 3.99e+05& \cone{0.00e+00}& \ctwo{1.27e+04}\cone{(+)}& \cthree{1.43e+04}\cone{(+)}\\
CnnCaltech-3000-1000 & 5.9e+02 & 10 & 2.32e+02& 1.06e+03& 2.90e+02& 2.90e+02& \cone{0.00e+00}& \cthree{7.90e+01}\cone{(+)}& \ctwo{3.80e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 10 & \ctwo{2.93e+02}& 3.78e+04& 8.94e+03& 7.45e+03& \cthree{1.90e+03}& \cone{0.00e+00}\cone{(+)}& 5.76e+03\cone{(+)}\\
randn-500-1000 & -2.0e+03 & 10 & 5.40e+02& 1.17e+03& 6.68e+02& 5.12e+02& \cone{0.00e+00}& \cthree{1.57e+02}\cone{(+)}& \ctwo{5.72e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -3.3e+03 & 20 & 1.72e+03& 4.45e+03& 4.45e+03& 4.45e+03& \ctwo{5.59e+01}& \cthree{1.07e+02}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+03 & 20 & 2.71e+02& 8.34e+02& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 2.09e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+03 & 20 & 1.59e+02& 2.90e+03& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 7.94e+01\cone{(+)}& \ctwo{1.30e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+03 & 20 & 9.94e+01& 2.45e+03& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{4.21e+01}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+03 & 20 & 1.21e+02& 1.11e+03& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 8.05e+01\cone{(+)}& \ctwo{1.83e-03}\cone{(+)}\\
MNIST-60000-784 & -3.3e+05 & 20 & \cthree{3.28e+03}& 3.31e+05& 3.31e+05& 3.31e+05& \cone{0.00e+00}& \ctwo{2.11e+03}\cone{(+)}& 3.82e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{2.30e+04}& 4.72e+05& 7.61e+04& 3.72e+05& \cone{0.00e+00}& \ctwo{1.27e+04}\cone{(+)}& 3.33e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 1.4e+03 & 20 & 2.46e+02& 3.72e+03& 2.66e+03& 3.90e+02& \cone{0.00e+00}& \cthree{3.32e+01}\cone{(+)}& \ctwo{4.63e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 20 & \ctwo{3.42e+02}& 5.36e+04& 1.35e+04& 1.30e+04& \cthree{1.96e+03}& \cone{0.00e+00}\cone{(+)}& 1.06e+04\cone{(+)}\\
randn-500-1000 & -3.9e+03 & 20 & 1.25e+03& 3.69e+03& 8.33e+02& 8.19e+02& \cone{0.00e+00}& \cthree{5.13e+02}\cone{(+)}& \ctwo{1.47e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -1.7e+03 & 100 & 5.04e+03& 4.60e+03& 7.36e+03& 5.29e+03& \cthree{1.07e+02}& \ctwo{5.22e+01}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 100 & 1.09e+03& 2.73e+04& \cthree{4.45e+00}& \cthree{4.45e+00}& \ctwo{1.37e-03}& 8.51e+02\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 100 & 8.15e+02& 5.60e+04& \cthree{9.25e-01}& \cthree{9.25e-01}& \ctwo{3.90e-04}& 6.68e+02\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
sector-6412-1000 & 9.9e+03 & 100 & 6.26e+01& 5.12e+04& 7.43e+01& 7.43e+01& \cone{0.00e+00}& \cthree{8.32e+00}\cone{(+)}& \ctwo{3.75e-02}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 100 & 1.09e+03& 3.39e+04& \cthree{6.71e-01}& \cthree{6.71e-01}& \ctwo{7.81e-04}& 9.16e+02\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
MNIST-60000-784 & -3.4e+05 & 100 & \cthree{3.32e+04}& 1.24e+05& 1.57e+05& 1.75e+05& \cone{0.00e+00}& \ctwo{2.70e+04}\cone{(+)}& 6.24e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & \cthree{3.90e+04}& 5.50e+05& 1.05e+05& 3.07e+05& \ctwo{9.59e+02}& \cone{0.00e+00}\cone{(+)}& 6.87e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 7.8e+03 & 100 & 9.37e+02& 3.93e+04& 1.81e+03& 9.92e+02& \ctwo{1.88e+00}& \cthree{6.63e+01}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.2e+05 & 100 & \ctwo{2.86e+02}& 1.32e+05& 3.72e+04& 5.68e+04& \cthree{2.65e+03}& \cone{0.00e+00}\cone{(+)}& 2.62e+04\cone{(+)}\\
randn-500-1000 & -1.8e+04 & 100 & 3.78e+03& 7.11e+04& 2.74e+03& 2.74e+03& \ctwo{2.73e+00}& \cthree{1.67e+03}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=30} \\ \hline
w1a-2477-300 & -3.0e+03 & 10 & 9.10e+02& 3.49e+03& 3.58e+03& 3.58e+03& \cone{0.00e+00}& \cthree{4.31e+01}\cone{(+)}& \ctwo{1.73e+01}\cone{(+)}\\
TDT2-500-1000 & 1.0e+03 & 10 & 3.24e+01& 7.93e+01& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 2.90e+01\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+03 & 10 & 6.88e+01& 3.86e+02& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.76e+01\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 9.7e+02 & 10 & 1.55e+01& 3.52e+02& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{3.21e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+03 & 10 & 4.77e+01& 2.10e+02& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 1.01e+01\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -3.0e+05 & 10 & \cthree{1.33e+03}& 3.01e+05& 3.01e+05& 3.01e+05& \cone{0.00e+00}& \ctwo{1.25e+03}\cone{(+)}& 7.85e+03\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 2.27e+04& 4.22e+05& 6.36e+04& 2.31e+05& \cone{0.00e+00}& \ctwo{1.21e+04}\cone{(+)}& \cthree{1.58e+04}\cone{(+)}\\
CnnCaltech-3000-1000 & 5.9e+02 & 10 & 2.32e+02& 4.55e+02& 2.90e+02& 2.90e+02& \cone{0.00e+00}& \cthree{7.90e+01}\cone{(+)}& \ctwo{3.80e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 10 & 1.37e+03& \ctwo{2.98e+01}& 1.00e+04& \cthree{6.75e+01}& 2.99e+03& 1.07e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
randn-500-1000 & -2.0e+03 & 10 & 5.41e+02& 4.89e+02& 6.69e+02& 5.13e+02& \cone{0.00e+00}& \cthree{1.57e+02}\cone{(+)}& \ctwo{7.08e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -3.3e+03 & 20 & 1.72e+03& 4.44e+03& 4.45e+03& 4.45e+03& \ctwo{3.07e+01}& \cthree{1.07e+02}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+03 & 20 & 2.71e+02& 3.75e+02& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 2.09e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+03 & 20 & 1.59e+02& 1.00e+03& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 7.93e+01\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+03 & 20 & 9.94e+01& 7.47e+02& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{4.21e+01}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+03 & 20 & 1.21e+02& 5.19e+02& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 8.05e+01\cone{(+)}& \ctwo{1.83e-03}\cone{(+)}\\
MNIST-60000-784 & -3.3e+05 & 20 & \cthree{4.26e+03}& 3.32e+05& 3.32e+05& 3.32e+05& \cone{0.00e+00}& \ctwo{3.09e+03}\cone{(+)}& 3.80e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{2.66e+04}& 4.51e+05& 7.96e+04& 3.60e+05& \cone{0.00e+00}& \ctwo{1.60e+04}\cone{(+)}& 3.52e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 1.4e+03 & 20 & 2.46e+02& 1.16e+03& 2.65e+03& 3.90e+02& \cone{0.00e+00}& \cthree{3.29e+01}\cone{(+)}& \ctwo{4.37e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 20 & \ctwo{3.42e+02}& 1.24e+04& 1.35e+04& 7.90e+03& \cthree{1.94e+03}& \cone{0.00e+00}\cone{(+)}& 7.12e+03\cone{(+)}\\
randn-500-1000 & -3.9e+03 & 20 & 1.26e+03& 1.31e+03& 8.40e+02& 8.26e+02& \cone{0.00e+00}& \cthree{4.98e+02}\cone{(+)}& \ctwo{2.17e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -1.6e+03 & 100 & 4.99e+03& 2.58e+03& 7.31e+03& 5.24e+03& \ctwo{3.09e+01}& \cone{0.00e+00}\cone{(+)}& \cthree{3.58e+01}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 100 & 1.08e+03& 1.13e+04& \cthree{4.45e+00}& \cthree{4.45e+00}& \cone{0.00e+00}& 9.69e+02\cone{(+)}& \ctwo{4.80e-03}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 100 & 8.15e+02& 2.28e+04& \cthree{9.26e-01}& \cthree{9.26e-01}& \cone{0.00e+00}& 6.68e+02\cone{(+)}& \ctwo{1.41e-03}\cone{(+)}\\
sector-6412-1000 & 9.9e+03 & 100 & 6.25e+01& 2.17e+04& 7.45e+01& 7.45e+01& \cone{0.00e+00}& \cthree{8.27e+00}\cone{(+)}& \ctwo{2.97e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 100 & 1.08e+03& 1.15e+04& \cthree{6.72e-01}& \cthree{6.72e-01}& \cone{0.00e+00}& 9.06e+02\cone{(+)}& \ctwo{4.94e-04}\cone{(+)}\\
MNIST-60000-784 & -3.5e+05 & 100 & \cthree{4.43e+04}& 8.22e+04& 1.68e+05& 1.69e+05& \cone{0.00e+00}& \ctwo{3.81e+04}\cone{(+)}& 7.46e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & \cthree{5.71e+04}& 4.81e+05& 1.23e+05& 3.23e+05& \cone{0.00e+00}& \ctwo{1.81e+04}\cone{(+)}& 8.55e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 7.8e+03 & 100 & 9.39e+02& 2.52e+04& 1.76e+03& 9.93e+02& \cone{0.00e+00}& \cthree{6.75e+01}\cone{(+)}& \ctwo{1.29e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.2e+05 & 100 & \ctwo{2.97e+02}& 8.07e+04& 3.72e+04& 5.66e+04& \cthree{2.28e+03}& \cone{0.00e+00}\cone{(+)}& 2.58e+04\cone{(+)}\\
randn-500-1000 & -1.8e+04 & 100 & 3.80e+03& 2.57e+04& 2.75e+03& 2.75e+03& \cone{0.00e+00}& \cthree{1.64e+03}\cone{(+)}& \ctwo{1.20e+01}\cone{(+)}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=60} \\ \hline
w1a-2477-300 & -3.0e+03 & 10 & 9.08e+02& 3.49e+03& 3.58e+03& 3.58e+03& \cone{0.00e+00}& \cthree{4.10e+01}\cone{(+)}& \ctwo{1.54e+01}\cone{(+)}\\
TDT2-500-1000 & 1.0e+03 & 10 & 3.23e+01& 2.86e+01& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 2.90e+01\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+03 & 10 & 6.88e+01& 1.03e+02& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.76e+01\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 9.7e+02 & 10 & 1.55e+01& 1.53e+02& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{3.21e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+03 & 10 & 4.77e+01& 8.87e+01& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 1.01e+01\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -3.0e+05 & 10 & \cthree{1.18e+03}& 3.01e+05& 3.01e+05& 3.01e+05& \cone{0.00e+00}& \ctwo{1.09e+03}\cone{(+)}& 7.17e+03\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 10 & 1.28e+04& 3.01e+05& 5.40e+04& 3.00e+05& \cone{0.00e+00}& \ctwo{2.18e+03}\cone{(+)}& \cthree{6.93e+03}\cone{(+)}\\
CnnCaltech-3000-1000 & 6.0e+02 & 10 & 2.28e+02& 3.15e+02& 2.86e+02& 2.86e+02& \ctwo{1.57e+01}& \cthree{6.79e+01}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 10 & 1.57e+03& \cthree{4.72e+01}& 1.02e+04& \ctwo{3.31e+01}& 3.11e+03& 1.28e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
randn-500-1000 & -2.0e+03 & 10 & 5.41e+02& 3.71e+02& 6.69e+02& 5.13e+02& \cone{0.00e+00}& \cthree{1.58e+02}\cone{(+)}& \ctwo{7.08e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -3.3e+03 & 20 & 1.72e+03& 4.44e+03& 4.45e+03& 4.45e+03& \ctwo{3.85e+01}& \cthree{1.07e+02}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+03 & 20 & 2.71e+02& 7.21e+01& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 2.09e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+03 & 20 & 1.59e+02& 4.86e+02& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 7.93e+01\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+03 & 20 & 9.93e+01& 4.84e+02& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{4.20e+01}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+03 & 20 & 1.20e+02& 2.25e+02& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 8.05e+01\cone{(+)}& \ctwo{1.70e-03}\cone{(+)}\\
MNIST-60000-784 & -3.3e+05 & 20 & \cthree{4.84e+03}& 3.32e+05& 3.32e+05& 3.32e+05& \cone{0.00e+00}& \ctwo{3.65e+03}\cone{(+)}& 3.83e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & \cthree{2.49e+04}& 3.82e+05& 7.81e+04& 3.36e+05& \cone{0.00e+00}& \ctwo{1.44e+04}\cone{(+)}& 3.52e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 1.4e+03 & 20 & 2.46e+02& 7.54e+02& 2.65e+03& 3.90e+02& \cone{0.00e+00}& \cthree{3.32e+01}\cone{(+)}& \ctwo{4.63e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.3e+05 & 20 & 1.18e+03& \cone{0.00e+00}& 1.43e+04& \cthree{5.38e+02}& 2.66e+03& 8.43e+02\cone{(+)}& \ctwo{3.75e+02}\cone{(+)}\\
randn-500-1000 & -3.9e+03 & 20 & 1.26e+03& 9.29e+02& 8.40e+02& 8.26e+02& \cone{0.00e+00}& \cthree{5.05e+02}\cone{(+)}& \ctwo{2.17e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & -1.6e+03 & 100 & 4.99e+03& 2.04e+03& 7.31e+03& 5.24e+03& \ctwo{1.13e+01}& \cone{0.00e+00}\cone{(+)}& \cthree{2.47e+01}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 100 & 1.08e+03& 3.86e+03& \cthree{4.45e+00}& \cthree{4.45e+00}& \cone{0.00e+00}& 9.69e+02\cone{(+)}& \ctwo{4.80e-03}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 100 & 8.15e+02& 1.19e+04& \cthree{9.26e-01}& \cthree{9.26e-01}& \cone{0.00e+00}& 6.68e+02\cone{(+)}& \ctwo{1.43e-03}\cone{(+)}\\
sector-6412-1000 & 9.9e+03 & 100 & 6.25e+01& 1.09e+04& 7.45e+01& 7.45e+01& \cone{0.00e+00}& \cthree{8.27e+00}\cone{(+)}& \ctwo{2.97e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 100 & 1.08e+03& 5.83e+03& \cthree{6.72e-01}& \cthree{6.72e-01}& \cone{0.00e+00}& 9.06e+02\cone{(+)}& \ctwo{4.94e-04}\cone{(+)}\\
MNIST-60000-784 & -3.6e+05 & 100 & \cthree{5.10e+04}& 6.43e+04& 1.75e+05& 1.62e+05& \cone{0.00e+00}& \ctwo{4.48e+04}\cone{(+)}& 7.91e+04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & \cthree{6.56e+04}& 4.70e+05& 1.32e+05& 3.29e+05& \cone{0.00e+00}& \ctwo{2.66e+04}\cone{(+)}& 9.34e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 7.8e+03 & 100 & 9.39e+02& 1.39e+04& 1.76e+03& 9.93e+02& \cone{0.00e+00}& \cthree{6.77e+01}\cone{(+)}& \ctwo{1.42e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.2e+05 & 100 & \ctwo{2.86e+02}& 6.01e+04& 3.72e+04& 5.64e+04& \cthree{2.23e+03}& \cone{0.00e+00}\cone{(+)}& 2.61e+04\cone{(+)}\\
randn-500-1000 & -1.8e+04 & 100 & 3.78e+03& 1.49e+04& 2.74e+03& 2.74e+03& \ctwo{7.43e+00}& \cthree{1.62e+03}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F_{\text{min}})$ of $L_1$ norm-based SPCA for all the compared methods with $\lambda=100$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$. }
\label{tab:L1PCA:2}
\end{table*}


\begin{table*}[!h]
\centering
\scalebox{0.52}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n} & \multirow{2}*{$F_{\text{min}}$}& \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{RSubGrad}  & \multirow{2}*{ADMM} & \multirow{2}*{ManPG} &\multirow{2}*{ODBC-OR} & LADMM   & ManPG \\
 &   &    &&   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
  \hline
   \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=10} \\ \hline
w1a-2477-300 & 7.0e+03 & 10 & \ctwo{3.03e+02}& 2.81e+03& \cthree{2.59e+03}& \cthree{2.59e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 10 & 1.24e+03& 1.39e+04& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 5.21e+02\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 10 & 8.97e+02& 7.55e+04& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.20e+02\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 1.0e+04 & 10 & 2.88e+01& 7.59e+04& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{1.29e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 10 & 3.88e+02& 3.77e+04& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 3.87e+02\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 10 & \ctwo{1.69e+02}& 2.27e+05& 2.27e+05& 2.27e+05& 1.71e+04& \cone{0.00e+00}\cone{(+)}& \cthree{9.07e+03}\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & \cthree{2.26e+04}& 5.38e+05& 6.58e+04& 4.70e+05& \cone{0.00e+00}& \ctwo{1.61e+04}\cone{(+)}& 4.39e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 9.6e+03 & 10 & \cthree{1.06e+02}& 7.01e+04& 1.20e+03& 2.90e+02& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \ctwo{3.80e+00}\cone{(+)}\\
Cifar-1000-1000 & -9.2e+04 & 10 & \cthree{1.89e+03}& 1.14e+05& \cone{0.00e+00}& 1.00e+05& 9.99e+04& \ctwo{1.80e+03}\cone{(+)}& 9.99e+04\cone{(+)}\\
randn-500-1000 & 7.0e+03 & 10 & 3.66e+02& 8.30e+04& 3.14e+04& 5.11e+02& \cone{0.00e+00}& \cthree{8.04e+00}\cone{(+)}& \ctwo{4.69e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{5.30e+02}& 5.72e+03& \cthree{3.90e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.40e+03& 7.01e+04& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 9.85e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 1.45e+03& 2.56e+05& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 1.45e+03\cone{(+)}& \ctwo{1.30e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 6.06e+02& 2.06e+05& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{1.37e+00}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.65e+03& 8.70e+04& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 7.18e+02\cone{(+)}& \ctwo{1.83e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 20 & \ctwo{3.85e+03}& 2.41e+05& 2.41e+05& 2.41e+05& \cthree{2.71e+04}& \cone{0.00e+00}\cone{(+)}& 3.00e+04\cone{(+)}\\
Gisette-3000-1000 & -9.9e+05 & 20 & \cthree{1.41e+04}& 6.98e+05& 1.15e+05& 3.45e+05& \cone{0.00e+00}& \ctwo{2.26e+03}\cone{(+)}& 9.40e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 2.01e+02& 2.05e+05& 8.77e+02& 3.90e+02& \cone{0.00e+00}& \ctwo{8.32e-01}\cone{(+)}& \cthree{4.37e+00}\cone{(+)}\\
Cifar-1000-1000 & -8.1e+04 & 20 & \ctwo{1.52e+02}& 2.22e+05& 1.04e+05& 9.83e+04& \cthree{9.72e+04}& \cone{0.00e+00}\cone{(+)}& \cthree{9.72e+04}\cone{(+)}\\
randn-500-1000 & 1.4e+04 & 20 & 4.49e+02& 1.98e+05& 3.61e+04& 8.21e+02& \cone{0.00e+00}& \ctwo{1.10e+01}\cone{(+)}& \cthree{1.69e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 8.8e+04 & 100 & \cthree{3.43e+03}& 2.56e+05& 8.92e+03& 6.89e+03& \ctwo{3.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 6.91e+03& 1.10e+06& \cthree{4.45e+00}& \cthree{4.45e+00}& \ctwo{4.80e-03}& 5.95e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
20News-8000-1000 & 1.0e+05 & 100 & 3.61e+03& 1.88e+06& \cthree{9.25e-01}& \cthree{9.25e-01}& \ctwo{1.01e-03}& 3.53e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
sector-6412-1000 & 1.0e+05 & 100 & 4.16e+03& 1.79e+06& \cthree{7.42e+01}& \cthree{7.42e+01}& \ctwo{8.04e-01}& 3.46e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
E2006-2000-1000 & 1.0e+05 & 100 & 4.18e+03& 1.19e+06& \cthree{6.71e-01}& \cthree{6.71e-01}& \ctwo{1.50e-03}& 4.18e+03\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
MNIST-60000-784 & -1.7e+05 & 100 & 5.23e+04& 1.05e+06& 1.02e+05& 2.72e+05& \cthree{1.05e+04}& \cone{0.00e+00}\cone{(+)}& \ctwo{5.25e+03}\cone{(+)}\\
Gisette-3000-1000 & -9.9e+05 & 100 & \cthree{5.95e+04}& 2.41e+06& 4.30e+05& 5.84e+05& \ctwo{3.49e+04}& \cone{0.00e+00}\cone{(+)}& 3.06e+05\cone{(+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 7.61e+02& 1.90e+06& 1.40e+03& 9.92e+02& \cthree{3.59e+00}& \cone{0.00e+00}\cone{(+)}& \ctwo{4.00e-02}\cone{(+)}\\
Cifar-1000-1000 & -2.5e+03 & 100 & \ctwo{1.28e+03}& 1.94e+06& 8.69e+04& 8.69e+04& \cthree{8.31e+04}& \cone{0.00e+00}\cone{(+)}& \cthree{8.31e+04}\cone{(+)}\\
randn-500-1000 & 7.2e+04 & 100 & 2.91e+03& 1.90e+06& 2.76e+05& 2.74e+03& \ctwo{7.14e+00}& \cthree{6.87e+02}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=30} \\ \hline
w1a-2477-300 & 7.0e+03 & 10 & \ctwo{3.03e+02}& 2.64e+03& \cthree{2.59e+03}& \cthree{2.59e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 10 & 1.24e+03& 5.07e+03& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 5.20e+02\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 10 & 8.96e+02& 3.10e+04& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.20e+02\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 1.0e+04 & 10 & 2.88e+01& 2.42e+04& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{1.29e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 10 & 3.87e+02& 1.26e+04& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 3.87e+02\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 10 & \ctwo{1.72e+02}& 2.27e+05& 2.27e+05& 2.27e+05& 1.68e+04& \cone{0.00e+00}\cone{(+)}& \cthree{8.98e+03}\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & \cthree{2.41e+04}& 4.51e+05& 6.72e+04& 2.94e+05& \cone{0.00e+00}& \ctwo{1.76e+04}\cone{(+)}& 3.24e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 9.6e+03 & 10 & \cthree{1.06e+02}& 2.33e+04& 1.19e+03& 2.90e+02& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \ctwo{3.80e+00}\cone{(+)}\\
Cifar-1000-1000 & -9.2e+04 & 10 & \cthree{1.89e+03}& 2.35e+04& \cone{0.00e+00}& 1.00e+05& 9.99e+04& \ctwo{1.80e+03}\cone{(+)}& 9.99e+04\cone{(+)}\\
randn-500-1000 & 7.0e+03 & 10 & 3.66e+02& 2.66e+04& 3.10e+04& 5.11e+02& \cone{0.00e+00}& \cthree{5.13e+00}\cone{(+)}& \ctwo{4.69e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{5.30e+02}& 4.27e+03& \cthree{3.90e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.40e+03& 2.96e+04& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 9.84e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 1.45e+03& 9.38e+04& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 1.45e+03\cone{(+)}& \ctwo{1.30e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 6.05e+02& 6.35e+04& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{1.37e+00}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.65e+03& 3.21e+04& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 7.18e+02\cone{(+)}& \ctwo{1.83e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 20 & \ctwo{3.90e+03}& 2.41e+05& 2.41e+05& 2.41e+05& \cthree{2.42e+04}& \cone{0.00e+00}\cone{(+)}& 2.78e+04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 20 & \cthree{1.91e+04}& 5.27e+05& 1.20e+05& 3.38e+05& \cone{0.00e+00}& \ctwo{7.17e+03}\cone{(+)}& 1.00e+05\cone{(+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 2.02e+02& 6.88e+04& 8.74e+02& 3.90e+02& \cone{0.00e+00}& \ctwo{1.09e+00}\cone{(+)}& \cthree{4.63e+00}\cone{(+)}\\
Cifar-1000-1000 & -8.1e+04 & 20 & \ctwo{1.56e+02}& \cthree{9.10e+04}& 1.04e+05& 9.83e+04& 9.72e+04& \cone{0.00e+00}\cone{(+)}& 9.72e+04\cone{(+)}\\
randn-500-1000 & 1.4e+04 & 20 & 4.49e+02& 8.47e+04& 3.54e+04& 8.21e+02& \cone{0.00e+00}& \ctwo{1.10e+01}\cone{(+)}& \cthree{1.69e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 8.8e+04 & 100 & \ctwo{3.43e+03}& 1.06e+05& 8.92e+03& \cthree{6.89e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 6.78e+03& 7.04e+05& \cthree{4.45e+00}& \cthree{4.45e+00}& \cone{0.00e+00}& 5.55e+03\cone{(+)}& \ctwo{2.74e-03}\cone{(+)}\\
20News-8000-1000 & 1.0e+05 & 100 & 3.61e+03& 1.38e+06& \cthree{9.26e-01}& \cthree{9.26e-01}& \cone{0.00e+00}& 3.53e+03\cone{(+)}& \ctwo{1.41e-03}\cone{(+)}\\
sector-6412-1000 & 1.0e+05 & 100 & 4.10e+03& 1.28e+06& \cthree{7.45e+01}& \cthree{7.45e+01}& \cone{0.00e+00}& 3.40e+03\cone{(+)}& \ctwo{3.12e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+05 & 100 & 4.13e+03& 7.75e+05& \cthree{6.72e-01}& \cthree{6.72e-01}& \cone{0.00e+00}& 4.13e+03\cone{(+)}& \ctwo{4.60e-04}\cone{(+)}\\
MNIST-60000-784 & -1.7e+05 & 100 & 5.23e+04& 6.81e+05& 1.02e+05& 2.72e+05& \ctwo{3.46e+03}& \cone{0.00e+00}\cone{(+)}& \cthree{5.25e+03}\cone{(+)}\\
Gisette-3000-1000 & -9.9e+05 & 100 & \cthree{5.98e+04}& 1.91e+06& 4.30e+05& 5.83e+05& \ctwo{2.23e+04}& \cone{0.00e+00}\cone{(+)}& 3.06e+05\cone{(+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 7.62e+02& 1.31e+06& 1.39e+03& 9.93e+02& \cone{0.00e+00}& \cthree{1.41e+00}\cone{(+)}& \ctwo{1.23e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.9e+03 & 100 & \ctwo{6.77e+02}& 1.48e+06& 8.63e+04& 8.63e+04& \cthree{8.25e+04}& \cone{0.00e+00}\cone{(+)}& \cthree{8.25e+04}\cone{(+)}\\
randn-500-1000 & 7.2e+04 & 100 & 2.91e+03& 1.35e+06& 2.22e+05& 2.74e+03& \cone{0.00e+00}& \cthree{6.90e+02}\cone{(+)}& \ctwo{3.33e+00}\cone{(+)}\\
 \hline \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=60} \\ \hline
w1a-2477-300 & 7.0e+03 & 10 & \ctwo{3.03e+02}& \cthree{2.58e+03}& 2.59e+03& 2.59e+03& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+04 & 10 & 1.24e+03& 1.98e+03& \cthree{3.40e+00}& \cthree{3.40e+00}& \cone{0.00e+00}& 5.19e+02\cone{(+)}& \ctwo{3.09e-02}\cone{(+)}\\
20News-8000-1000 & 1.0e+04 & 10 & 8.94e+02& 1.32e+04& \cthree{1.49e+00}& \cthree{1.49e+00}& \cone{0.00e+00}& 3.19e+02\cone{(+)}& \ctwo{3.07e-02}\cone{(+)}\\
sector-6412-1000 & 1.0e+04 & 10 & 2.88e+01& 1.18e+04& 3.00e+01& 3.00e+01& \cone{0.00e+00}& \ctwo{1.29e-01}\cone{(+)}& \cthree{3.68e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+04 & 10 & 3.87e+02& 5.62e+03& \cthree{6.18e-01}& \cthree{6.18e-01}& \cone{0.00e+00}& 3.87e+02\cone{(+)}& \ctwo{1.59e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 10 & \ctwo{1.71e+02}& 2.27e+05& 2.27e+05& 2.27e+05& 1.16e+04& \cone{0.00e+00}\cone{(+)}& \cthree{8.33e+03}\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & \cthree{2.62e+04}& 3.30e+05& 6.93e+04& 2.65e+05& \cone{0.00e+00}& \ctwo{1.97e+04}\cone{(+)}& 4.01e+04\cone{(+)}\\
CnnCaltech-3000-1000 & 9.6e+03 & 10 & \cthree{1.06e+02}& 1.29e+04& 1.19e+03& 2.90e+02& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \ctwo{3.80e+00}\cone{(+)}\\
Cifar-1000-1000 & -9.2e+04 & 10 & \cthree{1.89e+03}& 1.30e+04& \cone{0.00e+00}& 1.00e+05& 9.99e+04& \ctwo{1.80e+03}\cone{(+)}& 9.99e+04\cone{(+)}\\
randn-500-1000 & 7.0e+03 & 10 & 3.66e+02& 1.44e+04& 3.09e+04& 5.11e+02& \cone{0.00e+00}& \cthree{8.04e+00}\cone{(+)}& \ctwo{4.69e+00}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 1.5e+04 & 20 & \ctwo{5.30e+02}& 4.03e+03& \cthree{3.90e+03}& \cthree{3.90e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 2.0e+04 & 20 & 1.40e+03& 1.19e+04& \cthree{3.75e+00}& \cthree{3.75e+00}& \cone{0.00e+00}& 9.82e+02\cone{(+)}& \ctwo{1.10e-02}\cone{(+)}\\
20News-8000-1000 & 2.0e+04 & 20 & 1.45e+03& 5.00e+04& \cthree{1.66e+00}& \cthree{1.66e+00}& \cone{0.00e+00}& 1.45e+03\cone{(+)}& \ctwo{1.08e-02}\cone{(+)}\\
sector-6412-1000 & 2.0e+04 & 20 & 6.05e+02& 3.08e+04& 4.27e+01& 4.27e+01& \cone{0.00e+00}& \cthree{1.37e+00}\cone{(+)}& \ctwo{1.19e+00}\cone{(+)}\\
E2006-2000-1000 & 2.0e+04 & 20 & 1.65e+03& 1.64e+04& \cthree{6.38e-01}& \cthree{6.38e-01}& \cone{0.00e+00}& 7.18e+02\cone{(+)}& \ctwo{1.70e-03}\cone{(+)}\\
MNIST-60000-784 & -2.2e+05 & 20 & \ctwo{3.92e+03}& 2.41e+05& 2.41e+05& 2.41e+05& \cthree{1.17e+04}& \cone{0.00e+00}\cone{(+)}& 2.85e+04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 20 & \cthree{2.03e+04}& 4.31e+05& 1.22e+05& 4.61e+05& \cone{0.00e+00}& \ctwo{7.84e+03}\cone{(+)}& 1.07e+05\cone{(+)}\\
CnnCaltech-3000-1000 & 1.9e+04 & 20 & 2.02e+02& 3.98e+04& 8.74e+02& 3.90e+02& \cone{0.00e+00}& \ctwo{1.09e+00}\cone{(+)}& \cthree{4.63e+00}\cone{(+)}\\
Cifar-1000-1000 & -8.1e+04 & 20 & \ctwo{1.55e+02}& \cthree{4.42e+04}& 1.04e+05& 9.83e+04& 9.72e+04& \cone{0.00e+00}\cone{(+)}& 9.72e+04\cone{(+)}\\
randn-500-1000 & 1.4e+04 & 20 & 4.49e+02& 4.65e+04& 3.54e+04& 8.21e+02& \cone{0.00e+00}& \ctwo{1.10e+01}\cone{(+)}& \cthree{1.69e+01}\cone{(+)}\\
 \hline \hline
w1a-2477-300 & 8.8e+04 & 100 & \ctwo{3.43e+03}& 4.16e+04& 8.92e+03& \cthree{6.89e+03}& \cone{0.00e+00}& \cone{0.00e+00}\cone{(+)}& \cone{0.00e+00}\cone{(+)}\\
TDT2-500-1000 & 1.0e+05 & 100 & 6.78e+03& 4.62e+05& \cthree{4.45e+00}& \cthree{4.45e+00}& \cone{0.00e+00}& 5.20e+03\cone{(+)}& \ctwo{4.80e-03}\cone{(+)}\\
20News-8000-1000 & 1.0e+05 & 100 & 3.61e+03& 9.50e+05& \cthree{9.26e-01}& \cthree{9.26e-01}& \cone{0.00e+00}& 3.53e+03\cone{(+)}& \ctwo{1.43e-03}\cone{(+)}\\
sector-6412-1000 & 1.0e+05 & 100 & 4.10e+03& 8.69e+05& \cthree{7.45e+01}& \cthree{7.45e+01}& \cone{0.00e+00}& 3.40e+03\cone{(+)}& \ctwo{2.97e-01}\cone{(+)}\\
E2006-2000-1000 & 1.0e+05 & 100 & 4.13e+03& 4.91e+05& \cthree{6.72e-01}& \cthree{6.72e-01}& \cone{0.00e+00}& 4.13e+03\cone{(+)}& \ctwo{4.94e-04}\cone{(+)}\\
MNIST-60000-784 & -1.8e+05 & 100 & 5.53e+04& 4.36e+05& 1.06e+05& 2.75e+05& \cone{0.00e+00}& \ctwo{2.94e+03}\cone{(+)}& \cthree{8.25e+03}\cone{(+)}\\
Gisette-3000-1000 & -9.9e+05 & 100 & \cthree{5.98e+04}& 1.45e+06& 4.30e+05& 6.84e+05& \ctwo{1.43e+04}& \cone{0.00e+00}\cone{(+)}& 3.07e+05\cone{(+)}\\
CnnCaltech-3000-1000 & 9.8e+04 & 100 & 7.63e+02& 9.73e+05& 1.39e+03& 9.93e+02& \cone{0.00e+00}& \ctwo{1.58e+00}\cone{(+)}& \cthree{1.62e+00}\cone{(+)}\\
Cifar-1000-1000 & -1.9e+03 & 100 & \ctwo{6.75e+02}& 1.16e+06& 8.63e+04& 8.63e+04& \cthree{8.25e+04}& \cone{0.00e+00}\cone{(+)}& \cthree{8.25e+04}\cone{(+)}\\
randn-500-1000 & 7.2e+04 & 100 & 2.92e+03& 9.34e+05& 2.22e+05& 2.75e+03& \cone{0.00e+00}& \cthree{6.92e+02}\cone{(+)}& \ctwo{5.80e+00}\cone{(+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values $(F(\X)-F_{\text{min}})$ of $L_1$ norm-based SPCA for all the compared methods with $\lambda=1000$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively. If the objective values of `LADMM+ODBC-R' (or `PADM+ODBC-R') are significantly smaller than that of `LADMM' (or `PADM'), they will be marked with $\cone{(+)}$.}
\label{tab:L1PCA:3}
\end{table*}





==> L1PCA/NLEVP.tex <==


\begin{table*}[!h]
\centering
\scalebox{0.4}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline \multirow{2}*{data-m-n}  & \multirow{2}*{$F_{\text{min}}$}  & \multirow{2}*{r} & \multirow{2}*{FOForth-GR}  &  \multirow{2}*{FOForth-P}  & \multirow{2}*{FOForth-QR} & \multirow{2}*{OptM-QR} &\multirow{2}*{OptM-Cayley} &  \multirow{2}*{OBCD-SV}    &\multirow{2}*{OBCD-OR} \\
   &  &   &    &   &  &    &   &     &    \\
   \hline\hline
   \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=20} \\ \hline
w1a-2477-300 &-1.2e+02& 10 & 4.672e+01, 8e+02& 7.805e-06, 1e-02& 4.860e-06, 1e-02& \cthree{1.230e-08}, 6e-04& 3.352e-08, 8e-04& \ctwo{2.842e-14}, 6e-13& \cone{0.000e+00}, 1e-12\\
TDT2-500-1000 &-3.1e+02& 10 & 1.473e+05, 6e+05& 1.234e-04, 7e-02& 7.167e-05, 8e-02& \cthree{1.266e-07}, 3e-03& 3.710e-07, 4e-03& \cone{0.000e+00}, 4e-06& \ctwo{1.445e-08}, 1e-03\\
20News-8000-1000 &-2.6e+02& 10 & 1.865e+04, 5e+05& 1.930e+05, 9e+04& 5.043e-03, 4e-01& \cthree{5.735e-06}, 3e-02& 9.833e-05, 3e-01& \cone{0.000e+00}, 5e-08& \ctwo{2.945e-06}, 2e-02\\
sector-6412-1000 &-3.2e+02& 10 & 1.619e+07, 3e+08& 2.950e+08, 1e+01& 7.767e-01, 9e+00& \cone{0.000e+00}, 1e-01& \cthree{1.273e-01}, 3e+00& \ctwo{1.037e-02}, 2e+01& 6.192e-01, 2e+01\\
E2006-2000-1000 &-2.9e+02& 10 & 5.948e+03, 2e+05& 8.158e+05, 3e+00& 7.679e-05, 8e-02& 1.373e-07, 3e-03& \cthree{1.153e-08}, 2e-03& \cone{0.000e+00}, 1e-08& \ctwo{2.274e-13}, 1e-08\\
MNIST-60000-784 &-1.9e+02& 10 & 1.972e+05, 3e+04& 3.006e+05, 3e-01& 1.902e-04, 2e-01& \cthree{2.043e-06}, 8e-03& 5.525e-06, 1e-02& \cone{0.000e+00}, 2e-05& \ctwo{3.558e-09}, 8e-04\\
Gisette-3000-1000 &-1.3e+02& 10 & 1.007e+06, 2e+05& 2.342e-01, 5e+00& \cthree{5.245e-02}, 1e+00& \ctwo{7.213e-04}, 1e-01& \cone{0.000e+00}, 2e-01& 1.906e-01, 4e+00& 2.482e-01, 3e+00\\
CnnCaltech-3000-1000 &-2.7e+02& 10 & 7.784e-02, 3e+01& 4.655e+03, 2e+02& 3.776e-09, 1e-03& \ctwo{8.151e-11}, 1e-04& \cthree{7.567e-10}, 2e-04& \cone{0.000e+00}, 1e-12& \cone{0.000e+00}, 2e-12\\
Cifar-1000-1000 &-2.9e+02& 10 & 1.318e+05, 2e+04& 3.550e+04, 1e+05& 1.204e-05, 4e-02& 1.052e-06, 8e-03& \cthree{8.839e-07}, 7e-03& \cone{0.000e+00}, 1e-05& \ctwo{4.027e-08}, 2e-03\\
randn-500-1000 &-2.2e+02& 10 & 4.624e+03, 3e+03& 1.394e+04, 6e+01& 5.621e-06, 2e-02& 2.911e-08, 4e-03& \cthree{1.435e-08}, 2e-03& \cone{0.000e+00}, 4e-08& \ctwo{3.278e-09}, 5e-04\\
 \hline
w1a-2477-300 &-2.3e+02& 20 & 3.037e+03, 8e+02& 7.394e+03, 1e+02& 3.756e-06, 1e-02& \cthree{9.790e-08}, 1e-03& 1.562e-07, 1e-03& \ctwo{1.137e-13}, 1e-12& \cone{0.000e+00}, 2e-12\\
TDT2-500-1000 &-6.2e+02& 20 & 4.235e+04, 4e+05& 2.786e-01, 3e+01& 4.600e-04, 1e-01& 2.082e-06, 4e-02& \cthree{3.859e-07}, 2e-02& \cone{0.000e+00}, 7e-06& \ctwo{1.369e-07}, 4e-03\\
20News-8000-1000 &-4.9e+02& 20 & 7.679e+05, 3e+06& 7.619e+05, 3e+00& 7.014e-01, 4e+00& \cthree{3.087e-02}, 1e+00& 3.848e-02, 8e-01& \cone{0.000e+00}, 2e-07& \ctwo{3.796e-03}, 3e-01\\
sector-6412-1000 &-6.3e+02& 20 & 3.720e+06, 2e+08& 2.950e+08, 1e+02& 6.795e+02, 2e+02& \cone{0.000e+00}, 6e+00& 2.004e+01, 4e+03& \cthree{1.359e+00}, 9e+01& \ctwo{1.083e+00}, 1e+02\\
E2006-2000-1000 &-5.7e+02& 20 & 1.408e+03, 4e+04& 3.125e+06, 5e+00& 3.056e-03, 4e-01& 3.673e-06, 4e-02& \cthree{4.979e-07}, 4e-03& \cone{0.000e+00}, 3e-08& \ctwo{1.758e-10}, 9e-05\\
MNIST-60000-784 &-3.9e+02& 20 & 1.970e+05, 3e+04& 3.543e+05, 6e+01& 5.824e-03, 5e-01& 2.471e-05, 2e-01& \cthree{1.872e-05}, 3e-02& \cone{0.000e+00}, 2e-03& \ctwo{1.288e-05}, 4e-02\\
Gisette-3000-1000 &-2.6e+02& 20 & 9.982e+05, 3e+05& 1.122e+06, 2e+00& \cthree{2.739e-01}, 2e+00& \ctwo{1.707e-02}, 7e+00& \cone{0.000e+00}, 5e+00& 2.554e+01, 4e+01& 2.857e+01, 4e+01\\
CnnCaltech-3000-1000 &-5.5e+02& 20 & 6.219e+01, 8e+02& 5.859e+03, 3e+02& 6.235e-09, 1e-03& 6.782e-09, 8e-04& \cthree{5.834e-09}, 1e-03& \cone{0.000e+00}, 2e-12& \ctwo{1.137e-13}, 4e-08\\
Cifar-1000-1000 &-5.7e+02& 20 & 4.175e+04, 1e+05& 5.423e+04, 1e+05& 1.549e-03, 3e-01& \ctwo{2.377e-06}, 1e-02& \cthree{6.245e-05}, 2e-01& \cone{0.000e+00}, 9e-05& 1.359e-04, 1e-01\\
randn-500-1000 &-4.5e+02& 20 & 1.245e+04, 4e+03& 2.680e+04, 9e+01& 2.269e-05, 3e-02& \cone{0.000e+00}, 4e-04& \ctwo{2.176e-07}, 1e-02& \cthree{1.115e-05}, 3e-02& 2.771e-05, 4e-02\\
 \hline
w1a-2477-300 &-5.6e+02& 50 & 2.185e+03, 3e+03& 1.023e+04, 2e+02& 7.007e-06, 2e-02& 5.620e-07, 2e-03& \cthree{9.584e-08}, 2e-03& \cone{0.000e+00}, 3e-12& \ctwo{8.617e-11}, 4e-05\\
TDT2-500-1000 &-1.5e+03& 50 & 4.330e+04, 2e+05& 6.497e+04, 4e+04& 1.044e-02, 5e-01& \ctwo{1.288e-03}, 2e+00& 8.943e-03, 8e-01& \cone{0.000e+00}, 3e-05& \cthree{2.864e-03}, 4e-01\\
20News-8000-1000 &-1.1e+03& 50 & 8.254e+04, 5e+05& 1.636e+06, 3e+04& 1.283e+01, 2e+01& \cthree{7.286e+00}, 1e+01& 2.031e+01, 2e+02& \cone{0.000e+00}, 6e-02& \ctwo{3.759e+00}, 9e+00\\
sector-6412-1000 &-1.6e+03& 50 & 5.671e+08, 2e+09& 2.950e+08, 3e+02& 1.809e+03, 3e+02& \cthree{6.364e+01}, 6e+01& 5.643e+02, 2e+02& \ctwo{4.292e+01}, 2e+02& \cone{0.000e+00}, 3e+02\\
E2006-2000-1000 &-1.4e+03& 50 & 2.404e+05, 5e+05& 5.830e+06, 1e+05& 7.460e-03, 9e-01& \ctwo{3.085e-07}, 4e-03& \cthree{3.218e-07}, 6e-02& \cone{0.000e+00}, 1e-07& 9.558e-03, 7e-01\\
MNIST-60000-784 &-9.4e+02& 50 & 6.740e+03, 7e+04& 4.088e+05, 9e+01& \cthree{4.050e-02}, 9e-01& \cone{0.000e+00}, 3e-01& \ctwo{1.139e-04}, 8e-01& 3.629e+00, 2e+01& 8.501e+00, 3e+01\\
Gisette-3000-1000 &-6.4e+02& 50 & 1.009e+06, 1e+05& 1.160e+06, 9e+02& \cthree{2.267e-01}, 4e+00& \ctwo{2.025e-01}, 2e+01& \cone{0.000e+00}, 1e+00& 5.593e+02, 3e+02& 6.379e+02, 2e+02\\
CnnCaltech-3000-1000 &-1.4e+03& 50 & 4.604e+00, 2e+02& 6.053e+03, 4e+02& 1.462e-07, 6e-03& 4.699e-07, 2e-02& \cthree{1.589e-08}, 1e-03& \cone{0.000e+00}, 2e-07& \ctwo{9.126e-09}, 8e-04\\
Cifar-1000-1000 &-1.4e+03& 50 & 1.634e+05, 4e+05& 5.187e-03, 5e-01& \cthree{4.116e-03}, 5e-01& \cone{0.000e+00}, 5e-02& \ctwo{2.040e-05}, 3e-02& 1.346e+00, 1e+01& 2.016e+00, 1e+01\\
randn-500-1000 &-1.1e+03& 50 & 3.050e+04, 6e+03& 6.014e+04, 3e+02& \cthree{6.300e-05}, 5e-02& \cone{0.000e+00}, 3e-03& \ctwo{1.380e-07}, 3e-03& 2.857e+01, 5e+01& 3.763e+01, 5e+01\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=30} \\ \hline
w1a-2477-300 &-1.2e+02& 10 & 4.672e+01, 8e+02& 7.805e-06, 1e-02& 4.860e-06, 1e-02& \cthree{1.230e-08}, 6e-04& 3.352e-08, 8e-04& \cone{0.000e+00}, 6e-13& \ctwo{1.421e-14}, 1e-12\\
TDT2-500-1000 &-3.1e+02& 10 & 1.473e+05, 6e+05& 1.234e-04, 7e-02& 7.167e-05, 8e-02& \cthree{1.266e-07}, 3e-03& 3.710e-07, 4e-03& \cone{0.000e+00}, 4e-06& \ctwo{9.186e-10}, 3e-04\\
20News-8000-1000 &-2.6e+02& 10 & 1.865e+04, 5e+05& 1.930e+05, 9e+04& 5.043e-03, 4e-01& \cthree{5.735e-06}, 3e-02& 9.833e-05, 3e-01& \cone{0.000e+00}, 5e-08& \ctwo{1.019e-06}, 1e-02\\
sector-6412-1000 &-3.2e+02& 10 & 1.619e+07, 3e+08& 2.950e+08, 1e+01& 7.767e-01, 9e+00& \cone{0.000e+00}, 1e-01& \cthree{1.273e-01}, 3e+00& \ctwo{6.720e-03}, 2e+01& 5.410e-01, 1e+01\\
E2006-2000-1000 &-2.9e+02& 10 & 5.948e+03, 2e+05& 8.158e+05, 3e+00& 7.679e-05, 8e-02& 1.373e-07, 3e-03& \cthree{1.153e-08}, 2e-03& \cone{0.000e+00}, 1e-08& \ctwo{5.684e-14}, 1e-08\\
MNIST-60000-784 &-1.9e+02& 10 & 1.972e+05, 3e+04& 3.006e+05, 3e-01& 1.902e-04, 2e-01& \cthree{2.043e-06}, 8e-03& 5.525e-06, 1e-02& \cone{0.000e+00}, 2e-05& \ctwo{9.931e-11}, 1e-04\\
Gisette-3000-1000 &-1.3e+02& 10 & 1.007e+06, 2e+05& 2.342e-01, 5e+00& 5.245e-02, 1e+00& \ctwo{7.213e-04}, 1e-01& \cone{0.000e+00}, 2e-01& \cthree{1.259e-02}, 6e-01& 2.394e-02, 8e-01\\
CnnCaltech-3000-1000 &-2.7e+02& 10 & 7.784e-02, 3e+01& 4.655e+03, 2e+02& 3.776e-09, 1e-03& \cthree{8.151e-11}, 1e-04& 7.567e-10, 2e-04& \ctwo{5.684e-14}, 2e-12& \cone{0.000e+00}, 2e-12\\
Cifar-1000-1000 &-2.9e+02& 10 & 1.318e+05, 2e+04& 3.550e+04, 1e+05& 1.204e-05, 4e-02& 1.052e-06, 8e-03& \cthree{8.839e-07}, 7e-03& \cone{0.000e+00}, 1e-05& \ctwo{3.375e-10}, 2e-04\\
randn-500-1000 &-2.2e+02& 10 & 4.624e+03, 3e+03& 1.394e+04, 6e+01& 5.621e-06, 2e-02& 2.911e-08, 4e-03& \cthree{1.435e-08}, 2e-03& \cone{0.000e+00}, 7e-12& \ctwo{1.784e-10}, 1e-04\\
 \hline
w1a-2477-300 &-2.3e+02& 20 & 3.037e+03, 8e+02& 7.394e+03, 1e+02& 3.756e-06, 1e-02& \ctwo{9.790e-08}, 1e-03& \cthree{1.562e-07}, 1e-03& \cone{0.000e+00}, 1e-12& \cone{0.000e+00}, 2e-12\\
TDT2-500-1000 &-6.2e+02& 20 & 4.235e+04, 4e+05& 2.786e-01, 3e+01& 4.600e-04, 1e-01& 2.082e-06, 4e-02& \cthree{3.859e-07}, 2e-02& \cone{0.000e+00}, 7e-06& \ctwo{3.041e-08}, 2e-03\\
20News-8000-1000 &-4.9e+02& 20 & 7.679e+05, 3e+06& 7.619e+05, 3e+00& 7.014e-01, 4e+00& \cthree{3.087e-02}, 1e+00& 3.848e-02, 8e-01& \cone{0.000e+00}, 2e-07& \ctwo{6.536e-04}, 1e-01\\
sector-6412-1000 &-6.3e+02& 20 & 3.720e+06, 2e+08& 2.950e+08, 1e+02& 6.795e+02, 2e+02& \cone{0.000e+00}, 6e+00& 2.004e+01, 4e+03& \ctwo{9.142e-01}, 1e+02& \cthree{1.052e+00}, 1e+02\\
E2006-2000-1000 &-5.7e+02& 20 & 1.408e+03, 4e+04& 3.125e+06, 5e+00& 3.056e-03, 4e-01& 3.673e-06, 4e-02& \cthree{4.979e-07}, 4e-03& \cone{0.000e+00}, 3e-08& \ctwo{4.547e-13}, 1e-06\\
MNIST-60000-784 &-3.9e+02& 20 & 1.970e+05, 3e+04& 3.543e+05, 6e+01& 5.824e-03, 5e-01& 2.475e-05, 2e-01& \cthree{1.876e-05}, 3e-02& \cone{0.000e+00}, 4e-05& \ctwo{9.396e-07}, 1e-02\\
Gisette-3000-1000 &-2.6e+02& 20 & 9.982e+05, 3e+05& 1.122e+06, 2e+00& \cthree{2.739e-01}, 2e+00& \ctwo{1.707e-02}, 7e+00& \cone{0.000e+00}, 5e+00& 8.354e+00, 3e+01& 1.010e+01, 2e+01\\
CnnCaltech-3000-1000 &-5.5e+02& 20 & 6.219e+01, 8e+02& 5.859e+03, 3e+02& 6.235e-09, 1e-03& 6.782e-09, 8e-04& \cthree{5.834e-09}, 1e-03& \ctwo{1.137e-13}, 2e-12& \cone{0.000e+00}, 5e-10\\
Cifar-1000-1000 &-5.7e+02& 20 & 4.175e+04, 1e+05& 5.423e+04, 1e+05& 1.549e-03, 3e-01& \ctwo{2.377e-06}, 1e-02& 6.245e-05, 2e-01& \cone{0.000e+00}, 5e-05& \cthree{1.488e-05}, 4e-02\\
randn-500-1000 &-4.5e+02& 20 & 1.245e+04, 4e+03& 2.680e+04, 9e+01& 2.269e-05, 3e-02& \cone{0.000e+00}, 4e-04& \cthree{2.176e-07}, 1e-02& \ctwo{3.374e-09}, 5e-04& 2.383e-07, 4e-03\\
 \hline
w1a-2477-300 &-5.6e+02& 50 & 2.185e+03, 3e+03& 1.023e+04, 2e+02& 7.007e-06, 2e-02& 5.620e-07, 2e-03& \cthree{9.584e-08}, 2e-03& \cone{0.000e+00}, 3e-12& \ctwo{3.411e-13}, 2e-06\\
TDT2-500-1000 &-1.5e+03& 50 & 4.330e+04, 2e+05& 6.497e+04, 4e+04& 1.044e-02, 5e-01& \cthree{1.288e-03}, 2e+00& 8.943e-03, 8e-01& \cone{0.000e+00}, 3e-05& \ctwo{7.259e-04}, 2e-01\\
20News-8000-1000 &-1.1e+03& 50 & 8.254e+04, 5e+05& 1.636e+06, 3e+04& 1.283e+01, 2e+01& \cthree{7.286e+00}, 1e+01& 2.031e+01, 2e+02& \cone{0.000e+00}, 5e-03& \ctwo{2.679e+00}, 7e+00\\
sector-6412-1000 &-1.6e+03& 50 & 5.671e+08, 2e+09& 2.950e+08, 3e+02& 1.810e+03, 3e+02& \cthree{6.423e+01}, 6e+01& 5.649e+02, 2e+02& \ctwo{3.467e+01}, 2e+02& \cone{0.000e+00}, 2e+02\\
E2006-2000-1000 &-1.4e+03& 50 & 2.404e+05, 5e+05& 5.830e+06, 1e+05& 7.460e-03, 9e-01& \ctwo{3.085e-07}, 4e-03& \cthree{3.219e-07}, 6e-02& \cone{0.000e+00}, 8e-08& 8.483e-04, 2e-01\\
MNIST-60000-784 &-9.4e+02& 50 & 6.740e+03, 7e+04& 4.088e+05, 9e+01& \cthree{4.050e-02}, 9e-01& \cone{0.000e+00}, 3e-01& \ctwo{1.139e-04}, 8e-01& 3.053e-01, 5e+00& 5.622e-01, 6e+00\\
Gisette-3000-1000 &-6.4e+02& 50 & 1.009e+06, 1e+05& 1.160e+06, 9e+02& \cthree{2.267e-01}, 4e+00& \ctwo{2.025e-01}, 2e+01& \cone{0.000e+00}, 1e+00& 3.837e+02, 2e+02& 4.537e+02, 2e+02\\
CnnCaltech-3000-1000 &-1.4e+03& 50 & 4.604e+00, 2e+02& 6.053e+03, 4e+02& 1.462e-07, 6e-03& 4.699e-07, 2e-02& \cthree{1.589e-08}, 1e-03& \cone{0.000e+00}, 1e-11& \ctwo{5.637e-10}, 2e-04\\
Cifar-1000-1000 &-1.4e+03& 50 & 1.634e+05, 4e+05& 5.187e-03, 5e-01& \cthree{4.116e-03}, 5e-01& \cone{0.000e+00}, 5e-02& \ctwo{2.040e-05}, 3e-02& 8.315e-02, 3e+00& 1.319e-01, 3e+00\\
randn-500-1000 &-1.1e+03& 50 & 3.050e+04, 6e+03& 6.014e+04, 3e+02& \cthree{6.300e-05}, 5e-02& \cone{0.000e+00}, 3e-03& \ctwo{1.380e-07}, 3e-03& 4.662e+00, 2e+01& 6.682e+00, 2e+01\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1.00, time limit=50} \\ \hline
w1a-2477-300 &-1.2e+02& 10 & 4.672e+01, 8e+02& 7.805e-06, 1e-02& 4.860e-06, 1e-02& \cthree{1.230e-08}, 6e-04& 3.352e-08, 8e-04& \cone{0.000e+00}, 6e-13& \ctwo{1.421e-14}, 1e-12\\
TDT2-500-1000 &-3.1e+02& 10 & 1.473e+05, 6e+05& 1.234e-04, 7e-02& 7.167e-05, 8e-02& \cthree{1.266e-07}, 3e-03& 3.710e-07, 4e-03& \cone{0.000e+00}, 4e-06& \ctwo{4.263e-12}, 2e-05\\
20News-8000-1000 &-2.6e+02& 10 & 1.865e+04, 5e+05& 1.930e+05, 9e+04& 5.043e-03, 4e-01& \cthree{5.735e-06}, 3e-02& 9.833e-05, 3e-01& \cone{0.000e+00}, 5e-08& \ctwo{1.316e-07}, 5e-03\\
sector-6412-1000 &-3.2e+02& 10 & 1.619e+07, 3e+08& 2.950e+08, 1e+01& 7.767e-01, 9e+00& \cone{0.000e+00}, 1e-01& \cthree{1.273e-01}, 3e+00& \ctwo{4.534e-03}, 2e+01& 4.120e-01, 2e+01\\
E2006-2000-1000 &-2.9e+02& 10 & 5.948e+03, 2e+05& 8.158e+05, 3e+00& 7.679e-05, 8e-02& 1.373e-07, 3e-03& \cthree{1.153e-08}, 2e-03& \ctwo{2.274e-13}, 1e-08& \cone{0.000e+00}, 1e-08\\
MNIST-60000-784 &-1.9e+02& 10 & 1.972e+05, 3e+04& 3.006e+05, 3e-01& 1.902e-04, 2e-01& \cthree{2.043e-06}, 8e-03& 5.525e-06, 1e-02& \cone{0.000e+00}, 2e-05& \ctwo{2.558e-13}, 2e-05\\
Gisette-3000-1000 &-1.3e+02& 10 & 1.007e+06, 2e+05& 2.342e-01, 5e+00& 5.245e-02, 1e+00& \cthree{7.213e-04}, 1e-01& \cone{0.000e+00}, 2e-01& \ctwo{4.174e-05}, 5e-02& 4.357e-03, 4e-01\\
CnnCaltech-3000-1000 &-2.7e+02& 10 & 7.784e-02, 3e+01& 4.655e+03, 2e+02& 3.776e-09, 1e-03& \ctwo{8.134e-11}, 1e-04& \cthree{7.565e-10}, 2e-04& \cone{0.000e+00}, 2e-12& \cone{0.000e+00}, 2e-12\\
Cifar-1000-1000 &-2.9e+02& 10 & 1.318e+05, 2e+04& 3.550e+04, 1e+05& 1.204e-05, 4e-02& 1.052e-06, 8e-03& \cthree{8.839e-07}, 7e-03& \ctwo{1.137e-12}, 9e-06& \cone{0.000e+00}, 2e-06\\
randn-500-1000 &-2.2e+02& 10 & 4.624e+03, 3e+03& 1.394e+04, 6e+01& 5.621e-06, 2e-02& 2.911e-08, 4e-03& \cthree{1.435e-08}, 2e-03& \cone{0.000e+00}, 7e-12& \ctwo{8.811e-13}, 8e-06\\
 \hline
w1a-2477-300 &-2.3e+02& 20 & 3.037e+03, 8e+02& 7.394e+03, 1e+02& 3.756e-06, 1e-02& \ctwo{9.790e-08}, 1e-03& \cthree{1.562e-07}, 1e-03& \cone{0.000e+00}, 1e-12& \cone{0.000e+00}, 2e-12\\
TDT2-500-1000 &-6.2e+02& 20 & 4.235e+04, 4e+05& 2.786e-01, 3e+01& 4.600e-04, 1e-01& 2.082e-06, 4e-02& \cthree{3.859e-07}, 2e-02& \cone{0.000e+00}, 7e-06& \ctwo{2.330e-09}, 5e-04\\
20News-8000-1000 &-4.9e+02& 20 & 7.679e+05, 3e+06& 7.619e+05, 3e+00& 7.014e-01, 4e+00& \cthree{3.087e-02}, 1e+00& 3.848e-02, 8e-01& \cone{0.000e+00}, 2e-07& \ctwo{1.660e-05}, 2e-02\\
sector-6412-1000 &-6.3e+02& 20 & 3.720e+06, 2e+08& 2.950e+08, 1e+02& 6.795e+02, 2e+02& \cone{0.000e+00}, 6e+00& 2.004e+01, 4e+03& \ctwo{5.453e-01}, 9e+01& \cthree{9.415e-01}, 1e+02\\
E2006-2000-1000 &-5.7e+02& 20 & 1.408e+03, 4e+04& 3.125e+06, 5e+00& 3.056e-03, 4e-01& 3.673e-06, 4e-02& \cthree{4.979e-07}, 4e-03& \ctwo{1.137e-13}, 3e-08& \cone{0.000e+00}, 3e-08\\
MNIST-60000-784 &-3.9e+02& 20 & 1.970e+05, 3e+04& 3.543e+05, 6e+01& 5.824e-03, 5e-01& 2.475e-05, 2e-01& \cthree{1.876e-05}, 3e-02& \cone{0.000e+00}, 4e-05& \ctwo{5.542e-08}, 3e-03\\
Gisette-3000-1000 &-2.6e+02& 20 & 9.982e+05, 3e+05& 1.122e+06, 2e+00& \cthree{2.739e-01}, 2e+00& \ctwo{1.707e-02}, 7e+00& \cone{0.000e+00}, 5e+00& 1.007e+00, 8e+00& 1.641e+00, 8e+00\\
CnnCaltech-3000-1000 &-5.5e+02& 20 & 6.219e+01, 8e+02& 5.859e+03, 3e+02& 6.235e-09, 1e-03& 6.782e-09, 8e-04& \cthree{5.834e-09}, 1e-03& \ctwo{1.137e-13}, 2e-12& \cone{0.000e+00}, 3e-12\\
Cifar-1000-1000 &-5.7e+02& 20 & 4.175e+04, 1e+05& 5.423e+04, 1e+05& 1.549e-03, 3e-01& \cthree{2.378e-06}, 1e-02& 6.245e-05, 2e-01& \cone{0.000e+00}, 4e-05& \ctwo{2.291e-07}, 4e-03\\
randn-500-1000 &-4.5e+02& 20 & 1.245e+04, 4e+03& 2.680e+04, 9e+01& 2.269e-05, 3e-02& \ctwo{6.786e-10}, 4e-04& 2.183e-07, 1e-02& \cone{0.000e+00}, 3e-07& \cthree{2.186e-08}, 1e-03\\
 \hline
w1a-2477-300 &-5.6e+02& 50 & 2.185e+03, 3e+03& 1.023e+04, 2e+02& 7.007e-06, 2e-02& 5.620e-07, 2e-03& \cthree{9.584e-08}, 2e-03& \cone{0.000e+00}, 3e-12& \ctwo{1.137e-13}, 7e-09\\
TDT2-500-1000 &-1.5e+03& 50 & 4.330e+04, 2e+05& 6.497e+04, 4e+04& 1.044e-02, 5e-01& \cthree{1.288e-03}, 2e+00& 8.943e-03, 8e-01& \cone{0.000e+00}, 3e-05& \ctwo{7.843e-05}, 5e-02\\
20News-8000-1000 &-1.1e+03& 50 & 8.254e+04, 5e+05& 1.636e+06, 3e+04& 1.283e+01, 2e+01& \cthree{7.286e+00}, 1e+01& 2.031e+01, 2e+02& \cone{0.000e+00}, 8e-05& \ctwo{1.558e+00}, 5e+00\\
sector-6412-1000 &-1.6e+03& 50 & 5.671e+08, 2e+09& 2.950e+08, 3e+02& 1.810e+03, 3e+02& \cthree{6.428e+01}, 6e+01& 5.649e+02, 2e+02& \ctwo{2.579e+01}, 2e+02& \cone{0.000e+00}, 2e+02\\
E2006-2000-1000 &-1.4e+03& 50 & 2.404e+05, 5e+05& 5.830e+06, 1e+05& 7.460e-03, 9e-01& \ctwo{3.085e-07}, 4e-03& \cthree{3.218e-07}, 6e-02& \cone{0.000e+00}, 8e-08& 5.455e-06, 2e-02\\
MNIST-60000-784 &-9.4e+02& 50 & 6.740e+03, 7e+04& 4.088e+05, 9e+01& 4.050e-02, 9e-01& \cone{0.000e+00}, 3e-01& \ctwo{1.139e-04}, 8e-01& \cthree{2.605e-03}, 5e-01& 3.430e-03, 6e-01\\
Gisette-3000-1000 &-6.4e+02& 50 & 1.009e+06, 1e+05& 1.160e+06, 9e+02& \cthree{2.267e-01}, 4e+00& \ctwo{2.025e-01}, 2e+01& \cone{0.000e+00}, 1e+00& 2.086e+02, 1e+02& 2.638e+02, 1e+02\\
CnnCaltech-3000-1000 &-1.4e+03& 50 & 4.604e+00, 2e+02& 6.053e+03, 4e+02& 1.462e-07, 6e-03& 4.699e-07, 2e-02& \cthree{1.589e-08}, 1e-03& \cone{0.000e+00}, 5e-12& \ctwo{2.728e-12}, 1e-05\\
Cifar-1000-1000 &-1.4e+03& 50 & 1.634e+05, 4e+05& 5.187e-03, 5e-01& 4.116e-03, 5e-01& \cone{0.000e+00}, 5e-02& \ctwo{2.040e-05}, 3e-02& \cthree{2.152e-04}, 1e-01& 9.108e-03, 1e+00\\
randn-500-1000 &-1.1e+03& 50 & 3.050e+04, 6e+03& 6.014e+04, 3e+02& \cthree{6.300e-05}, 5e-02& \cone{0.000e+00}, 3e-03& \ctwo{1.380e-07}, 3e-03& 2.012e-01, 4e+00& 3.110e-01, 4e+00\\
\hline
\end{tabular}}
\caption{Comparisons of objective values and Riemannian gradient residuals $(F(\X)-F_{\text{min}}, \| \G^t - \X^t [\G^t]\trans \X^t \|_{\fro})$ for nonlinear eigenvalue problems for all the compared methods with $\lambda=1$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively.}
\label{tab:nlevp:1}
\end{table*}




\begin{table*}[!h]
\centering
\scalebox{0.4}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline \multirow{2}*{data-m-n}  & \multirow{2}*{$F_{\text{min}}$}  & \multirow{2}*{r} & \multirow{2}*{FOForth-GR}  &  \multirow{2}*{FOForth-P}  & \multirow{2}*{FOForth-QR} & \multirow{2}*{OptM-QR} &\multirow{2}*{OptM-Cayley} &  \multirow{2}*{OBCD-SV}    &\multirow{2}*{OBCD-OR} \\
   &  &   &    &   &  &    &   &     &    \\
   \hline\hline
\multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=20} \\ \hline
w1a-2477-300 &1.0e+03& 10 & 1.733e+04, 5e+04& \ctwo{5.517e+03}, 2e+03& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cone{0.000e+00}, 2e+03\\
TDT2-500-1000 &2.1e+03& 10 & 3.938e+10, 2e+11& 1.352e+07, 1e+08& 1.140e+06, 1e+07& \cthree{6.451e+04}, 4e+05& 7.522e+04, 1e+06& \ctwo{5.516e+04}, 3e+05& \cone{0.000e+00}, 4e+04\\
20News-8000-1000 &2.2e+05& 10 & 1.137e+11, 1e+12& 1.806e+11, 1e+06& 2.039e+06, 3e+06& \cthree{5.350e+05}, 1e+06& 7.305e+05, 1e+06& \ctwo{7.368e+04}, 9e+05& \cone{0.000e+00}, 4e+05\\
sector-6412-1000 &2.4e+03& 10 & 6.879e+14, 1e+15& 2.950e+14, 1e+07& 1.415e+15, 3e+15& \cthree{1.285e+06}, 2e+06& 3.704e+06, 3e+06& \ctwo{1.566e+05}, 2e+07& \cone{0.000e+00}, 1e+08\\
E2006-2000-1000 &-1.0e+02& 10 & 4.841e+11, 5e+11& 1.195e+12, 1e+11& \ctwo{4.664e+04}, 6e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cone{0.000e+00}, 6e+03\\
MNIST-60000-784 &2.9e+02& 10 & 1.206e+07, 2e+08& 1.140e+10, 9e+05& 1.357e+04, 9e+04& \ctwo{1.354e+04}, 9e+04& \cthree{1.356e+04}, 9e+04& \ctwo{1.354e+04}, 9e+04& \cone{0.000e+00}, 2e+03\\
Gisette-3000-1000 &6.5e+02& 10 & 1.015e+06, 1e+05& 3.550e+04, 4e+05& 7.393e+03, 3e+04& \cthree{7.388e+03}, 3e+04& \ctwo{7.341e+03}, 3e+04& 7.463e+03, 3e+04& \cone{0.000e+00}, 2e+03\\
CnnCaltech-3000-1000 &-7.9e+01& 10 & \cthree{3.364e+03}, 5e+03& 5.438e+03, 5e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \cone{0.000e+00}, 1e+03\\
Cifar-1000-1000 &2.0e+02& 10 & 1.897e+10, 8e+10& 4.606e+04, 2e+06& 6.244e+03, 1e+06& \cthree{6.089e+03}, 3e+05& 6.106e+03, 3e+05& \ctwo{5.449e+03}, 9e+04& \cone{0.000e+00}, 1e+04\\
randn-500-1000 &-1.9e+02& 10 & \cthree{7.163e+03}, 3e+03& 1.387e+04, 2e+02& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \cone{0.000e+00}, 7e+01\\
 \hline
w1a-2477-300 &4.4e+03& 20 & 4.831e+04, 8e+04& \ctwo{5.014e+03}, 3e+03& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cone{0.000e+00}, 4e+03\\
TDT2-500-1000 &1.0e+04& 20 & 3.171e+11, 1e+12& 4.426e+08, 1e+09& 3.895e+06, 8e+06& \cthree{1.293e+05}, 1e+06& 1.322e+05, 6e+05& \ctwo{1.112e+05}, 5e+05& \cone{0.000e+00}, 1e+05\\
20News-8000-1000 &1.0e+06& 20 & 8.928e+10, 9e+11& 7.614e+11, 1e+06& 8.550e+06, 2e+07& \cthree{1.019e+06}, 4e+06& 1.412e+06, 2e+06& \cone{0.000e+00}, 1e+06& \ctwo{9.134e+05}, 1e+06\\
sector-6412-1000 &5.8e+03& 20 & 5.112e+14, 8e+14& 2.949e+14, 2e+08& 1.954e+15, 2e+15& \cthree{1.097e+06}, 2e+06& 4.854e+06, 4e+07& \ctwo{3.945e+05}, 2e+08& \cone{0.000e+00}, 6e+08\\
E2006-2000-1000 &-2.6e+02& 20 & 6.260e+11, 2e+12& 2.954e+12, 2e+06& \ctwo{7.775e+04}, 8e+05& \cthree{8.194e+04}, 8e+05& 8.197e+04, 8e+05& \cthree{8.194e+04}, 8e+05& \cone{0.000e+00}, 9e+03\\
MNIST-60000-784 &6.8e+02& 20 & 1.041e+07, 1e+07& 1.222e+10, 1e+06& 3.203e+04, 2e+05& \ctwo{3.160e+04}, 2e+05& \cthree{3.175e+04}, 2e+05& \ctwo{3.160e+04}, 2e+05& \cone{0.000e+00}, 3e+03\\
Gisette-3000-1000 &1.9e+03& 20 & \ctwo{1.804e+04}, 3e+05& 1.120e+06, 1e+03& 1.958e+04, 5e+04& \cthree{1.950e+04}, 5e+04& 1.952e+04, 5e+04& 2.445e+04, 6e+04& \cone{0.000e+00}, 3e+03\\
CnnCaltech-3000-1000 &-3.1e+02& 20 & \ctwo{2.418e+03}, 1e+04& \cthree{7.702e+03}, 9e+03& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &9.6e+02& 20 & 1.231e+10, 8e+10& 3.894e+04, 3e+05& 4.082e+04, 6e+07& \cthree{1.102e+04}, 2e+07& 1.171e+04, 3e+06& \ctwo{5.351e+03}, 1e+05& \cone{0.000e+00}, 4e+04\\
randn-500-1000 &-3.3e+02& 20 & 1.310e+04, 4e+03& 2.680e+04, 2e+02& \ctwo{6.728e+00}, 2e+02& \cthree{6.731e+00}, 2e+02& \cthree{6.731e+00}, 2e+02& \cthree{6.731e+00}, 2e+02& \cone{0.000e+00}, 2e+02\\
 \hline
w1a-2477-300 &1.6e+04& 50 & \cthree{2.238e+05}, 2e+05& \cone{0.000e+00}, 9e+03& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& \ctwo{6.037e+03}, 1e+04\\
TDT2-500-1000 &8.6e+04& 50 & 1.719e+11, 7e+11& 3.835e+09, 3e+09& 3.783e+07, 2e+07& \cthree{2.735e+05}, 2e+06& 4.909e+05, 1e+06& \ctwo{2.246e+05}, 9e+05& \cone{0.000e+00}, 4e+05\\
20News-8000-1000 &3.1e+07& 50 & 4.593e+10, 4e+11& 1.630e+12, 4e+10& 2.496e+06, 6e+07& \cthree{4.338e+05}, 2e+07& \ctwo{2.755e+05}, 2e+07& \cone{0.000e+00}, 2e+06& 5.304e+06, 8e+06\\
sector-6412-1000 &3.8e+04& 50 & 2.327e+14, 1e+15& 2.950e+14, 4e+08& 8.104e+14, 1e+15& \cthree{8.457e+06}, 7e+06& 9.531e+06, 4e+07& \ctwo{1.754e+06}, 5e+08& \cone{0.000e+00}, 1e+09\\
E2006-2000-1000 &-7.5e+02& 50 & 4.266e+10, 2e+11& 5.868e+12, 3e+10& 1.695e+05, 1e+06& \ctwo{1.651e+05}, 1e+06& \cthree{1.662e+05}, 1e+06& \ctwo{1.651e+05}, 1e+06& \cone{0.000e+00}, 1e+04\\
MNIST-60000-784 &3.2e+03& 50 & 1.797e+09, 1e+10& 1.425e+10, 6e+06& \cthree{1.018e+05}, 3e+05& \ctwo{1.013e+05}, 3e+05& 1.021e+05, 3e+05& 1.028e+05, 3e+05& \cone{0.000e+00}, 7e+03\\
Gisette-3000-1000 &7.6e+03& 50 & 1.026e+06, 9e+04& 1.158e+06, 2e+03& 8.110e+04, 1e+05& \cthree{8.105e+04}, 1e+05& \ctwo{8.101e+04}, 1e+05& 8.472e+04, 2e+05& \cone{0.000e+00}, 8e+03\\
CnnCaltech-3000-1000 &-8.6e+02& 50 & \cthree{6.567e+03}, 3e+04& 1.130e+04, 2e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &5.2e+03& 50 & 1.716e+09, 2e+10& 1.010e+06, 2e+06& 1.805e+05, 1e+07& \cthree{7.957e+03}, 3e+05& 1.047e+04, 1e+07& \ctwo{7.682e+03}, 3e+05& \cone{0.000e+00}, 1e+05\\
randn-500-1000 &-4.4e+02& 50 & 3.284e+04, 6e+03& 6.135e+04, 7e+02& \cthree{3.018e+01}, 6e+02& \ctwo{3.017e+01}, 6e+02& \ctwo{3.017e+01}, 6e+02& 6.981e+01, 6e+02& \cone{0.000e+00}, 6e+02\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=30} \\ \hline
w1a-2477-300 &1.0e+03& 10 & 1.733e+04, 5e+04& \ctwo{5.517e+03}, 2e+03& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cone{0.000e+00}, 2e+03\\
TDT2-500-1000 &1.1e+03& 10 & 3.938e+10, 2e+11& 1.353e+07, 1e+08& 1.141e+06, 1e+07& \cthree{6.549e+04}, 4e+05& 7.620e+04, 1e+06& \ctwo{5.614e+04}, 3e+05& \cone{0.000e+00}, 2e+04\\
20News-8000-1000 &1.1e+05& 10 & 1.137e+11, 1e+12& 1.806e+11, 1e+06& 2.148e+06, 3e+06& \cthree{6.444e+05}, 1e+06& 8.398e+05, 1e+06& \ctwo{1.830e+05}, 9e+05& \cone{0.000e+00}, 3e+05\\
sector-6412-1000 &2.4e+03& 10 & 6.879e+14, 1e+15& 2.950e+14, 1e+07& 1.415e+15, 3e+15& \cthree{1.285e+06}, 2e+06& 3.704e+06, 3e+06& \ctwo{1.576e+05}, 3e+07& \cone{0.000e+00}, 1e+08\\
E2006-2000-1000 &-1.0e+02& 10 & 4.841e+11, 5e+11& 1.195e+12, 1e+11& \ctwo{4.664e+04}, 6e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cone{0.000e+00}, 6e+03\\
MNIST-60000-784 &2.9e+02& 10 & 1.206e+07, 2e+08& 1.140e+10, 9e+05& 1.357e+04, 9e+04& \ctwo{1.354e+04}, 9e+04& \cthree{1.356e+04}, 9e+04& \ctwo{1.354e+04}, 9e+04& \cone{0.000e+00}, 2e+03\\
Gisette-3000-1000 &6.3e+02& 10 & 1.015e+06, 1e+05& 3.551e+04, 4e+05& 7.411e+03, 3e+04& 7.406e+03, 3e+04& \ctwo{7.359e+03}, 3e+04& \cthree{7.399e+03}, 3e+04& \cone{0.000e+00}, 2e+03\\
CnnCaltech-3000-1000 &-7.9e+01& 10 & \cthree{3.364e+03}, 5e+03& 5.438e+03, 5e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \cone{0.000e+00}, 1e+03\\
Cifar-1000-1000 &3.6e+01& 10 & 1.897e+10, 8e+10& 4.623e+04, 2e+06& 6.411e+03, 1e+06& \cthree{6.256e+03}, 3e+05& 6.272e+03, 3e+05& \ctwo{5.616e+03}, 9e+04& \cone{0.000e+00}, 8e+03\\
randn-500-1000 &-1.9e+02& 10 & \cthree{7.163e+03}, 3e+03& 1.387e+04, 2e+02& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \cone{0.000e+00}, 7e+01\\
 \hline
w1a-2477-300 &4.4e+03& 20 & 4.831e+04, 8e+04& \ctwo{5.014e+03}, 3e+03& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cone{0.000e+00}, 4e+03\\
TDT2-500-1000 &5.7e+03& 20 & 3.171e+11, 1e+12& 4.426e+08, 1e+09& 3.900e+06, 8e+06& \cthree{1.338e+05}, 1e+06& 1.368e+05, 6e+05& \ctwo{1.158e+05}, 5e+05& \cone{0.000e+00}, 8e+04\\
20News-8000-1000 &1.0e+06& 20 & 8.928e+10, 9e+11& 7.614e+11, 1e+06& 8.550e+06, 2e+07& \cthree{1.019e+06}, 4e+06& 1.412e+06, 2e+06& \cone{0.000e+00}, 1e+06& \ctwo{3.283e+05}, 1e+06\\
sector-6412-1000 &5.7e+03& 20 & 5.112e+14, 8e+14& 2.949e+14, 2e+08& 1.954e+15, 2e+15& \cthree{1.097e+06}, 2e+06& 4.854e+06, 4e+07& \ctwo{3.899e+05}, 2e+08& \cone{0.000e+00}, 6e+08\\
E2006-2000-1000 &-2.6e+02& 20 & 6.260e+11, 2e+12& 2.954e+12, 2e+06& \ctwo{7.775e+04}, 8e+05& \cthree{8.194e+04}, 8e+05& 8.197e+04, 8e+05& \cthree{8.194e+04}, 8e+05& \cone{0.000e+00}, 9e+03\\
MNIST-60000-784 &6.7e+02& 20 & 1.041e+07, 1e+07& 1.222e+10, 1e+06& 3.204e+04, 2e+05& \ctwo{3.161e+04}, 2e+05& \cthree{3.176e+04}, 2e+05& \ctwo{3.161e+04}, 2e+05& \cone{0.000e+00}, 3e+03\\
Gisette-3000-1000 &1.8e+03& 20 & \ctwo{1.813e+04}, 3e+05& 1.120e+06, 1e+03& 1.966e+04, 5e+04& \cthree{1.959e+04}, 5e+04& 1.961e+04, 5e+04& 2.111e+04, 6e+04& \cone{0.000e+00}, 3e+03\\
CnnCaltech-3000-1000 &-3.1e+02& 20 & \ctwo{2.418e+03}, 1e+04& \cthree{7.702e+03}, 9e+03& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &4.6e+02& 20 & 1.231e+10, 8e+10& 3.943e+04, 3e+05& 4.131e+04, 6e+07& \cthree{1.151e+04}, 2e+07& 1.220e+04, 3e+06& \ctwo{5.815e+03}, 1e+05& \cone{0.000e+00}, 2e+04\\
randn-500-1000 &-3.3e+02& 20 & 1.310e+04, 4e+03& 2.680e+04, 2e+02& \ctwo{6.729e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cone{0.000e+00}, 2e+02\\
 \hline
w1a-2477-300 &1.6e+04& 50 & \cthree{2.238e+05}, 2e+05& \cone{0.000e+00}, 9e+03& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& \ctwo{6.033e+03}, 1e+04\\
TDT2-500-1000 &5.3e+04& 50 & 1.719e+11, 7e+11& 3.835e+09, 3e+09& 3.787e+07, 2e+07& \cthree{3.060e+05}, 2e+06& 5.233e+05, 1e+06& \ctwo{2.571e+05}, 9e+05& \cone{0.000e+00}, 3e+05\\
20News-8000-1000 &3.1e+07& 50 & 4.593e+10, 4e+11& 1.630e+12, 4e+10& 2.516e+06, 6e+07& \cthree{4.539e+05}, 2e+07& \ctwo{2.956e+05}, 2e+07& \cone{0.000e+00}, 2e+06& 3.502e+06, 7e+06\\
sector-6412-1000 &2.1e+04& 50 & 2.327e+14, 1e+15& 2.950e+14, 4e+08& 8.104e+14, 1e+15& \cthree{8.474e+06}, 7e+06& 9.548e+06, 4e+07& \ctwo{1.654e+06}, 5e+08& \cone{0.000e+00}, 1e+09\\
E2006-2000-1000 &-7.7e+02& 50 & 4.266e+10, 2e+11& 5.868e+12, 3e+10& 1.695e+05, 1e+06& \ctwo{1.651e+05}, 1e+06& 1.662e+05, 1e+06& \cthree{1.652e+05}, 1e+06& \cone{0.000e+00}, 1e+04\\
MNIST-60000-784 &2.7e+03& 50 & 1.797e+09, 1e+10& 1.425e+10, 6e+06& 1.023e+05, 3e+05& \ctwo{1.018e+05}, 3e+05& 1.026e+05, 3e+05& \cthree{1.021e+05}, 3e+05& \cone{0.000e+00}, 7e+03\\
Gisette-3000-1000 &7.6e+03& 50 & 1.026e+06, 9e+04& 1.158e+06, 2e+03& 8.105e+04, 1e+05& \cthree{8.099e+04}, 1e+05& \ctwo{8.096e+04}, 1e+05& 9.215e+04, 1e+05& \cone{0.000e+00}, 8e+03\\
CnnCaltech-3000-1000 &-8.6e+02& 50 & \cthree{6.567e+03}, 3e+04& 1.130e+04, 2e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &3.6e+03& 50 & 1.716e+09, 2e+10& 1.012e+06, 2e+06& 1.821e+05, 1e+07& \cthree{9.595e+03}, 3e+05& 1.211e+04, 1e+07& \ctwo{6.024e+03}, 5e+05& \cone{0.000e+00}, 6e+04\\
randn-500-1000 &-4.7e+02& 50 & 3.287e+04, 6e+03& 6.138e+04, 7e+02& \cthree{6.788e+01}, 6e+02& \ctwo{6.787e+01}, 6e+02& \ctwo{6.787e+01}, 6e+02& 7.418e+01, 6e+02& \cone{0.000e+00}, 6e+02\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 100.00, time limit=50} \\ \hline
w1a-2477-300 &1.0e+03& 10 & 1.733e+04, 5e+04& \ctwo{5.517e+03}, 2e+03& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cthree{1.691e+04}, 5e+04& \cone{0.000e+00}, 2e+03\\
TDT2-500-1000 &5.0e+02& 10 & 3.938e+10, 2e+11& 1.353e+07, 1e+08& 1.141e+06, 1e+07& \cthree{6.610e+04}, 4e+05& 7.681e+04, 1e+06& \ctwo{5.675e+04}, 3e+05& \cone{0.000e+00}, 1e+04\\
20News-8000-1000 &3.3e+04& 10 & 1.137e+11, 1e+12& 1.806e+11, 1e+06& 2.223e+06, 3e+06& \cthree{7.188e+05}, 1e+06& 9.143e+05, 1e+06& \ctwo{2.575e+05}, 9e+05& \cone{0.000e+00}, 1e+05\\
sector-6412-1000 &2.4e+03& 10 & 6.879e+14, 1e+15& 2.950e+14, 1e+07& 1.415e+15, 3e+15& \cthree{1.285e+06}, 2e+06& 3.704e+06, 3e+06& \ctwo{1.580e+05}, 2e+07& \cone{0.000e+00}, 1e+08\\
E2006-2000-1000 &-1.0e+02& 10 & 4.841e+11, 5e+11& 1.195e+12, 1e+11& \ctwo{4.664e+04}, 6e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cthree{4.666e+04}, 5e+05& \cone{0.000e+00}, 6e+03\\
MNIST-60000-784 &2.9e+02& 10 & 1.206e+07, 2e+08& 1.140e+10, 9e+05& 1.357e+04, 9e+04& \ctwo{1.354e+04}, 9e+04& \cthree{1.356e+04}, 9e+04& \ctwo{1.354e+04}, 9e+04& \cone{0.000e+00}, 2e+03\\
Gisette-3000-1000 &6.2e+02& 10 & 1.015e+06, 1e+05& 3.552e+04, 4e+05& 7.419e+03, 3e+04& 7.413e+03, 3e+04& \ctwo{7.367e+03}, 3e+04& \cthree{7.397e+03}, 3e+04& \cone{0.000e+00}, 2e+03\\
CnnCaltech-3000-1000 &-7.9e+01& 10 & \cthree{3.364e+03}, 5e+03& 5.438e+03, 5e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \ctwo{1.145e+03}, 6e+03& \cone{0.000e+00}, 1e+03\\
Cifar-1000-1000 &-8.6e+01& 10 & 1.897e+10, 8e+10& 4.635e+04, 2e+06& 6.533e+03, 1e+06& \cthree{6.378e+03}, 3e+05& 6.395e+03, 3e+05& \ctwo{5.738e+03}, 9e+04& \cone{0.000e+00}, 9e+03\\
randn-500-1000 &-1.9e+02& 10 & \cthree{7.163e+03}, 3e+03& 1.387e+04, 2e+02& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \ctwo{1.015e+00}, 7e+01& \cone{0.000e+00}, 7e+01\\
 \hline
w1a-2477-300 &4.4e+03& 20 & 4.831e+04, 8e+04& \ctwo{5.014e+03}, 3e+03& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cthree{4.827e+04}, 8e+04& \cone{0.000e+00}, 4e+03\\
TDT2-500-1000 &2.3e+03& 20 & 3.171e+11, 1e+12& 4.426e+08, 1e+09& 3.903e+06, 8e+06& \cthree{1.372e+05}, 1e+06& 1.401e+05, 6e+05& \ctwo{1.192e+05}, 5e+05& \cone{0.000e+00}, 4e+04\\
20News-8000-1000 &9.7e+05& 20 & 8.928e+10, 9e+11& 7.614e+11, 1e+06& 8.608e+06, 2e+07& \cthree{1.077e+06}, 4e+06& 1.470e+06, 2e+06& \ctwo{5.819e+04}, 1e+06& \cone{0.000e+00}, 6e+05\\
sector-6412-1000 &5.7e+03& 20 & 5.112e+14, 8e+14& 2.949e+14, 2e+08& 1.954e+15, 2e+15& \cthree{1.097e+06}, 2e+06& 4.854e+06, 4e+07& \ctwo{3.868e+05}, 2e+08& \cone{0.000e+00}, 6e+08\\
E2006-2000-1000 &-2.6e+02& 20 & 6.260e+11, 2e+12& 2.954e+12, 2e+06& \ctwo{7.775e+04}, 8e+05& \cthree{8.194e+04}, 8e+05& 8.197e+04, 8e+05& \cthree{8.194e+04}, 8e+05& \cone{0.000e+00}, 9e+03\\
MNIST-60000-784 &6.7e+02& 20 & 1.041e+07, 1e+07& 1.222e+10, 1e+06& 3.204e+04, 2e+05& \ctwo{3.162e+04}, 2e+05& \cthree{3.177e+04}, 2e+05& \ctwo{3.162e+04}, 2e+05& \cone{0.000e+00}, 3e+03\\
Gisette-3000-1000 &1.7e+03& 20 & \ctwo{1.823e+04}, 3e+05& 1.121e+06, 1e+03& 1.977e+04, 5e+04& \cthree{1.969e+04}, 5e+04& 1.971e+04, 5e+04& 1.989e+04, 6e+04& \cone{0.000e+00}, 3e+03\\
CnnCaltech-3000-1000 &-3.1e+02& 20 & \ctwo{2.418e+03}, 1e+04& \cthree{7.702e+03}, 9e+03& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \ctwo{2.418e+03}, 1e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &9.4e+00& 20 & 1.231e+10, 8e+10& 3.989e+04, 3e+05& 4.177e+04, 6e+07& \cthree{1.196e+04}, 2e+07& 1.266e+04, 3e+06& \ctwo{6.268e+03}, 1e+05& \cone{0.000e+00}, 2e+04\\
randn-500-1000 &-3.3e+02& 20 & 1.310e+04, 4e+03& 2.680e+04, 2e+02& \ctwo{6.729e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cthree{6.732e+00}, 2e+02& \cone{0.000e+00}, 2e+02\\
 \hline
w1a-2477-300 &1.6e+04& 50 & \cthree{2.238e+05}, 2e+05& \cone{0.000e+00}, 9e+03& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& 2.291e+05, 2e+05& \ctwo{6.031e+03}, 1e+04\\
TDT2-500-1000 &2.5e+04& 50 & 1.719e+11, 7e+11& 3.835e+09, 3e+09& 3.790e+07, 2e+07& \cthree{3.342e+05}, 2e+06& 5.516e+05, 1e+06& \ctwo{2.853e+05}, 9e+05& \cone{0.000e+00}, 3e+05\\
20News-8000-1000 &3.1e+07& 50 & 4.593e+10, 4e+11& 1.630e+12, 4e+10& 2.527e+06, 6e+07& \cthree{4.646e+05}, 2e+07& \ctwo{3.063e+05}, 2e+07& \cone{0.000e+00}, 2e+06& 1.715e+06, 5e+06\\
sector-6412-1000 &1.7e+04& 50 & 2.327e+14, 1e+15& 2.950e+14, 4e+08& 8.104e+14, 1e+15& \cthree{8.478e+06}, 7e+06& 9.552e+06, 4e+07& \ctwo{1.559e+06}, 5e+08& \cone{0.000e+00}, 1e+09\\
E2006-2000-1000 &-7.7e+02& 50 & 4.266e+10, 2e+11& 5.868e+12, 3e+10& 1.695e+05, 1e+06& \ctwo{1.651e+05}, 1e+06& 1.662e+05, 1e+06& \cthree{1.652e+05}, 1e+06& \cone{0.000e+00}, 1e+04\\
MNIST-60000-784 &2.3e+03& 50 & 1.797e+09, 1e+10& 1.425e+10, 6e+06& 1.027e+05, 3e+05& \cthree{1.023e+05}, 3e+05& 1.031e+05, 3e+05& \ctwo{1.021e+05}, 3e+05& \cone{0.000e+00}, 6e+03\\
Gisette-3000-1000 &7.3e+03& 50 & 1.026e+06, 9e+04& 1.158e+06, 2e+03& 8.131e+04, 1e+05& \cthree{8.126e+04}, 1e+05& \ctwo{8.122e+04}, 1e+05& 9.099e+04, 1e+05& \cone{0.000e+00}, 7e+03\\
CnnCaltech-3000-1000 &-8.6e+02& 50 & \cthree{6.567e+03}, 3e+04& 1.130e+04, 2e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \ctwo{6.566e+03}, 3e+04& \cone{0.000e+00}, 2e+03\\
Cifar-1000-1000 &2.0e+03& 50 & 1.716e+09, 2e+10& 1.014e+06, 2e+06& 1.836e+05, 1e+07& \cthree{1.113e+04}, 3e+05& 1.364e+04, 1e+07& \ctwo{5.078e+03}, 2e+05& \cone{0.000e+00}, 5e+04\\
randn-500-1000 &-4.8e+02& 50 & 3.288e+04, 6e+03& 6.140e+04, 7e+02& \cthree{7.907e+01}, 6e+02& \ctwo{7.906e+01}, 6e+02& \ctwo{7.906e+01}, 6e+02& 7.948e+01, 6e+02& \cone{0.000e+00}, 6e+02\\
\hline
\end{tabular}}
\caption{Comparisons of objective values and Riemannian gradient residuals $(F(\X)-F_{\text{min}}, \| \G^t - \X^t [\G^t]\trans \X^t \|_{\fro})$ for nonlinear eigenvalue problems for all the compared methods with $\lambda=100$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively.}
\label{tab:nlevp:2}
\end{table*}




\begin{table*}[!h]
\centering
\scalebox{0.4}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline \multirow{2}*{data-m-n}  & \multirow{2}*{$F_{\text{min}}$}  & \multirow{2}*{r} & \multirow{2}*{FOForth-GR}  &  \multirow{2}*{FOForth-P}  & \multirow{2}*{FOForth-QR} & \multirow{2}*{OptM-QR} &\multirow{2}*{OptM-Cayley} &  \multirow{2}*{OBCD-SV}    &\multirow{2}*{OBCD-OR} \\
   &  &   &    &   &  &    &   &     &    \\
   \hline\hline
\multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=20} \\ \hline
w1a-2477-300 &4.5e+03& 10 & 7.536e+06, 1e+07& \ctwo{6.164e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cone{0.000e+00}, 3e+04\\
TDT2-500-1000 &2.2e+06& 10 & 7.867e+14, 2e+15& 2.353e+11, 2e+11& 2.088e+09, 2e+09& 3.596e+07, 2e+08& \cthree{1.286e+07}, 9e+07& \ctwo{3.620e+06}, 4e+07& \cone{0.000e+00}, 4e+07\\
20News-8000-1000 &1.5e+07& 10 & 1.883e+15, 3e+15& 1.806e+14, 3e+08& 6.430e+09, 1e+10& \cthree{5.718e+08}, 1e+09& 7.112e+08, 2e+10& \cone{0.000e+00}, 1e+08& \ctwo{2.756e+08}, 5e+08\\
sector-6412-1000 &3.8e+05& 10 & 3.004e+17, 6e+17& 2.950e+17, 1e+10& 1.969e+18, 3e+18& \cthree{1.355e+08}, 9e+10& 3.637e+09, 2e+10& \ctwo{2.651e+07}, 6e+10& \cone{0.000e+00}, 3e+11\\
E2006-2000-1000 &1.0e+02& 10 & 7.927e+12, 2e+14& 1.501e+15, 2e+08& 5.255e+06, 1e+08& 2.753e+06, 6e+07& \ctwo{2.717e+06}, 6e+07& \cthree{2.752e+06}, 6e+07& \cone{0.000e+00}, 6e+04\\
MNIST-60000-784 &5.4e+03& 10 & 4.121e+08, 8e+08& 1.312e+13, 9e+07& \ctwo{2.610e+06}, 1e+07& 2.742e+06, 1e+07& \cthree{2.741e+06}, 1e+07& 2.742e+06, 1e+07& \cone{0.000e+00}, 4e+04\\
Gisette-3000-1000 &3.1e+04& 10 & 3.248e+06, 2e+07& 9.757e+06, 8e+08& 2.990e+06, 8e+06& \ctwo{2.971e+06}, 8e+06& \cthree{2.977e+06}, 8e+06& 3.008e+06, 8e+06& \cone{0.000e+00}, 8e+04\\
CnnCaltech-3000-1000 &6.5e+03& 10 & \cthree{9.057e+05}, 4e+06& 1.047e+06, 6e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &5.2e+05& 10 & 1.126e+13, 5e+13& 1.525e+09, 2e+09& 2.618e+07, 8e+07& 1.989e+06, 8e+07& \cthree{1.460e+06}, 5e+08& \ctwo{4.326e+05}, 2e+07& \cone{0.000e+00}, 7e+06\\
randn-500-1000 &1.0e+04& 10 & 2.875e+04, 6e+04& 3.612e+04, 7e+04& \cthree{2.406e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \cone{0.000e+00}, 2e+04\\
 \hline
w1a-2477-300 &1.5e+05& 20 & 2.042e+07, 2e+07& \ctwo{2.156e+06}, 3e+06& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cone{0.000e+00}, 2e+05\\
TDT2-500-1000 &1.1e+07& 20 & 2.734e+13, 2e+14& 1.674e+12, 2e+12& 5.777e+09, 9e+09& \cthree{8.100e+07}, 3e+08& 1.292e+08, 4e+08& \ctwo{2.167e+05}, 7e+07& \cone{0.000e+00}, 1e+08\\
20News-8000-1000 &6.7e+08& 20 & 8.388e+13, 9e+14& 9.134e+14, 3e+08& 5.325e+11, 4e+11& 2.993e+09, 2e+09& \cthree{2.759e+09}, 2e+09& \cone{0.000e+00}, 2e+08& \ctwo{1.432e+09}, 2e+09\\
sector-6412-1000 &2.3e+06& 20 & 5.014e+17, 1e+18& 2.950e+17, 2e+11& 8.719e+17, 2e+18& \cthree{1.649e+09}, 4e+09& 4.498e+09, 3e+09& \ctwo{6.307e+07}, 4e+11& \cone{0.000e+00}, 7e+11\\
E2006-2000-1000 &7.6e+01& 20 & 5.457e+13, 5e+14& 1.841e+15, 4e+08& 4.168e+07, 3e+08& \cthree{4.663e+06}, 1e+08& 4.974e+06, 6e+08& \ctwo{4.645e+06}, 9e+07& \cone{0.000e+00}, 9e+04\\
MNIST-60000-784 &1.5e+04& 20 & 2.670e+11, 2e+11& 1.418e+13, 4e+10& 7.359e+06, 7e+08& 6.582e+06, 2e+07& \ctwo{6.434e+06}, 2e+07& \cthree{6.567e+06}, 2e+07& \cone{0.000e+00}, 7e+04\\
Gisette-3000-1000 &8.1e+04& 20 & \ctwo{4.320e+06}, 3e+07& 1.623e+07, 7e+07& 7.767e+06, 1e+07& \cthree{7.721e+06}, 1e+07& 7.794e+06, 1e+07& 9.044e+06, 2e+07& \cone{0.000e+00}, 1e+05\\
CnnCaltech-3000-1000 &2.3e+04& 20 & \cthree{1.335e+06}, 6e+06& 2.394e+06, 1e+07& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &1.2e+06& 20 & 5.981e+12, 7e+13& 1.955e+08, 1e+09& 6.344e+07, 2e+08& 1.721e+06, 1e+08& \cthree{1.553e+06}, 3e+07& \ctwo{3.365e+05}, 5e+07& \cone{0.000e+00}, 2e+07\\
randn-500-1000 &2.6e+04& 20 & \cthree{1.063e+05}, 2e+05& 1.177e+05, 2e+05& \ctwo{9.968e+04}, 2e+05& \ctwo{9.968e+04}, 2e+05& \ctwo{9.968e+04}, 2e+05& \ctwo{9.968e+04}, 2e+05& \cone{0.000e+00}, 4e+04\\
 \hline
w1a-2477-300 &9.3e+05& 50 & \ctwo{1.034e+08}, 4e+07& 1.280e+09, 4e+08& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cone{0.000e+00}, 4e+05\\
TDT2-500-1000 &2.6e+07& 50 & 1.433e+14, 6e+14& 2.885e+13, 5e+13& 4.064e+10, 1e+12& 1.995e+09, 3e+09& \cthree{1.214e+09}, 4e+09& \cone{0.000e+00}, 1e+08& \ctwo{6.745e+07}, 6e+08\\
20News-8000-1000 &3.1e+10& 50 & 6.006e+14, 3e+15& 1.569e+15, 3e+13& 4.089e+09, 2e+11& \cthree{3.492e+09}, 8e+09& \ctwo{7.238e+08}, 3e+09& \cone{0.000e+00}, 4e+08& 5.729e+09, 8e+09\\
sector-6412-1000 &3.8e+07& 50 & 1.352e+17, 9e+17& 2.950e+17, 4e+11& 4.159e+17, 2e+18& \cthree{6.185e+09}, 4e+09& 9.221e+09, 3e+11& \ctwo{3.945e+08}, 9e+11& \cone{0.000e+00}, 2e+12\\
E2006-2000-1000 &1.2e+03& 50 & 6.760e+14, 2e+15& 6.144e+15, 1e+14& 1.097e+08, 8e+08& 2.023e+07, 5e+09& \cthree{9.152e+06}, 1e+08& \ctwo{9.022e+06}, 1e+08& \cone{0.000e+00}, 6e+05\\
MNIST-60000-784 &8.3e+04& 50 & 8.237e+12, 8e+12& 1.431e+13, 7e+09& 2.563e+07, 6e+08& 2.213e+07, 5e+07& \ctwo{2.045e+07}, 4e+07& \cthree{2.078e+07}, 4e+07& \cone{0.000e+00}, 3e+05\\
Gisette-3000-1000 &2.8e+05& 50 & \ctwo{8.235e+06}, 3e+07& 2.937e+09, 2e+10& \cthree{2.997e+07}, 3e+07& 3.033e+07, 4e+07& 3.022e+07, 3e+07& 3.970e+07, 4e+07& \cone{0.000e+00}, 3e+05\\
CnnCaltech-3000-1000 &1.4e+05& 50 & \cthree{2.455e+06}, 1e+07& 2.968e+06, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \cone{0.000e+00}, 6e+04\\
Cifar-1000-1000 &3.0e+06& 50 & 9.414e+11, 2e+13& 1.791e+09, 7e+09& 4.126e+08, 1e+09& 6.530e+06, 1e+08& \cthree{3.729e+06}, 1e+09& \cone{0.000e+00}, 8e+08& \ctwo{2.213e+06}, 9e+07\\
randn-500-1000 &9.3e+04& 50 & 6.432e+05, 6e+05& 6.778e+05, 6e+05& \ctwo{6.091e+05}, 6e+05& \ctwo{6.091e+05}, 6e+05& \ctwo{6.091e+05}, 6e+05& \cthree{6.187e+05}, 6e+05& \cone{0.000e+00}, 1e+05\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=30} \\ \hline
w1a-2477-300 &4.5e+03& 10 & 7.536e+06, 1e+07& \ctwo{6.164e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cone{0.000e+00}, 3e+04\\
TDT2-500-1000 &1.1e+06& 10 & 7.867e+14, 2e+15& 2.353e+11, 2e+11& 2.089e+09, 2e+09& 3.709e+07, 2e+08& \cthree{1.399e+07}, 9e+07& \ctwo{4.756e+06}, 4e+07& \cone{0.000e+00}, 2e+07\\
20News-8000-1000 &1.5e+07& 10 & 1.883e+15, 3e+15& 1.806e+14, 3e+08& 6.430e+09, 1e+10& \cthree{5.718e+08}, 1e+09& 7.112e+08, 2e+10& \cone{0.000e+00}, 1e+08& \ctwo{1.434e+08}, 3e+08\\
sector-6412-1000 &3.9e+05& 10 & 3.004e+17, 6e+17& 2.950e+17, 1e+10& 1.969e+18, 3e+18& \cthree{1.355e+08}, 9e+10& 3.637e+09, 2e+10& \ctwo{2.656e+07}, 6e+10& \cone{0.000e+00}, 2e+11\\
E2006-2000-1000 &1.0e+02& 10 & 7.927e+12, 2e+14& 1.501e+15, 2e+08& 5.255e+06, 1e+08& 2.753e+06, 6e+07& \ctwo{2.717e+06}, 6e+07& \cthree{2.752e+06}, 6e+07& \cone{0.000e+00}, 6e+04\\
MNIST-60000-784 &5.2e+03& 10 & 4.121e+08, 8e+08& 1.312e+13, 9e+07& \ctwo{2.610e+06}, 1e+07& 2.743e+06, 1e+07& \cthree{2.742e+06}, 1e+07& \cthree{2.742e+06}, 1e+07& \cone{0.000e+00}, 4e+04\\
Gisette-3000-1000 &3.1e+04& 10 & 3.248e+06, 2e+07& 9.758e+06, 8e+08& 2.990e+06, 8e+06& \ctwo{2.971e+06}, 8e+06& 2.977e+06, 8e+06& \cthree{2.975e+06}, 8e+06& \cone{0.000e+00}, 8e+04\\
CnnCaltech-3000-1000 &6.5e+03& 10 & \cthree{9.057e+05}, 4e+06& 1.047e+06, 6e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &3.8e+05& 10 & 1.126e+13, 5e+13& 1.525e+09, 2e+09& 2.633e+07, 8e+07& 2.131e+06, 8e+07& \cthree{1.603e+06}, 5e+08& \ctwo{5.086e+05}, 1e+07& \cone{0.000e+00}, 7e+06\\
randn-500-1000 &1.0e+04& 10 & 2.875e+04, 6e+04& 3.612e+04, 7e+04& \cthree{2.406e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \cone{0.000e+00}, 2e+04\\
 \hline
w1a-2477-300 &1.5e+05& 20 & 2.042e+07, 2e+07& \ctwo{2.156e+06}, 3e+06& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cone{0.000e+00}, 2e+05\\
TDT2-500-1000 &6.2e+06& 20 & 2.734e+13, 2e+14& 1.674e+12, 2e+12& 5.782e+09, 9e+09& \cthree{8.629e+07}, 3e+08& 1.345e+08, 4e+08& \ctwo{5.502e+06}, 7e+07& \cone{0.000e+00}, 8e+07\\
20News-8000-1000 &6.6e+08& 20 & 8.388e+13, 9e+14& 9.134e+14, 3e+08& 5.325e+11, 4e+11& 2.995e+09, 2e+09& \cthree{2.760e+09}, 2e+09& \cone{0.000e+00}, 1e+08& \ctwo{8.945e+08}, 1e+09\\
sector-6412-1000 &2.3e+06& 20 & 5.014e+17, 1e+18& 2.950e+17, 2e+11& 8.719e+17, 2e+18& \cthree{1.649e+09}, 4e+09& 4.498e+09, 3e+09& \ctwo{5.954e+07}, 4e+11& \cone{0.000e+00}, 5e+11\\
E2006-2000-1000 &7.5e+01& 20 & 5.457e+13, 5e+14& 1.841e+15, 4e+08& 4.168e+07, 3e+08& \cthree{4.663e+06}, 1e+08& 4.974e+06, 6e+08& \ctwo{4.645e+06}, 9e+07& \cone{0.000e+00}, 9e+04\\
MNIST-60000-784 &1.2e+04& 20 & 2.670e+11, 2e+11& 1.418e+13, 4e+10& 7.361e+06, 7e+08& 6.584e+06, 2e+07& \ctwo{6.436e+06}, 2e+07& \cthree{6.570e+06}, 2e+07& \cone{0.000e+00}, 6e+04\\
Gisette-3000-1000 &8.0e+04& 20 & \ctwo{4.321e+06}, 3e+07& 1.623e+07, 7e+07& 7.768e+06, 1e+07& \cthree{7.722e+06}, 1e+07& 7.795e+06, 1e+07& 8.162e+06, 1e+07& \cone{0.000e+00}, 1e+05\\
CnnCaltech-3000-1000 &2.3e+04& 20 & \cthree{1.335e+06}, 6e+06& 2.394e+06, 1e+07& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &8.0e+05& 20 & 5.981e+12, 7e+13& 1.959e+08, 1e+09& 6.383e+07, 2e+08& 2.111e+06, 1e+08& \cthree{1.943e+06}, 3e+07& \ctwo{4.714e+05}, 4e+07& \cone{0.000e+00}, 2e+07\\
randn-500-1000 &2.6e+04& 20 & \cthree{1.061e+05}, 2e+05& 1.174e+05, 2e+05& \ctwo{9.944e+04}, 2e+05& \ctwo{9.944e+04}, 2e+05& \ctwo{9.944e+04}, 2e+05& \ctwo{9.944e+04}, 2e+05& \cone{0.000e+00}, 4e+04\\
 \hline
w1a-2477-300 &9.3e+05& 50 & \ctwo{1.034e+08}, 4e+07& 1.280e+09, 4e+08& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cone{0.000e+00}, 4e+05\\
TDT2-500-1000 &2.6e+07& 50 & 1.433e+14, 6e+14& 2.885e+13, 5e+13& 4.064e+10, 1e+12& 1.996e+09, 3e+09& \cthree{1.214e+09}, 4e+09& \cone{0.000e+00}, 1e+08& \ctwo{3.095e+07}, 4e+08\\
20News-8000-1000 &3.1e+10& 50 & 6.006e+14, 3e+15& 1.569e+15, 3e+13& 4.094e+09, 2e+11& \cthree{3.498e+09}, 8e+09& \ctwo{7.292e+08}, 3e+09& \cone{0.000e+00}, 3e+08& 3.969e+09, 7e+09\\
sector-6412-1000 &1.6e+07& 50 & 1.352e+17, 9e+17& 2.950e+17, 4e+11& 4.159e+17, 2e+18& \cthree{6.207e+09}, 4e+09& 9.243e+09, 3e+11& \ctwo{3.276e+08}, 1e+12& \cone{0.000e+00}, 2e+12\\
E2006-2000-1000 &-1.3e+02& 50 & 6.760e+14, 2e+15& 6.144e+15, 1e+14& 1.097e+08, 8e+08& 2.024e+07, 5e+09& \cthree{9.154e+06}, 1e+08& \ctwo{9.023e+06}, 1e+08& \cone{0.000e+00}, 2e+05\\
MNIST-60000-784 &6.1e+04& 50 & 8.237e+12, 8e+12& 1.431e+13, 7e+09& 2.565e+07, 6e+08& 2.215e+07, 5e+07& \ctwo{2.047e+07}, 4e+07& \cthree{2.080e+07}, 4e+07& \cone{0.000e+00}, 2e+05\\
Gisette-3000-1000 &2.7e+05& 50 & \ctwo{8.247e+06}, 3e+07& 2.937e+09, 2e+10& \cthree{2.998e+07}, 3e+07& 3.034e+07, 4e+07& 3.023e+07, 3e+07& 3.939e+07, 4e+07& \cone{0.000e+00}, 3e+05\\
CnnCaltech-3000-1000 &1.4e+05& 50 & \cthree{2.455e+06}, 1e+07& 2.968e+06, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \ctwo{2.387e+06}, 1e+07& \cone{0.000e+00}, 5e+04\\
Cifar-1000-1000 &2.5e+06& 50 & 9.414e+11, 2e+13& 1.792e+09, 7e+09& 4.131e+08, 1e+09& 6.992e+06, 1e+08& \cthree{4.190e+06}, 1e+09& \cone{0.000e+00}, 1e+08& \ctwo{1.100e+06}, 5e+07\\
randn-500-1000 &8.9e+04& 50 & 6.471e+05, 6e+05& 6.817e+05, 6e+05& \ctwo{6.130e+05}, 6e+05& \ctwo{6.130e+05}, 6e+05& \ctwo{6.130e+05}, 6e+05& \cthree{6.161e+05}, 6e+05& \cone{0.000e+00}, 1e+05\\
 \hline
 \hline \multicolumn{10}{|c|}{\centering $\lambda$ = 1000.00, time limit=50} \\ \hline
w1a-2477-300 &4.5e+03& 10 & 7.536e+06, 1e+07& \ctwo{6.164e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cthree{7.202e+06}, 1e+07& \cone{0.000e+00}, 3e+04\\
TDT2-500-1000 &3.6e+05& 10 & 7.867e+14, 2e+15& 2.353e+11, 2e+11& 2.089e+09, 2e+09& 3.780e+07, 2e+08& \cthree{1.470e+07}, 9e+07& \ctwo{5.465e+06}, 4e+07& \cone{0.000e+00}, 1e+07\\
20News-8000-1000 &1.5e+07& 10 & 1.883e+15, 3e+15& 1.806e+14, 3e+08& 6.430e+09, 1e+10& \cthree{5.718e+08}, 1e+09& 7.112e+08, 2e+10& \cone{0.000e+00}, 1e+08& \ctwo{3.432e+07}, 2e+08\\
sector-6412-1000 &3.9e+05& 10 & 3.004e+17, 6e+17& 2.950e+17, 1e+10& 1.969e+18, 3e+18& \cthree{1.355e+08}, 9e+10& 3.637e+09, 2e+10& \ctwo{2.667e+07}, 6e+10& \cone{0.000e+00}, 3e+11\\
E2006-2000-1000 &1.0e+02& 10 & 7.927e+12, 2e+14& 1.501e+15, 2e+08& 5.255e+06, 1e+08& 2.753e+06, 6e+07& \ctwo{2.717e+06}, 6e+07& \cthree{2.752e+06}, 6e+07& \cone{0.000e+00}, 6e+04\\
MNIST-60000-784 &5.2e+03& 10 & 4.121e+08, 8e+08& 1.312e+13, 9e+07& \ctwo{2.611e+06}, 1e+07& 2.743e+06, 1e+07& \cthree{2.742e+06}, 1e+07& \cthree{2.742e+06}, 1e+07& \cone{0.000e+00}, 4e+04\\
Gisette-3000-1000 &3.0e+04& 10 & 3.249e+06, 2e+07& 9.759e+06, 8e+08& 2.991e+06, 8e+06& \cthree{2.972e+06}, 8e+06& 2.978e+06, 8e+06& \ctwo{2.968e+06}, 8e+06& \cone{0.000e+00}, 8e+04\\
CnnCaltech-3000-1000 &6.5e+03& 10 & \cthree{9.057e+05}, 4e+06& 1.047e+06, 6e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \ctwo{8.594e+05}, 4e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &2.6e+05& 10 & 1.126e+13, 5e+13& 1.526e+09, 2e+09& 2.645e+07, 8e+07& 2.257e+06, 8e+07& \cthree{1.728e+06}, 5e+08& \ctwo{6.165e+05}, 1e+07& \cone{0.000e+00}, 3e+06\\
randn-500-1000 &1.0e+04& 10 & 2.875e+04, 6e+04& 3.612e+04, 7e+04& \cthree{2.406e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \ctwo{2.405e+04}, 7e+04& \cone{0.000e+00}, 2e+04\\
 \hline
w1a-2477-300 &1.5e+05& 20 & 2.042e+07, 2e+07& \ctwo{2.156e+06}, 3e+06& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cthree{2.010e+07}, 2e+07& \cone{0.000e+00}, 2e+05\\
TDT2-500-1000 &2.2e+06& 20 & 2.734e+13, 2e+14& 1.674e+12, 2e+12& 5.786e+09, 9e+09& \cthree{9.023e+07}, 3e+08& 1.384e+08, 4e+08& \ctwo{9.447e+06}, 7e+07& \cone{0.000e+00}, 6e+07\\
20News-8000-1000 &6.6e+08& 20 & 8.388e+13, 9e+14& 9.134e+14, 3e+08& 5.325e+11, 4e+11& 2.995e+09, 2e+09& \cthree{2.761e+09}, 2e+09& \cone{0.000e+00}, 1e+08& \ctwo{3.539e+08}, 6e+08\\
sector-6412-1000 &2.2e+06& 20 & 5.014e+17, 1e+18& 2.950e+17, 2e+11& 8.719e+17, 2e+18& \cthree{1.649e+09}, 4e+09& 4.498e+09, 3e+09& \ctwo{5.679e+07}, 4e+11& \cone{0.000e+00}, 7e+11\\
E2006-2000-1000 &7.5e+01& 20 & 5.457e+13, 5e+14& 1.841e+15, 4e+08& 4.168e+07, 3e+08& \cthree{4.663e+06}, 1e+08& 4.974e+06, 6e+08& \ctwo{4.645e+06}, 9e+07& \cone{0.000e+00}, 9e+04\\
MNIST-60000-784 &1.1e+04& 20 & 2.670e+11, 2e+11& 1.418e+13, 4e+10& 7.363e+06, 7e+08& 6.586e+06, 2e+07& \ctwo{6.438e+06}, 2e+07& \cthree{6.571e+06}, 2e+07& \cone{0.000e+00}, 6e+04\\
Gisette-3000-1000 &7.9e+04& 20 & \ctwo{4.322e+06}, 3e+07& 1.623e+07, 7e+07& 7.769e+06, 1e+07& \cthree{7.723e+06}, 1e+07& 7.796e+06, 1e+07& 7.798e+06, 1e+07& \cone{0.000e+00}, 1e+05\\
CnnCaltech-3000-1000 &2.3e+04& 20 & \cthree{1.335e+06}, 6e+06& 2.394e+06, 1e+07& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \ctwo{1.324e+06}, 6e+06& \cone{0.000e+00}, 3e+04\\
Cifar-1000-1000 &5.2e+05& 20 & 5.981e+12, 7e+13& 1.962e+08, 1e+09& 6.411e+07, 2e+08& 2.391e+06, 1e+08& \cthree{2.224e+06}, 3e+07& \ctwo{5.409e+05}, 1e+08& \cone{0.000e+00}, 6e+06\\
randn-500-1000 &2.6e+04& 20 & \cthree{1.064e+05}, 2e+05& 1.177e+05, 2e+05& \ctwo{9.969e+04}, 2e+05& \ctwo{9.969e+04}, 2e+05& \ctwo{9.969e+04}, 2e+05& \ctwo{9.969e+04}, 2e+05& \cone{0.000e+00}, 4e+04\\
 \hline
w1a-2477-300 &9.3e+05& 50 & \ctwo{1.034e+08}, 4e+07& 1.280e+09, 4e+08& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cthree{1.061e+08}, 4e+07& \cone{0.000e+00}, 4e+05\\
TDT2-500-1000 &2.6e+07& 50 & 1.433e+14, 6e+14& 2.885e+13, 5e+13& 4.064e+10, 1e+12& 1.996e+09, 3e+09& \cthree{1.214e+09}, 4e+09& \cone{0.000e+00}, 1e+08& \ctwo{9.137e+05}, 3e+08\\
20News-8000-1000 &3.1e+10& 50 & 6.006e+14, 3e+15& 1.569e+15, 3e+13& 4.097e+09, 2e+11& 3.500e+09, 8e+09& \ctwo{7.316e+08}, 3e+09& \cone{0.000e+00}, 3e+08& \cthree{2.003e+09}, 5e+09\\
sector-6412-1000 &9.6e+06& 50 & 1.352e+17, 9e+17& 2.950e+17, 4e+11& 4.159e+17, 2e+18& \cthree{6.214e+09}, 4e+09& 9.250e+09, 3e+11& \ctwo{2.769e+08}, 1e+12& \cone{0.000e+00}, 2e+12\\
E2006-2000-1000 &-1.5e+02& 50 & 6.760e+14, 2e+15& 6.144e+15, 1e+14& 1.097e+08, 8e+08& 2.024e+07, 5e+09& \cthree{9.154e+06}, 1e+08& \ctwo{9.023e+06}, 1e+08& \cone{0.000e+00}, 1e+05\\
MNIST-60000-784 &4.7e+04& 50 & 8.237e+12, 8e+12& 1.431e+13, 7e+09& 2.566e+07, 6e+08& 2.217e+07, 5e+07& \ctwo{2.049e+07}, 4e+07& \cthree{2.077e+07}, 4e+07& \cone{0.000e+00}, 1e+05\\
Gisette-3000-1000 &2.6e+05& 50 & \ctwo{8.255e+06}, 3e+07& 2.937e+09, 2e+10& \cthree{2.999e+07}, 3e+07& 3.035e+07, 4e+07& 3.024e+07, 3e+07& 3.640e+07, 3e+07& \cone{0.000e+00}, 3e+05\\
CnnCaltech-3000-1000 &1.4e+05& 50 & \cthree{2.456e+06}, 1e+07& 2.969e+06, 1e+07& \ctwo{2.388e+06}, 1e+07& \ctwo{2.388e+06}, 1e+07& \ctwo{2.388e+06}, 1e+07& \ctwo{2.388e+06}, 1e+07& \cone{0.000e+00}, 4e+04\\
Cifar-1000-1000 &2.2e+06& 50 & 9.414e+11, 2e+13& 1.792e+09, 7e+09& 4.134e+08, 1e+09& 7.301e+06, 1e+08& \cthree{4.499e+06}, 1e+09& \cone{0.000e+00}, 2e+08& \ctwo{3.010e+05}, 3e+07\\
randn-500-1000 &8.7e+04& 50 & 6.499e+05, 6e+05& 6.845e+05, 6e+05& \ctwo{6.158e+05}, 6e+05& \ctwo{6.158e+05}, 6e+05& \ctwo{6.158e+05}, 6e+05& \cthree{6.163e+05}, 6e+05& \cone{0.000e+00}, 1e+05\\
\hline
\end{tabular}}
\caption{Comparisons of objective values and Riemannian gradient residuals $(F(\X)-F_{\text{min}}, \| \G^t - \X^t [\G^t]\trans \X^t \|_{\fro})$ for nonlinear eigenvalue problems for all the compared methods with $\lambda=10000$. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively.}
\label{tab:nlevp:3}
\end{table*}


==> L1PCA/NNPCA.tex <==









\begin{table*}[!h]
\centering
\scalebox{0.5}{\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
  \hline
 \multirow{2}*{data-m-n}   & \multirow{2}*{$F_{\text{min}}$}   & \multirow{2}*{r} & \multirow{2}*{LADMM}  &  \multirow{2}*{PADM}  & \multirow{2}*{ODBC-R} & \multirow{2}*{ODBC-SV} &\multirow{2}*{ODBC-OR} & LADMM   & PADM \\
      &   & &    &   &  &    &   &  + ODBC-R   & +{ODBC-R}  \\
        \hline  \hline
\multicolumn{10}{|c|}{\centering time limit=10} \\ \hline
w1a-2477-300 & -5.2e+03 & 10 & 5.14e+02, 2e-13& 1.29e+03, 1e-05& 2.77e+02, 6e-14& 5.00e+02, 2e-14& \ctwo{1.77e+02}, 2e-14& \cone{0.00e+00}, 2e-13\cone{(+)}& \cthree{1.93e+02}, 1e-05\cone{(+)}\\
TDT2-500-1000 & -3.5e+00 & 10 & 9.22e-01, 1e-14& 9.39e-01, 5e-05& 1.59e+00, 1e-14& \cone{0.00e+00}, 3e-14& \ctwo{2.67e-02}, 3e-14& \cthree{6.50e-01}, 4e-14\cone{(+)}& 6.56e-01, 5e-05\cone{(+)}\\
20News-8000-1000 & -1.5e+00 & 10 & 5.03e-01, 4e-14& 5.16e-01, 1e-04& 8.90e-01, 9e-14& \cone{0.00e+00}, 5e-14& \ctwo{7.71e-03}, 4e-14& \cthree{2.87e-01}, 1e-13\cone{(+)}& 3.46e-01, 1e-04\cone{(+)}\\
sector-6412-1000 & -3.4e+01 & 10 & 2.03e+00, 2e-08& 2.28e+00, 3e-04& 1.52e+01, 7e-14& \cone{0.00e+00}, 5e-14& \ctwo{6.37e-02}, 5e-14& \cthree{1.03e+00}, 2e-08\cone{(+)}& 1.13e+00, 3e-04\cone{(+)}\\
E2006-2000-1000 & -6.2e-01 & 10 & 1.18e-01, 4e-15& 1.20e-01, 6e-05& 4.19e-01, 2e-14& \cone{0.00e+00}, 1e-13& \ctwo{2.68e-05}, 6e-14& \cthree{8.37e-02}, 4e-14\cone{(+)}& 1.01e-01, 6e-05\cone{(+)}\\
MNIST-60000-784 & -2.5e+05 & 10 & 4.23e+04, 9e-10& 6.51e+04, 5e-04& \ctwo{5.98e+02}, 7e-15& 4.60e+03, 2e-15& \cthree{3.83e+03}, 1e-15& \cone{0.00e+00}, 9e-10\cone{(+)}& 2.14e+04, 5e-04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & 4.55e+04, 8e-10& 3.89e+04, 7e-04& \cone{0.00e+00}, 6e-15& \ctwo{3.18e+03}, 2e-15& \cthree{3.64e+03}, 2e-15& 7.47e+03, 8e-10\cone{(+)}& 4.05e+03, 7e-04\cone{(+)}\\
CnnCaltech-3000-1000 & -3.4e+03 & 10 & 9.82e+02, 1e-14& 7.56e+02, 5e-04& \cone{0.00e+00}, 6e-15& \ctwo{8.11e+01}, 2e-15& \cthree{1.09e+02}, 2e-15& 4.91e+02, 4e-14\cone{(+)}& 1.89e+02, 5e-04\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 1.63e+04, 2e-09& 2.27e+04, 6e-04& \cone{0.00e+00}, 5e-15& \cthree{4.17e+02}, 2e-15& \ctwo{3.73e+02}, 2e-15& 9.84e+03, 2e-09\cone{(+)}& 4.20e+03, 6e-04\cone{(+)}\\
randn-500-1000 & -6.8e+03 & 10 & 6.38e+02, 2e-11& \cthree{2.80e+02}, 5e-04& 3.05e+02, 6e-15& 5.60e+02, 2e-15& 5.50e+02, 4e-15& \ctwo{2.68e+02}, 2e-11\cone{(+)}& \cone{0.00e+00}, 5e-04\cone{(+)}\\
 \hline
w1a-2477-300 & -6.6e+03 & 20 & 1.94e+03, 1e-12& 2.62e+03, 4e-05& 3.13e+02, 5e-14& \ctwo{1.85e+02}, 2e-14& \cthree{2.96e+02}, 7e-15& \cone{0.00e+00}, 1e-12\cone{(+)}& 4.21e+02, 4e-05\cone{(+)}\\
TDT2-500-1000 & -3.9e+00 & 20 & 1.04e+00, 2e-08& 1.05e+00, 3e-04& 1.65e+00, 8e-15& \cone{0.00e+00}, 2e-14& \ctwo{5.94e-02}, 1e-14& \cthree{6.78e-01}, 2e-08\cone{(+)}& 7.34e-01, 3e-04\cone{(+)}\\
20News-8000-1000 & -1.7e+00 & 20 & 6.52e-01, 3e-08& 6.68e-01, 7e-05& 7.88e-01, 5e-14& \cone{0.00e+00}, 5e-14& \ctwo{5.28e-02}, 3e-14& \cthree{4.56e-01}, 3e-08\cone{(+)}& 5.13e-01, 7e-05\cone{(+)}\\
sector-6412-1000 & -4.6e+01 & 20 & 4.84e+00, 1e-07& 4.86e+00, 7e-04& 2.03e+01, 5e-14& \cone{0.00e+00}, 5e-14& \ctwo{3.92e-01}, 3e-14& \cthree{2.11e+00}, 1e-07\cone{(+)}& 2.43e+00, 7e-04\cone{(+)}\\
E2006-2000-1000 & -6.5e-01 & 20 & 1.42e-01, 7e-15& 1.45e-01, 9e-05& 3.17e-01, 1e-14& \cone{0.00e+00}, 5e-14& \ctwo{5.53e-04}, 2e-14& \cthree{1.00e-01}, 2e-14\cone{(+)}& 1.22e-01, 9e-05\cone{(+)}\\
MNIST-60000-784 & -2.7e+05 & 20 & 6.64e+04, 7e-12& 2.49e+05, 6e-04& \cone{0.00e+00}, 5e-15& \ctwo{2.51e+03}, 1e-15& \cthree{3.92e+03}, 1e-15& 4.75e+04, 7e-12\cone{(+)}& 1.13e+04, 6e-04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 20 & 2.22e+05, 1e-08& 3.51e+04, 1e-03& \cone{0.00e+00}, 3e-15& \cthree{8.37e+03}, 1e-15& 1.09e+04, 7e-16& 5.96e+04, 1e-08\cone{(+)}& \ctwo{8.33e+03}, 1e-03\cone{(+)}\\
CnnCaltech-3000-1000 & -3.6e+03 & 20 & 1.43e+03, 4e-12& 1.30e+03, 1e-03& \cone{0.00e+00}, 3e-15& \ctwo{1.28e+02}, 1e-15& \cthree{1.40e+02}, 1e-15& 4.13e+02, 4e-12\cone{(+)}& 3.26e+02, 1e-03\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 2.74e+04, 3e-09& 5.00e+04, 2e-03& \cone{0.00e+00}, 3e-15& \cthree{6.34e+02}, 8e-16& \ctwo{5.78e+02}, 8e-16& 1.62e+04, 3e-09\cone{(+)}& 1.41e+04, 2e-03\cone{(+)}\\
randn-500-1000 & -1.1e+04 & 20 & 6.96e+02, 2e-10& 5.08e+02, 1e-03& \ctwo{1.92e+02}, 4e-15& 9.19e+02, 9e-16& 9.03e+02, 1e-15& \cthree{3.62e+02}, 2e-10\cone{(+)}& \cone{0.00e+00}, 1e-03\cone{(+)}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 6.69e+03, 1e-07& 8.92e+03, 9e-04& 7.44e+01, 3e-14& 1.18e+02, 2e-14& \cone{0.00e+00}, 7e-15& \ctwo{1.12e+01}, 1e-07\cone{(+)}& \cthree{3.96e+01}, 9e-04\cone{(+)}\\
TDT2-500-1000 & -4.5e+00 & 100 & 1.25e+00, 3e-05& 1.29e+00, 2e-04& 1.96e+00, 1e-15& \cone{0.00e+00}, 5e-15& \ctwo{2.09e-01}, 4e-15& \cthree{1.01e+00}, 3e-05\cone{(+)}& 1.06e+00, 2e-04\cone{(+)}\\
20News-8000-1000 & -1.9e+00 & 100 & 5.92e-01, 2e-05& 6.01e-01, 2e-04& 9.31e-01, 3e-15& \cone{0.00e+00}, 4e-15& \ctwo{1.29e-02}, 8e-15& \cthree{4.90e-01}, 2e-05\cone{(+)}& 5.11e-01, 2e-04\cone{(+)}\\
sector-6412-1000 & -8.5e+01 & 100 & 1.41e+01, 1e-04& 2.59e+01, 5e-03& 4.80e+01, 7e-15& \cone{0.00e+00}, 2e-14& \ctwo{2.31e+00}, 1e-14& \cthree{9.98e+00}, 1e-04\cone{(+)}& 1.03e+01, 5e-03\cone{(+)}\\
E2006-2000-1000 & -6.9e-01 & 100 & 1.63e-01, 3e-07& 1.66e-01, 4e-06& 3.64e-01, 2e-15& \cone{0.00e+00}, 1e-14& \ctwo{2.41e-03}, 1e-14& \cthree{1.42e-01}, 3e-07\cone{(+)}& \cthree{1.42e-01}, 4e-06\cone{(+)}\\
MNIST-60000-784 & -3.3e+05 & 100 & 1.45e+05, 3e-06& 3.20e+05, 2e-03& 1.72e+04, 2e-15& \cone{0.00e+00}, 2e-15& \cthree{2.59e+03}, 2e-15& 3.88e+04, 3e-06\cone{(+)}& \ctwo{1.74e+03}, 2e-03\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 8.19e+05, 5e-06& 5.37e+05, 3e-02& \cone{0.00e+00}, 2e-15& \ctwo{2.62e+04}, 1e-15& \cthree{2.74e+04}, 8e-16& 5.68e+05, 5e-06\cone{(+)}& 3.18e+05, 3e-02\cone{(+)}\\
CnnCaltech-3000-1000 & -4.5e+03 & 100 & 3.28e+03, 8e-05& 2.02e+03, 2e-02& \cone{0.00e+00}, 2e-15& \ctwo{1.33e+02}, 1e-15& \cthree{1.74e+02}, 1e-15& 1.91e+03, 8e-05\cone{(+)}& 5.63e+02, 2e-02\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 100 & 1.18e+05, 3e-05& 4.92e+04, 3e-02& \cone{0.00e+00}, 2e-15& \ctwo{2.78e+02}, 9e-16& \cthree{1.26e+03}, 1e-15& 5.10e+04, 3e-05\cone{(+)}& 3.77e+04, 3e-02\cone{(+)}\\
randn-500-1000 & -3.4e+04 & 100 & 4.75e+03, 5e-05& 1.63e+03, 2e-02& \ctwo{2.83e+02}, 2e-15& \cthree{6.24e+02}, 1e-15& \cone{0.00e+00}, 1e-15& 2.82e+03, 5e-05\cone{(+)}& 8.40e+02, 2e-02\cone{(+)}\\
 \hline
 \hline   \multicolumn{10}{|c|}{\centering time limit=30} \\ \hline
w1a-2477-300 & -5.2e+03 & 10 & 5.14e+02, 2e-13& 1.28e+03, 1e-05& 2.77e+02, 1e-13& 4.96e+02, 4e-14& \cthree{1.61e+02}, 4e-14& \cone{0.00e+00}, 2e-13\cone{(+)}& \ctwo{1.45e+02}, 1e-05\cone{(+)}\\
TDT2-500-1000 & -3.5e+00 & 10 & 9.22e-01, 1e-14& 9.39e-01, 3e-05& \cthree{6.60e-01}, 6e-14& \cone{0.00e+00}, 4e-14& \ctwo{2.65e-02}, 3e-14& 6.70e-01, 4e-14\cone{(+)}& 6.98e-01, 3e-05\cone{(+)}\\
20News-8000-1000 & -1.6e+00 & 10 & 5.09e-01, 2e-14& 5.22e-01, 1e-05& 3.08e-01, 1e-13& \ctwo{6.47e-03}, 8e-14& \cone{0.00e+00}, 6e-14& \cthree{2.84e-01}, 1e-13\cone{(+)}& 3.25e-01, 1e-05\cone{(+)}\\
sector-6412-1000 & -3.4e+01 & 10 & 2.04e+00, 1e-11& 2.29e+00, 1e-04& 4.46e+00, 1e-13& \cone{0.00e+00}, 9e-14& \ctwo{6.42e-02}, 6e-14& 1.09e+00, 1e-11\cone{(+)}& \cthree{1.04e+00}, 1e-04\cone{(+)}\\
E2006-2000-1000 & -6.2e-01 & 10 & 1.18e-01, 3e-15& 1.20e-01, 2e-05& 1.15e-01, 6e-14& \cone{0.00e+00}, 2e-13& \ctwo{2.68e-05}, 6e-14& \cthree{8.32e-02}, 3e-14\cone{(+)}& 9.95e-02, 2e-05\cone{(+)}\\
MNIST-60000-784 & -2.5e+05 & 10 & 4.47e+04, 6e-10& 6.46e+04, 3e-04& \cone{0.00e+00}, 3e-14& \cthree{5.73e+02}, 1e-14& \ctwo{5.11e+02}, 4e-15& 3.82e+03, 6e-10\cone{(+)}& 2.49e+04, 3e-04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & 4.49e+04, 9e-10& 3.32e+04, 5e-04& \cone{0.00e+00}, 2e-14& \ctwo{1.04e+03}, 4e-15& \cthree{1.09e+03}, 4e-15& 6.41e+03, 9e-10\cone{(+)}& 4.03e+03, 5e-04\cone{(+)}\\
CnnCaltech-3000-1000 & -3.4e+03 & 10 & 1.01e+03, 1e-14& 7.85e+02, 1e-04& \cone{0.00e+00}, 2e-14& \ctwo{1.75e+01}, 5e-15& \cthree{6.63e+01}, 4e-15& 4.70e+02, 3e-14\cone{(+)}& 2.05e+02, 1e-04\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 1.61e+04, 2e-09& 2.09e+04, 3e-04& \cone{0.00e+00}, 2e-14& \cthree{1.48e+02}, 5e-15& \ctwo{6.74e+01}, 4e-15& 9.37e+03, 2e-09\cone{(+)}& 3.27e+03, 3e-04\cone{(+)}\\
randn-500-1000 & -6.8e+03 & 10 & 6.34e+02, 2e-11& 2.82e+02, 1e-04& \ctwo{6.97e+01}, 2e-14& 2.66e+02, 6e-15& 2.74e+02, 7e-15& \cthree{2.23e+02}, 2e-11\cone{(+)}& \cone{0.00e+00}, 1e-04\cone{(+)}\\
 \hline
w1a-2477-300 & -6.6e+03 & 20 & 1.95e+03, 1e-12& 2.63e+03, 2e-05& 3.10e+02, 1e-13& \ctwo{1.65e+02}, 3e-14& \cthree{2.73e+02}, 2e-14& \cone{0.00e+00}, 1e-12\cone{(+)}& 3.42e+02, 2e-05\cone{(+)}\\
TDT2-500-1000 & -3.9e+00 & 20 & 1.04e+00, 8e-14& 1.06e+00, 6e-05& 7.34e-01, 4e-14& \cone{0.00e+00}, 3e-14& \ctwo{9.44e-03}, 3e-14& \cthree{6.71e-01}, 1e-13\cone{(+)}& 7.16e-01, 6e-05\cone{(+)}\\
20News-8000-1000 & -1.7e+00 & 20 & 6.52e-01, 1e-13& 6.69e-01, 1e-05& \cthree{3.75e-01}, 1e-13& \cone{0.00e+00}, 5e-14& \ctwo{5.20e-02}, 5e-14& 4.58e-01, 2e-13\cone{(+)}& 5.01e-01, 1e-05\cone{(+)}\\
sector-6412-1000 & -4.6e+01 & 20 & 4.86e+00, 6e-09& 4.89e+00, 2e-04& 7.49e+00, 1e-13& \cone{0.00e+00}, 6e-14& \ctwo{4.06e-01}, 4e-14& \cthree{2.13e+00}, 6e-09\cone{(+)}& 2.59e+00, 2e-04\cone{(+)}\\
E2006-2000-1000 & -6.5e-01 & 20 & 1.42e-01, 8e-15& 1.45e-01, 4e-05& \cthree{2.48e-02}, 4e-14& \cone{0.00e+00}, 6e-14& \ctwo{5.54e-04}, 3e-14& 1.04e-01, 4e-14\cone{(+)}& 1.18e-01, 4e-05\cone{(+)}\\
MNIST-60000-784 & -2.7e+05 & 20 & 7.33e+04, 7e-12& 2.27e+05, 4e-04& \cone{0.00e+00}, 2e-14& \ctwo{2.19e+03}, 3e-15& \cthree{3.53e+03}, 3e-15& 5.49e+04, 7e-12\cone{(+)}& 1.73e+04, 4e-04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 20 & 2.11e+05, 8e-09& 3.36e+04, 8e-04& \cone{0.00e+00}, 9e-15& \ctwo{3.21e+03}, 2e-15& \cthree{4.36e+03}, 2e-15& 6.19e+04, 8e-09\cone{(+)}& 1.06e+04, 8e-04\cone{(+)}\\
CnnCaltech-3000-1000 & -3.7e+03 & 20 & 1.50e+03, 4e-12& 1.38e+03, 3e-04& \cone{0.00e+00}, 1e-14& \ctwo{4.37e+01}, 2e-15& \cthree{7.19e+01}, 2e-15& 4.98e+02, 4e-12\cone{(+)}& 3.24e+02, 3e-04\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 2.74e+04, 3e-09& 5.00e+04, 5e-04& \cone{0.00e+00}, 1e-14& \ctwo{3.07e+02}, 2e-15& \cthree{3.97e+02}, 2e-15& 1.65e+04, 3e-09\cone{(+)}& 9.86e+03, 5e-04\cone{(+)}\\
randn-500-1000 & -1.1e+04 & 20 & 8.52e+02, 2e-11& 6.83e+02, 3e-04& \cone{0.00e+00}, 1e-14& 5.34e+02, 3e-15& \cthree{4.87e+02}, 2e-15& 5.21e+02, 2e-11\cone{(+)}& \ctwo{1.80e+02}, 3e-04\cone{(+)}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 6.75e+03, 4e-09& 8.98e+03, 2e-04& \cthree{1.40e+01}, 3e-14& 1.47e+02, 2e-14& \cone{0.00e+00}, 9e-15& \ctwo{4.21e-02}, 4e-09\cone{(+)}& 8.87e+01, 2e-04\cone{(+)}\\
TDT2-500-1000 & -4.8e+00 & 100 & 1.50e+00, 3e-14& 1.53e+00, 7e-05& 1.62e+00, 2e-15& \cone{0.00e+00}, 9e-15& \ctwo{1.45e-02}, 8e-15& \cthree{1.23e+00}, 4e-14\cone{(+)}& 1.28e+00, 7e-05\cone{(+)}\\
20News-8000-1000 & -2.0e+00 & 100 & 7.14e-01, 2e-07& 7.23e-01, 7e-05& \cthree{3.83e-01}, 1e-14& \cone{0.00e+00}, 2e-14& \ctwo{6.30e-03}, 2e-14& 5.85e-01, 2e-07\cone{(+)}& 6.18e-01, 7e-05\cone{(+)}\\
sector-6412-1000 & -8.5e+01 & 100 & 1.49e+01, 6e-08& 2.67e+01, 2e-03& 3.17e+01, 3e-14& \cone{0.00e+00}, 4e-14& \ctwo{6.21e-02}, 2e-14& \cthree{9.81e+00}, 6e-08\cone{(+)}& 1.10e+01, 2e-03\cone{(+)}\\
E2006-2000-1000 & -6.9e-01 & 100 & 1.64e-01, 5e-14& 1.67e-01, 2e-06& \cthree{1.19e-01}, 3e-15& \cone{0.00e+00}, 4e-14& \ctwo{3.06e-04}, 4e-14& 1.42e-01, 5e-14\cone{(+)}& 1.45e-01, 2e-06\cone{(+)}\\
MNIST-60000-784 & -3.5e+05 & 100 & 1.60e+05, 3e-08& 3.39e+05, 6e-04& \cthree{7.01e+03}, 3e-15& \cone{0.00e+00}, 2e-15& \ctwo{6.68e+03}, 2e-15& 5.71e+04, 3e-08\cone{(+)}& 1.92e+04, 6e-04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 7.91e+05, 6e-07& 5.95e+05, 5e-03& \cone{0.00e+00}, 3e-15& \cthree{2.16e+04}, 1e-15& \ctwo{2.12e+04}, 1e-15& 5.06e+05, 6e-07\cone{(+)}& 3.53e+05, 5e-03\cone{(+)}\\
CnnCaltech-3000-1000 & -4.9e+03 & 100 & 3.62e+03, 7e-07& 2.44e+03, 3e-03& \cone{0.00e+00}, 3e-15& \cthree{1.78e+02}, 1e-15& \ctwo{1.61e+02}, 2e-15& 2.09e+03, 7e-07\cone{(+)}& 8.27e+02, 3e-03\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 100 & 1.20e+05, 2e-07& 5.97e+04, 3e-03& \cone{0.00e+00}, 3e-15& \ctwo{5.10e+02}, 1e-15& \cthree{7.80e+02}, 1e-15& 2.98e+04, 2e-07\cone{(+)}& 4.22e+04, 3e-03\cone{(+)}\\
randn-500-1000 & -3.6e+04 & 100 & 6.37e+03, 1e-08& 3.53e+03, 2e-03& \cone{0.00e+00}, 4e-15& \cthree{1.10e+03}, 2e-15& \ctwo{3.46e+02}, 1e-15& 4.32e+03, 1e-08\cone{(+)}& 2.50e+03, 2e-03\cone{(+)}\\
 \hline
 \hline   \multicolumn{10}{|c|}{\centering time limit=60} \\ \hline
w1a-2477-300 & -5.2e+03 & 10 & 5.15e+02, 2e-13& 1.27e+03, 1e-05& 2.78e+02, 2e-13& 4.98e+02, 9e-14& \cthree{1.56e+02}, 1e-13& \cone{0.00e+00}, 2e-13\cone{(+)}& \ctwo{1.46e+02}, 1e-05\cone{(+)}\\
TDT2-500-1000 & -3.5e+00 & 10 & 9.22e-01, 1e-14& 9.39e-01, 1e-05& \cthree{5.16e-02}, 1e-13& \cone{0.00e+00}, 6e-14& \ctwo{2.66e-02}, 5e-14& 6.43e-01, 5e-14\cone{(+)}& 6.49e-01, 1e-05\cone{(+)}\\
20News-8000-1000 & -1.6e+00 & 10 & 5.09e-01, 1e-14& 5.22e-01, 9e-07& \cthree{1.83e-02}, 2e-13& \ctwo{6.49e-03}, 9e-14& \cone{0.00e+00}, 7e-14& 2.71e-01, 9e-14\cone{(+)}& 3.09e-01, 9e-07\cone{(+)}\\
sector-6412-1000 & -3.4e+01 & 10 & 2.04e+00, 1e-11& 2.29e+00, 5e-05& 1.46e+00, 2e-13& \cone{0.00e+00}, 2e-13& \ctwo{5.85e-02}, 1e-13& \cthree{9.61e-01}, 1e-11\cone{(+)}& 1.00e+00, 5e-05\cone{(+)}\\
E2006-2000-1000 & -6.2e-01 & 10 & 1.18e-01, 3e-15& 1.20e-01, 8e-06& \cthree{1.67e-03}, 7e-14& \cone{0.00e+00}, 2e-13& \ctwo{2.67e-05}, 6e-14& 7.55e-02, 4e-14\cone{(+)}& 9.28e-02, 8e-06\cone{(+)}\\
MNIST-60000-784 & -2.5e+05 & 10 & 4.52e+04, 3e-11& 6.19e+04, 2e-04& \cthree{3.11e+02}, 9e-14& \cone{0.00e+00}, 2e-14& \ctwo{1.25e+02}, 1e-14& 1.41e+03, 3e-11\cone{(+)}& 2.76e+04, 2e-04\cone{(+)}\\
Gisette-3000-1000 & -1.0e+06 & 10 & 4.23e+04, 9e-10& 2.62e+04, 4e-04& \cone{0.00e+00}, 7e-14& \cthree{6.86e+02}, 1e-14& \ctwo{6.03e+02}, 9e-15& 7.00e+03, 9e-10\cone{(+)}& 2.26e+03, 4e-04\cone{(+)}\\
CnnCaltech-3000-1000 & -3.4e+03 & 10 & 1.03e+03, 1e-14& 8.05e+02, 4e-05& \cone{0.00e+00}, 5e-14& \ctwo{1.58e+01}, 1e-14& \cthree{5.04e+01}, 9e-15& 4.62e+02, 4e-14\cone{(+)}& 2.08e+02, 4e-05\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 10 & 1.56e+04, 2e-09& 1.79e+04, 2e-04& \ctwo{5.10e+01}, 6e-14& \cthree{8.57e+01}, 1e-14& \cone{0.00e+00}, 1e-14& 9.32e+03, 2e-09\cone{(+)}& 2.44e+03, 2e-04\cone{(+)}\\
randn-500-1000 & -6.8e+03 & 10 & 6.74e+02, 2e-11& 3.23e+02, 3e-05& \cone{0.00e+00}, 5e-14& \cthree{1.95e+02}, 2e-14& 2.04e+02, 1e-14& 2.36e+02, 2e-11\cone{(+)}& \ctwo{2.77e+01}, 3e-05\cone{(+)}\\
 \hline
w1a-2477-300 & -6.6e+03 & 20 & 1.94e+03, 1e-12& 2.62e+03, 1e-05& 3.08e+02, 2e-13& \ctwo{1.60e+02}, 7e-14& \cthree{2.67e+02}, 4e-14& \cone{0.00e+00}, 1e-12\cone{(+)}& 3.08e+02, 1e-05\cone{(+)}\\
TDT2-500-1000 & -3.9e+00 & 20 & 1.05e+00, 1e-14& 1.06e+00, 1e-05& \cthree{8.31e-02}, 7e-14& \ctwo{3.93e-03}, 4e-14& \cone{0.00e+00}, 4e-14& 6.53e-01, 4e-14\cone{(+)}& 7.16e-01, 1e-05\cone{(+)}\\
20News-8000-1000 & -1.7e+00 & 20 & 6.53e-01, 2e-14& 6.69e-01, 6e-06& \cthree{1.13e-01}, 1e-13& \cone{0.00e+00}, 7e-14& \ctwo{3.17e-02}, 6e-14& 4.35e-01, 8e-14\cone{(+)}& 4.82e-01, 6e-06\cone{(+)}\\
sector-6412-1000 & -4.6e+01 & 20 & 4.87e+00, 2e-13& 4.90e+00, 1e-04& \cthree{2.10e+00}, 2e-13& \cone{0.00e+00}, 1e-13& \ctwo{4.08e-01}, 5e-14& 2.13e+00, 3e-13\cone{(+)}& 2.38e+00, 1e-04\cone{(+)}\\
E2006-2000-1000 & -6.5e-01 & 20 & 1.42e-01, 5e-15& 1.45e-01, 5e-06& \cthree{2.18e-03}, 8e-14& \cone{0.00e+00}, 6e-14& \ctwo{5.42e-04}, 3e-14& 1.02e-01, 2e-14\cone{(+)}& 1.13e-01, 5e-06\cone{(+)}\\
MNIST-60000-784 & -2.8e+05 & 20 & 7.55e+04, 7e-12& 1.08e+05, 3e-04& \ctwo{8.77e+02}, 6e-14& \cone{0.00e+00}, 2e-14& \cthree{1.04e+03}, 6e-15& 5.67e+04, 7e-12\cone{(+)}& 5.17e+04, 3e-04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 20 & 1.90e+05, 8e-09& 3.23e+04, 7e-04& \cone{0.00e+00}, 3e-14& \cthree{2.06e+03}, 5e-15& \ctwo{1.59e+03}, 4e-15& 5.05e+04, 8e-09\cone{(+)}& 8.92e+03, 7e-04\cone{(+)}\\
CnnCaltech-3000-1000 & -3.7e+03 & 20 & 1.53e+03, 4e-12& 1.41e+03, 1e-04& \ctwo{6.78e+00}, 3e-14& \cone{0.00e+00}, 5e-15& \cthree{4.81e+01}, 4e-15& 5.00e+02, 4e-12\cone{(+)}& 3.26e+02, 1e-04\cone{(+)}\\
Cifar-1000-1000 & -1.4e+05 & 20 & 2.70e+04, 2e-09& 4.88e+04, 4e-04& \cone{0.00e+00}, 3e-14& \ctwo{1.76e+02}, 5e-15& \cthree{2.54e+02}, 5e-15& 1.65e+04, 2e-09\cone{(+)}& 8.28e+03, 4e-04\cone{(+)}\\
randn-500-1000 & -1.1e+04 & 20 & 1.07e+03, 2e-11& 9.02e+02, 9e-05& \cone{0.00e+00}, 3e-14& \cthree{4.35e+02}, 6e-15& 4.49e+02, 5e-15& 6.91e+02, 2e-11\cone{(+)}& \ctwo{3.55e+02}, 9e-05\cone{(+)}\\
 \hline
w1a-2477-300 & -1.2e+04 & 100 & 6.75e+03, 1e-09& 8.98e+03, 6e-05& \ctwo{1.83e+01}, 5e-14& 1.45e+02, 3e-14& \cone{0.00e+00}, 1e-14& \cthree{5.73e+01}, 1e-09\cone{(+)}& 8.76e+01, 6e-05\cone{(+)}\\
TDT2-500-1000 & -4.8e+00 & 100 & 1.52e+00, 3e-14& 1.55e+00, 5e-05& \cthree{4.46e-01}, 5e-15& \cone{0.00e+00}, 1e-14& \ctwo{1.41e-02}, 9e-15& 1.22e+00, 4e-14\cone{(+)}& 1.27e+00, 5e-05\cone{(+)}\\
20News-8000-1000 & -2.0e+00 & 100 & 7.18e-01, 1e-08& 7.26e-01, 3e-05& \cthree{1.28e-01}, 5e-14& \cone{0.00e+00}, 4e-14& \ctwo{1.65e-03}, 5e-14& 5.91e-01, 1e-08\cone{(+)}& 6.26e-01, 3e-05\cone{(+)}\\
sector-6412-1000 & -8.6e+01 & 100 & 1.52e+01, 3e-09& 2.69e+01, 8e-04& 1.09e+01, 8e-14& \ctwo{8.85e-02}, 5e-14& \cone{0.00e+00}, 4e-14& \cthree{9.94e+00}, 3e-09\cone{(+)}& 1.13e+01, 8e-04\cone{(+)}\\
E2006-2000-1000 & -6.9e-01 & 100 & 1.64e-01, 5e-14& 1.67e-01, 5e-07& \cthree{2.06e-02}, 8e-15& \cone{0.00e+00}, 4e-14& \ctwo{6.25e-05}, 4e-14& 1.34e-01, 5e-14\cone{(+)}& 1.43e-01, 5e-07\cone{(+)}\\
MNIST-60000-784 & -3.6e+05 & 100 & 1.63e+05, 1e-08& 3.45e+05, 4e-04& \cone{0.00e+00}, 5e-15& \ctwo{1.94e+03}, 2e-15& \cthree{8.98e+03}, 2e-14& 6.47e+04, 1e-08\cone{(+)}& 2.92e+04, 4e-04\cone{(+)}\\
Gisette-3000-1000 & -1.1e+06 & 100 & 6.45e+05, 4e-07& 5.89e+05, 3e-03& \cone{0.00e+00}, 5e-15& \ctwo{1.49e+04}, 2e-15& \cthree{1.60e+04}, 1e-15& 3.93e+05, 4e-07\cone{(+)}& 3.26e+05, 3e-03\cone{(+)}\\
CnnCaltech-3000-1000 & -5.0e+03 & 100 & 3.74e+03, 4e-08& 2.57e+03, 8e-04& \cone{0.00e+00}, 5e-15& \cthree{1.85e+02}, 2e-15& \ctwo{1.77e+02}, 2e-15& 2.19e+03, 4e-08\cone{(+)}& 9.76e+02, 8e-04\cone{(+)}\\
Cifar-1000-1000 & -1.5e+05 & 100 & 1.21e+05, 5e-08& 6.10e+04, 1e-03& \cone{0.00e+00}, 5e-15& \ctwo{4.59e+02}, 2e-15& \cthree{7.68e+02}, 2e-15& 5.51e+04, 5e-08\cone{(+)}& 4.07e+04, 1e-03\cone{(+)}\\
randn-500-1000 & -3.7e+04 & 100 & 7.17e+03, 1e-10& 4.36e+03, 9e-04& \cone{0.00e+00}, 6e-15& \cthree{1.26e+03}, 2e-15& \ctwo{4.94e+02}, 2e-15& 5.02e+03, 1e-10\cone{(+)}& 3.32e+03, 9e-04\cone{(+)}\\
 \hline
\end{tabular}}
\caption{Comparisons of objective values and the violation of the constraints $(F(\X)-F_{\text{min}} , \|\min(\mathbf{0},\X)\|_{\fro} + \|\X\trans \X - \I_r\|_{\fro})$ for nonnegative PCA for all the compared methods. The $1^{st}$, $2^{nd}$, and $3^{rd}$ best results are colored with \cone{red}, \ctwo{blue} and \cthree{green}, respectively.}
\label{tab:NNPCA}
%\vspace{-10pt}
\end{table*}






